READY or Not: Reliable Enterprise Agent Deployment

An AI agent can perform well on benchmarks and still be unsuitable for deployment. Existing AI-agent benchmarks measure whether an agent can complete realistic professional work, whereas enterprise deployment asks a different question: whether an agent can meet a required reliability level, under acceptable human oversight, and at tolerable cost. We introduce Reliable Enterprise Agent Deployment (READY), a framework for qualifying AI agents for deployment on enterprise workflows. READY preserves each workflow's own definition of successful execution while applying a common qualification procedure. Given an agent, a workflow, and a class of candidate oversight policies, READY measures the reliability and operating cost of the human-AI system, selects the minimum-cost policy that satisfies a specified reliability target, and statistically qualifies it on held-out cases. The resulting deployment profile characterizes the supported operating point: reliability, human-oversight burden, and cost. READY is implemented as an open testbed that decouples workflow specification, execution, evaluation, and qualification, and runs on existing agent-evaluation infrastructure. In an end-to-end clinical-audit case study spanning 16 agent systems and 750 cases, READY reveals differences hidden by autonomous performance: two systems separated by only 0.3 points in autonomous accuracy (72.8% vs. 72.5%) require 39.2% versus 29.6% human review, respectively, to qualify at the same 76% reliability target under the evaluated oversight policy. READY thus shifts enterprise agent evaluation from how well can the agent perform the work? to under what conditions, and at what cost, can it be reliably deployed? By making those conditions explicit and statistically testable, READY provides a basis for comparing agent systems, setting oversight requirements, and making evidence-based deployment decisions.

==> figures/cost-reliability-figure.tex <==
% Cost-of-reliability figure (input-able into a figure environment).
% Requires: \usepackage{pgfplots}\pgfplotsset{compat=1.18}
% Reads pse-cost-data.csv: total $/case vs target reliability Y for
% representative PSEBench models, at the default human-review cost k_h=$25.
% Regenerate the data with gen_paper_results.py.

\definecolor{efeA}{HTML}{1F4EFF}  % GPT-5.5
\definecolor{efeB}{HTML}{0E7C66}  % Gemini 3.1 Pro
\definecolor{efeC}{HTML}{7A3CC4}  % Claude Opus 4.7
\definecolor{efeD}{HTML}{B4690E}  % GPT-5
\definecolor{efeE}{HTML}{697077}  % DeepSeek-R1
\definecolor{efeF}{HTML}{9B2242}  % GPT-5-nano

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth, height=0.62\linewidth,
    xlabel={Target reliability $Y$ (\%)},
    ylabel={Total cost per case (\$)},
    xmin=90, xmax=99,
    ymin=0, ymax=27,
    xtick={90,92,94,96,98},
    legend pos=north west,
    legend cell align=left,
    legend style={font=\small, draw=none, fill=none},
    grid=both, grid style={line width=.2pt, draw=gray!18},
    major grid style={line width=.2pt, draw=gray!30},
    tick align=outside,
    every axis plot/.append style={line width=1.2pt},
]
  % all-human baseline ($25/case)
  \addplot[dashed, line width=1pt, color=efeF, forget plot]
    coordinates {(90,25) (99,25)};
  \node[anchor=north east, font=\small, color=efeF] at (axis cs:99,25) {all-human \$25};

  \addplot[color=efeA] table[col sep=comma, x=Y, y=gpt55]{pse-cost-data.csv};
  \addlegendentry{GPT-5.5}
  \addplot[color=efeB] table[col sep=comma, x=Y, y=gemini]{pse-cost-data.csv};
  \addlegendentry{Gemini 3.1 Pro}
  \addplot[color=efeC] table[col sep=comma, x=Y, y=opus]{pse-cost-data.csv};
  \addlegendentry{Claude Opus 4.7}
  \addplot[color=efeD, densely dashed] table[col sep=comma, x=Y, y=gpt5]{pse-cost-data.csv};
  \addlegendentry{GPT-5}
  \addplot[color=efeE] table[col sep=comma, x=Y, y=deepseek]{pse-cost-data.csv};
  \addlegendentry{DeepSeek-R1}
  \addplot[color=efeF] table[col sep=comma, x=Y, y=nano]{pse-cost-data.csv};
  \addlegendentry{GPT-5-nano}
\end{axis}
\end{tikzpicture}


==> old/conclude.tex <==

% ==================================================================
\section{Conclusion and Call to Participation}
\label{sec:conclusion}
% ==================================================================

Enterprise deployment requires more than evidence that an agent can complete
a valuable task. It requires evidence that the agent can operate within a
defined workflow, authority boundary, reliability target, risk tolerance,
and human-oversight policy.

EFE converts enterprise-agent evaluation from a task score into a
conditional and auditable deployment profile. \PSEBench{} and
\CliniCARE{} demonstrate that the open standard and implemented platform
operate end to end. The next stage is to expand EFE through contributed
enterprise workflows, task instances, environments, policies, assets,
graders, and oversight methods.

\begin{quote}
\textbf{The question is no longer only whether an agent can do the work,
but where it can operate, under what authority and oversight, with what
residual risk, and at what total cost.}
\end{quote}


==> old/contribution_bk_0810.tex <==

% ==================================================================
\section{Open Contribution Program}
\label{sec:contribution}
% ==================================================================

\subsection{What Can Be Contributed}
\label{sec:contribution-what}

Contributions may include:

\begin{itemize}
    \item enterprise workflow templates;
    \item concrete task instances;
    \item governed enterprise assets;
    \item policy and regulatory corpora;
    \item executable environments;
    \item expert reference work products;
    \item deterministic and rubric-based graders;
    \item human-review and oversight studies;
    \item red-team and adversarial scenarios;
    \item new reliability and escalation methods.
\end{itemize}


\subsection{Who Participates}
\label{sec:contribution-who}

EFE is intended to support collaboration among:

\begin{itemize}
    \item enterprises and workflow owners;
    \item domain practitioners;
    \item AI and evaluation researchers;
    \item model and agent developers;
    \item evaluation engineers;
    \item security, privacy, and governance experts.
\end{itemize}


\subsection{Contribution Lifecycle}
\label{sec:contribution-lifecycle}

A contribution proceeds through:

\begin{enumerate}
    \item workflow nomination;
    \item scope, rights, privacy, and feasibility review;
    \item EFE standard encoding;
    \item task and reference construction;
    \item domain-expert validation;
    \item agent dry runs;
    \item grader validation;
    \item benchmark acceptance;
    \item release, monitoring, and maintenance.
\end{enumerate}


\subsection{Participation and Access Modes}
\label{sec:contribution-access}

EFE supports public, gated, private, and server-side contributions. Openness
of the standard and evaluation methodology does not require unrestricted
release of confidential enterprise data.


\subsection{Expansion Priorities}
\label{sec:contribution-priorities}

Expansion priorities include:

\begin{itemize}
    \item additional industries, including finance, legal, insurance, retail,
          manufacturing, government, and life sciences;
    \item state-changing enterprise workflows;
    \item open user-facing task-completion workflows;
    \item new policy, privacy, and adversarial evaluation surfaces;
    \item cross-domain reliability and oversight methods.
\end{itemize}


% ==================================================================
\section{Governance and Benchmark Evolution}
\label{sec:governance}
% ==================================================================

\subsection{Standard Stewardship and Decision Rights}
\label{sec:governance-stewardship}

% TODO:
% Define:
% - standard maintainer;
% - schema-change process;
% - contributor decision rights;
% - technical steering and domain advisory mechanisms.


\subsection{Task Acceptance and Validation}
\label{sec:governance-acceptance}

A task enters EFE only after review for:

\begin{itemize}
    \item workflow authenticity;
    \item gradeability;
    \item data and asset rights;
    \item policy correctness;
    \item safety and privacy;
    \item evaluator quality;
    \item benchmark difficulty and discrimination.
\end{itemize}


\subsection{Versioning and Backward Compatibility}
\label{sec:governance-versioning}

EFE separately versions:

\begin{itemize}
    \item the open standard;
    \item workflow templates;
    \item task instances;
    \item benchmark releases;
    \item policy corpora;
    \item environments;
    \item graders;
    \item evaluated agent configurations.
\end{itemize}


\subsection{Benchmark Integrity and Contamination Controls}
\label{sec:governance-integrity}

% TODO:
% Cover:
% - hidden and private evaluation instances;
% - server-side evaluation;
% - task rotation;
% - contamination monitoring;
% - reference protection;
% - submission logging and rate limits.


\subsection{Data Governance and Privacy}
\label{sec:governance-privacy}

% TODO:
% Cover:
% - data rights;
% - de-identification;
% - access control;
% - audit logs;
% - retention;
% - permitted derivative artifacts;
% - contributor and evaluator confidentiality.


\subsection{Appeals, Corrections, and Errata}
\label{sec:governance-appeals}

% TODO:
% Define:
% - score appeals;
% - grader-error review;
% - task-defect correction;
% - benchmark errata;
% - preservation of historical results.


\subsection{Refresh, Retirement, and Requalification}
\label{sec:governance-refresh}

EFE qualification is specific to the evaluated model, agent harness,
environment, policy corpus, benchmark version, and deployment assumptions.
Material changes to these components may require requalification.


% \input{sections/11_call_for_participation}


==> old/intro_bk_0810.tex <==

% ==================================================================
\section{Introduction: Enterprise Deployment Requires a Different Exam}
\label{sec:introduction}
% ==================================================================

\subsection{From Task Completion to Safe Employment}
\label{sec:intro-safe-employment}

% Key message:
% Professional-work benchmarks ask whether an agent can do the work.
% EFE asks whether an organization can safely employ the agent under
% a specified operating policy and at an acceptable total cost.

AI-agent benchmarks increasingly evaluate authentic professional work,
long-horizon computer use, tool use, and economically valuable task
completion. These evaluations answer an important question: can an agent
produce the requested work product or reach the intended task state?

Enterprise deployment requires a different exam. An organization must
determine not only whether an agent can complete a task, but whether it can
be employed within a defined role, authority boundary, oversight policy,
reliability requirement, and cost budget. A system may produce a strong work
product and still be unsuitable for deployment if it relies on unsupported
evidence, exceeds its authority, fails to escalate ambiguous cases, performs
an unauthorized write, or requires economically prohibitive human review.

\begin{quote}
\textbf{Professional-work benchmarks ask whether an agent can do the work.
Enterprise's First Exam asks whether an organization can safely employ the
agent, under what operating policy, and at what total cost.}
\end{quote}


\subsection{The Unit of Evaluation}
\label{sec:intro-unit}

EFE evaluates the joint system
\begin{equation}
    \text{Agent}
    \times
    \text{Workflow}
    \times
    \text{Deployment Policy}.
    \label{eq:efe-unit}
\end{equation}

The agent is therefore not assigned a context-free designation such as
``enterprise ready.'' Qualification is conditional on a particular workflow,
execution environment, authority envelope, risk tolerance, reliability
target, and human-oversight policy.


\subsection{EFE at Launch}
\label{sec:intro-launch}

EFE is an implemented platform and open standard, rather than a proposal for
a future benchmark. The initial release includes:

\begin{itemize}
    \item an open task and deployment standard;
    \item an implemented agent-execution and evaluation platform;
    \item an oversight simulator and deployment-profile generator;
    \item two completed seed benchmarks, \PSEBench{} and \CliniCARE{};
    \item an open contribution process for expanding EFE to additional
          industries, workflows, risk surfaces, and evaluation methods.
\end{itemize}

\PSEBench{} and \CliniCARE{} are completed reference implementations of the
EFE standard. They demonstrate how an authentic enterprise workflow is
specified, instantiated in a controlled environment, executed by different
agent systems, evaluated through reusable reliability primitives, and
translated into a deployment profile.


\subsection{Positioning and Contributions}
\label{sec:intro-contributions}

EFE makes five primary contributions:

\begin{enumerate}
    \item \textbf{An open enterprise-agent evaluation standard.}
    EFE defines a canonical representation of deployment tracks, risk
    surfaces, agent authority, expected end states, escalation requirements,
    consequence and reversibility, and evaluation requirements.

    \item \textbf{An implemented evaluation platform.}
    EFE executes heterogeneous agent systems in controlled environments,
    records immutable trajectories and state changes, evaluates outcomes and
    processes, and simulates candidate oversight policies.

    \item \textbf{A deployment-qualification methodology.}
    EFE combines hard safety and authority gates with reliability,
    autonomous coverage, escalation behavior, and oversight-adjusted
    operating cost.

    \item \textbf{Two completed seed benchmarks.}
    \PSEBench{} and \CliniCARE{} provide the first end-to-end reference
    implementations of the EFE standard and platform.

    \item \textbf{An open contribution and governance model.}
    EFE enables enterprises, domain experts, researchers, and agent
    developers to contribute additional workflows, environments, policies,
    task instances, graders, and reliability methods.
\end{enumerate}


==> old/metrics_bk_0810.tex <==

% ==================================================================
\section{Deployment Qualification:
Safety Gates, Reliability, and Oversight Economics}
\label{sec:qualification}
% ==================================================================

\subsection{Three Layers of Qualification}
\label{sec:qualification-layers}

EFE deployment qualification has three layers:

\begin{enumerate}
    \item \textbf{Hard safety and authority gates.}
    The system must satisfy non-negotiable privacy, security, authority,
    policy, safety, and auditability requirements.

    \item \textbf{Reliability and autonomy frontier.}
    The evaluation determines what fraction of work can be completed
    autonomously while meeting a specified reliability target.

    \item \textbf{Oversight economics.}
    Among policies satisfying the gates and target reliability, EFE selects
    the policy with the lowest expected model, review, approval, escalation,
    and recovery cost.
\end{enumerate}


\subsection{Hard Safety and Authority Gates}
\label{sec:qualification-gates}

Hard gates may include:

\begin{itemize}
    \item zero tolerance for specified prohibited actions;
    \item upper bounds on critical safety or privacy violations;
    \item authority and approval compliance;
    \item minimum evidence traceability;
    \item minimum logging and auditability;
    \item required escalation under specified conditions.
\end{itemize}


\subsection{One-Shot Accept-or-Escalate Formulation}
\label{sec:qualification-one-shot}

For verdict-oriented evidence-grounded tasks, let each case be represented by
an input--label pair $(x_i,y_i)$. The agent produces a verdict and confidence:

\begin{equation}
    m(x_i) = (\hat{y}_i,s_i),
    \qquad s_i \in [0,1].
    \label{eq:model-output}
\end{equation}

A threshold policy handles the case autonomously when $s_i \geq \tau$ and
escalates it otherwise.


\subsection{Reliability, Autonomy, and Cost}
\label{sec:qualification-cost}

Let $c$ denote autonomous coverage, $a(c)$ the accuracy among autonomously
handled cases, $a_h$ human-review accuracy, $k_m$ model cost per case, and
$k_h$ human-review cost per escalated case. System reliability is

\begin{equation}
    R(c)
    =
    c\,a(c) + (1-c)a_h.
    \label{eq:system-reliability}
\end{equation}

Expected operating cost is

\begin{equation}
    C(c)
    =
    k_m + k_h(1-c).
    \label{eq:operating-cost}
\end{equation}

For a target reliability $Y$, the cost-optimal autonomous coverage is

\begin{equation}
    c^{\star}(Y)
    =
    \max\left\{
        c \in [0,1] : R(c) \geq Y
    \right\},
    \label{eq:optimal-coverage}
\end{equation}

and the corresponding oversight-adjusted operating cost is

\begin{equation}
    C^{\star}(Y)
    =
    k_m + k_h\left(1-c^{\star}(Y)\right).
    \label{eq:cost-reliability}
\end{equation}


\subsection{Confidence Discrimination, Calibration, and Threshold Validity}
\label{sec:qualification-confidence}

EFE distinguishes three properties:

\begin{description}
    \item[Discrimination.]
    Whether confidence ranks correct or safely autonomous cases ahead of
    incorrect or escalation-worthy cases.

    \item[Calibration.]
    Whether reported numerical confidence corresponds to empirical
    correctness probabilities.

    \item[Threshold validity.]
    Whether a policy selected on development data continues to satisfy its
    reliability requirement on held-out or shifted data.
\end{description}


\subsection{Oracle and Discrimination Diagnostics}
\label{sec:qualification-diagnostics}

% TODO:
% Present:
% - risk--autonomy curve;
% - AURC;
% - E-AURC;
% - oracle escalation policy;
% - oracle cost floor;
% - cost gap caused by imperfect discrimination.
%
% Consider moving the full Beta-model derivation to an appendix.


\subsection{Deployment-Profile Generation}
\label{sec:qualification-profile}

The deployment profile combines:

\begin{itemize}
    \item hard-gate outcomes;
    \item achievable reliability;
    \item autonomous coverage;
    \item required escalation and approval policies;
    \item residual risk by failure class;
    \item expected oversight and operating cost.
\end{itemize}


\subsection{Extensions to Stateful and Interactive Workflows}
\label{sec:qualification-extensions}

For state-changing and open-interaction workflows, oversight may occur at
multiple points. At each decision point, an agent may:

\begin{itemize}
    \item act autonomously;
    \item propose an action for approval;
    \item ask for clarification;
    \item retry or recover;
    \item escalate to a human;
    \item terminate without acting.
\end{itemize}

% TODO:
% Add the generalized multi-stage risk-constrained cost objective.


\subsection{Statistical Qualification Protocol}
\label{sec:qualification-statistics}

% TODO:
% Specify:
% - development and held-out qualification splits;
% - lower confidence bounds on reliability;
% - upper confidence bounds on critical violation rates;
% - repeated-trial requirements;
% - minimum sample sizes by risk class;
% - bootstrap confidence intervals;
% - requalification triggers after changes to models, tools, policies,
%   environments, or task distributions.


==> old/metrics_bk_0817.tex <==
% ==================================================================
\section{Deployment Qualification:
Safety Gates, Reliability, and Oversight Economics}
\label{sec:qualification}
% ==================================================================

The EFE standard specifies what must be measured about an enterprise
workflow; deployment qualification determines how those measurements are
translated into an operating policy.

The central principle is that qualification is conditional rather than
absolute. EFE does not assign an agent a context-free label such as
``enterprise ready.'' It asks whether a particular agent configuration can
operate within a specified workflow, environment, authority boundary,
consequence class, reliability requirement, and oversight policy.

Formally, EFE treats deployment as a constrained policy-selection problem.
The objective is not maximal autonomy. It is to identify the least costly
deployment policy that satisfies the workflow's non-negotiable gates and
reliability requirements while respecting the deployment contract defined
in Section~\ref{sec:standard-contract}.

% ------------------------------------------------------------------
\subsection{Three Layers of Qualification}
\label{sec:qualification-layers}
% ------------------------------------------------------------------

EFE deployment qualification has three layers.

\begin{enumerate}

    \item \textbf{Hard safety and authority gates.}
    The system must first satisfy the non-negotiable requirements declared
    by the task's evaluation profile. These may concern privacy, security,
    authority, policy compliance, prohibited actions, evidence traceability,
    required escalation, or auditability. A system that fails a hard gate is
    not qualified for the corresponding deployment contract regardless of
    its average task performance.

    \item \textbf{Reliability and autonomy frontier.}
    Among systems that satisfy the hard gates, EFE estimates which portions
    of the workflow can be handled autonomously while meeting a specified
    reliability requirement. The resulting frontier describes the tradeoff
    between autonomous coverage and residual risk rather than reducing the
    system to a single accuracy score.

    \item \textbf{Oversight economics.}
    Among deployment policies that satisfy the gates and reliability
    requirement, EFE evaluates the expected cost of model execution, human
    review, approval, escalation, and recovery. The preferred policy is the
    minimum-cost feasible policy under the deployment assumptions supplied
    by the organization.

\end{enumerate}

The three layers are ordered. Economic advantage cannot compensate for a
hard-gate violation, and increased autonomous coverage is useful only while
the required reliability remains satisfied.

The mathematical form of the reliability--autonomy frontier depends on the
workflow. We first develop a one-shot accept-or-escalate formulation, which
applies directly to verdict-oriented evidence-grounded workflows such as the
two seed benchmarks in Section~\ref{sec:seed-benchmarks}. We then generalize
the qualification objective to stateful and interactive workflows in
Section~\ref{sec:qualification-extensions}.

% ------------------------------------------------------------------
\subsection{Hard Safety and Authority Gates}
\label{sec:qualification-gates}
% ------------------------------------------------------------------

Hard gates operationalize requirements that should not be averaged into an
aggregate benchmark score. Let $\mathcal{G}$ denote the set of gates declared
by the task's evaluation profile. A gate $g \in \mathcal{G}$ specifies a
measurable failure condition and an allowable tolerance $\epsilon_g$.

Examples include:

\begin{itemize}
    \item prohibited actions that must never be observed;
    \item upper bounds on critical safety, privacy, or security violations;
    \item compliance with role, authority, and approval boundaries;
    \item required escalation or abstention under specified conditions;
    \item minimum evidence and policy traceability;
    \item minimum logging and audit completeness; and
    \item workflow-specific safety constraints associated with the
    consequence class.
\end{itemize}

For a trial $z$, let
\[
V_g(z) \in \{0,1\}
\]
indicate whether gate $g$ is violated. Qualification requires the estimated
violation rate to remain within the declared tolerance,

\begin{equation}
\Pr\!\left[V_g(Z)=1\right] \leq \epsilon_g,
\qquad
\forall g \in \mathcal{G}.
\label{eq:gate-constraint}
\end{equation}

Some gates are \emph{event-disqualifying}: observing even one specified
prohibited action is sufficient to reject the evaluated configuration for
that deployment contract. Other gates permit a small nonzero failure rate,
but qualification must establish that the corresponding statistical upper
bound remains below the declared tolerance.

A ``zero-tolerance'' deployment requirement should therefore not be
interpreted as statistical proof that the true violation probability is
exactly zero. EFE reports both the absence or presence of observed
violations and the uncertainty supported by the available evaluation
sample.

Hard-gate results remain separate from continuous or aggregate performance
measures. In particular, high outcome accuracy cannot compensate for an
unauthorized action, privacy breach, required-escalation failure, or
unverifiable audit trail.

% ------------------------------------------------------------------
\subsection{One-Shot Accept-or-Escalate Formulation}
\label{sec:qualification-one-shot}
% ------------------------------------------------------------------

We first consider a common Track~1 deployment pattern: an agent completes a
case, produces a gradeable outcome together with a scalar confidence or
other ranking signal, and the deployment policy either accepts the result
autonomously or sends the case to a human review path.

Let the benchmark contain cases

\begin{equation}
\mathcal{D}
=
\{(x_i,y_i)\}_{i=1}^{N},
\end{equation}

where $x_i$ is the task input and $y_i$ is the reference outcome. The
evaluated system produces

\begin{equation}
m(x_i)
=
(\hat{y}_i,s_i),
\qquad
s_i \in [0,1],
\label{eq:model-output}
\end{equation}

where $s_i$ is a confidence or ranking signal associated with the proposed
outcome.

A threshold policy $\pi_\tau$ accepts the result autonomously when

\[
s_i \geq \tau
\]

and escalates the case otherwise. Define

\begin{align}
c(\tau)
&=
\Pr(s \geq \tau),
&&\text{autonomous coverage},
\label{eq:coverage}
\\
e(\tau)
&=
1-c(\tau),
&&\text{escalation rate},
\label{eq:escalation}
\\
r(c)
&=
\Pr(\hat{y}\neq y \mid s\geq\tau),
&&\text{selective risk},
\label{eq:selective-risk}
\\
a(c)
&=
1-r(c),
&&\text{selective accuracy}.
\label{eq:selective-accuracy}
\end{align}

Sweeping $\tau$ produces the \emph{risk--autonomy frontier}. At
$c=1$, all cases are handled autonomously and

\[
a(1)=a_0,
\]

where $a_0$ is the system's ordinary full-autonomy task accuracy.
Reducing coverage is useful only when the ranking signal preferentially
removes cases on which the autonomous system is likely to fail.

This formulation does not require the numerical confidence values to be
calibrated probabilities. Any score that induces a case ordering can be
used to construct the empirical risk--autonomy curve.

% ------------------------------------------------------------------
\subsection{Reliability, Autonomy, and Cost}
\label{sec:qualification-cost}
\label{sec:cost-reliability}
% ------------------------------------------------------------------

Let $a_h$ denote the correctness of the escalated path and $k_h$ its
incremental cost per escalated case. The escalated path may represent an
independent human review or a human reviewing and correcting an
agent-produced artifact; $a_h$ and $k_h$ should be defined according to the
actual deployment being modeled.

Let $k_m$ denote the expected agent-execution cost incurred before the
accept-or-escalate decision, including model and other execution costs that
the deployment chooses to include.

Under the basic assumption that $a_h$ is constant across escalated cases,
system-level reliability at autonomous coverage $c$ is

\begin{equation}
R(c)
=
c\,a(c)
+
(1-c)a_h.
\label{eq:system-reliability}
\end{equation}

Expected operating cost is

\begin{equation}
C(c)
=
k_m
+
k_h(1-c).
\label{eq:operating-cost}
\end{equation}

For a required reliability $Y$, EFE selects the largest autonomous coverage
that satisfies the requirement,

\begin{equation}
c^{\star}(Y)
=
\max
\left\{
c \in [0,1]:
R(c)\geq Y
\right\},
\label{eq:optimal-coverage}
\end{equation}

and reports the corresponding oversight-adjusted operating cost,

\begin{equation}
C^{\star}(Y)
=
k_m
+
k_h\left(1-c^{\star}(Y)\right).
\label{eq:cost-reliability}
\end{equation}

Equivalently, writing

\[
e^{\star}(Y)=1-c^{\star}(Y),
\]

the headline one-shot quantity is

\begin{equation}
\boxed{
C^{\star}(Y)
=
k_m
+
k_h e^{\star}(Y)
}.
\label{eq:headline-cost}
\end{equation}

This quantity has a direct operational interpretation: the cost of running
the agent on every case plus the residual human oversight required to meet
the target reliability.

The all-human baseline is a separate deployment policy in which the agent
is not run. If the same human process costs $k_h$ per case, its cost is
$k_h$, whereas a policy that runs the agent and then escalates every case
costs $k_m+k_h$. EFE therefore reports both absolute operating cost and,
where appropriate, savings relative to the declared human baseline.

\paragraph{The reliability ceiling need not equal human accuracy.}
Reliability is not necessarily monotone as autonomy decreases. Once the
deployment begins escalating cases on which the agent would have been more
reliable than the human path, additional escalation can reduce reliability
while increasing cost. Equation~\ref{eq:optimal-coverage} therefore selects
the \emph{largest} coverage satisfying the target rather than assuming that
more escalation is always better.

With a perfect ranking that keeps every correct autonomous result and
escalates every incorrect one, the maximum achievable reliability is

\begin{equation}
R_{\max}
=
a_0
+
a_h(1-a_0),
\label{eq:oracle-reliability-ceiling}
\end{equation}

which may exceed $a_h$ because the deployed system combines the agent's
correct cases with human recovery on its errors.

\paragraph{Case-dependent human performance.}
The constant-$a_h$ assumption is a convenience, not a requirement of EFE.
Because escalation deliberately routes harder cases to humans, human
performance may itself depend on the selected subset. When data are
available, Equation~\ref{eq:system-reliability} should instead use the
empirically estimated conditional performance $a_h(c)$:

\begin{equation}
R(c)
=
c\,a(c)
+
(1-c)a_h(c).
\label{eq:system-reliability-conditional-human}
\end{equation}

Likewise, case-dependent review or recovery cost can replace the constant
$k_h$. EFE requires these assumptions to be stated in the deployment
profile rather than treating them as benchmark measurements.

% ------------------------------------------------------------------
\subsection{Confidence Discrimination, Calibration, and Threshold Validity}
\label{sec:qualification-confidence}
% ------------------------------------------------------------------

EFE distinguishes three properties of an uncertainty or routing signal.

\begin{description}

    \item[Discrimination.]
    Whether the signal ranks cases that are safe for autonomous handling
    ahead of cases that are incorrect, unsafe, or otherwise require
    escalation. Discrimination determines the shape of the
    risk--autonomy frontier.

    \item[Calibration.]
    Whether the numerical value of the signal corresponds to an empirical
    probability of correctness or another declared event. Calibration is
    important when the numerical score itself has operational meaning, but
    it is not required to construct a rank-based risk--autonomy curve.

    \item[Threshold validity.]
    Whether an operating policy selected using development data continues
    to satisfy its reliability and gate requirements on a held-out
    qualification set and, where measured, under relevant distribution
    shift.

\end{description}

These properties should not be conflated. A system may be poorly calibrated
but still provide a useful ordering for selective autonomy. Conversely, a
globally calibrated score can provide weak discrimination among the cases
near the deployment threshold.

For deployment-policy selection, the threshold or routing rule is chosen on
development data and then frozen before qualification. A threshold that
achieves $R(c)\geq Y$ on the same examples used to select it does not by
itself establish deployment reliability.

When many examples share an identical routing score, EFE treats the tied
set as a common operating group unless the deployment policy declares an
additional pre-specified feature for separating them. This avoids creating
artificial performance from an arbitrary ordering within tied confidence
values.

% ------------------------------------------------------------------
\subsection{Oracle and Discrimination Diagnostics}
\label{sec:qualification-diagnostics}
% ------------------------------------------------------------------

EFE reports diagnostics that separate three factors that determine selective
deployment performance:

\begin{enumerate}
    \item base task capability;
    \item quality of the ranking or escalation signal; and
    \item the deployment target and human-review assumptions.
\end{enumerate}

\paragraph{Risk--autonomy curve and AURC.}
The risk--autonomy curve plots selective risk $r(c)$ against autonomous
coverage $c$. Its scalar summary is the area under the curve,

\begin{equation}
\mathrm{AURC}
=
\int_0^1 r(c)\,dc,
\label{eq:aurc}
\end{equation}

with lower values indicating better selective performance.

Raw AURC depends on base accuracy. If the full-autonomy accuracy is $a_0$,
a perfect ordering places all correct cases ahead of all incorrect cases.
The corresponding oracle risk curve is

\begin{equation}
r^{\star}(c)
=
\begin{cases}
0,
& c\leq a_0,
\\[4pt]
1-\dfrac{a_0}{c},
& c>a_0,
\end{cases}
\label{eq:oracle-risk}
\end{equation}

with

\begin{equation}
\mathrm{AURC}^{\star}
=
(1-a_0)
+
a_0\ln a_0.
\label{eq:optimal-aurc}
\end{equation}

EFE therefore reports excess AURC,

\begin{equation}
\mathrm{E\mbox{-}AURC}
=
\mathrm{AURC}
-
\mathrm{AURC}^{\star}
\geq 0,
\label{eq:eaurc}
\end{equation}

which isolates the discrimination deficit relative to the best ordering
possible at the system's observed base accuracy.

\paragraph{Oracle escalation cost.}
The same perfect ordering defines an economic lower bound. An oracle that
knows which autonomous outcomes are wrong would escalate those failures
first. For

\[
a_0 < Y
\leq
a_0+a_h(1-a_0),
\]

the minimum required oracle escalation rate is

\begin{equation}
e_{\mathrm{oracle}}^{\star}(Y)
=
\frac{Y-a_0}{a_h},
\label{eq:oracle-escalation}
\end{equation}

and the corresponding cost floor is

\begin{equation}
C_{\mathrm{oracle}}^{\star}(Y)
=
k_m
+
k_h
\frac{Y-a_0}{a_h}.
\label{eq:oracle-cost}
\end{equation}

If $Y\leq a_0$, no escalation is required by the oracle. If

\[
Y>a_0+a_h(1-a_0),
\]

the target is infeasible even under perfect discrimination given the
assumed human-review path.

The realized excess cost

\begin{equation}
\Delta(Y)
=
C^{\star}(Y)
-
C_{\mathrm{oracle}}^{\star}(Y)
\geq 0
\label{eq:discrimination-cost-gap}
\end{equation}

is the economic cost of imperfect routing. The system spends human effort
on some cases it could have handled correctly while failing to isolate all
of the cases on which autonomous handling is unsafe.

E-AURC and $\Delta(Y)$ are therefore complementary views of the same
discrimination deficit. E-AURC is target-independent and expressed in risk
units; $\Delta(Y)$ is evaluated at a particular deployment target and
expressed in operating-cost units.

The closed-form Beta model used to illustrate these relationships is not
required for EFE qualification and is therefore given in
Appendix~\ref{app:math}.

% ------------------------------------------------------------------
\subsection{Extensions to Stateful and Interactive Workflows}
\label{sec:qualification-extensions}
% ------------------------------------------------------------------

The one-shot formulation above is appropriate when oversight occurs after a
completed agent result and changes only whether that result is accepted or
escalated. State-changing and open-interaction workflows are more general:
oversight decisions can occur at multiple points and can change the future
trajectory itself.

At a decision point $t$, an EFE deployment policy may allow the agent to:

\begin{itemize}
    \item act autonomously;
    \item prepare or propose an action for approval;
    \item request clarification;
    \item retry or execute a recovery procedure;
    \item escalate responsibility to a human; or
    \item terminate without acting.
\end{itemize}

Let $h_t$ denote the observable workflow history at decision point $t$ and
let

\[
\pi(o_t\mid h_t)
\]

denote a deployment policy over oversight decisions $o_t$. Executing an
agent under policy $\pi$ induces a complete trajectory $Z^{\pi}$ containing
the agent's observations, actions, approvals, state transitions, user
interactions, recovery behavior, final outcome, and associated costs.

Let $L(Z^{\pi})\in[0,1]$ denote a workflow-defined deployment loss, with
$1-L$ representing deployment success or reliability. Let
$V_g(Z^{\pi})$ denote the hard-gate violation indicators defined above, and
let total deployment cost be decomposed as

\begin{equation}
K(Z^{\pi})
=
K_{\mathrm{agent}}
+
K_{\mathrm{review}}
+
K_{\mathrm{approval}}
+
K_{\mathrm{escalation}}
+
K_{\mathrm{recovery}}.
\label{eq:general-cost}
\end{equation}

The general EFE qualification problem is

\begin{equation}
\pi^{\star}
=
\arg\min_{\pi\in\Pi}
\mathbb{E}
\left[
K(Z^{\pi})
\right]
\label{eq:general-policy-objective}
\end{equation}

subject to

\begin{align}
\mathbb{E}
\left[
1-L(Z^{\pi})
\right]
&\geq Y,
\label{eq:general-reliability-constraint}
\\
\Pr
\left[
V_g(Z^{\pi})=1
\right]
&\leq \epsilon_g,
\qquad
g\in\mathcal{G},
\label{eq:general-gate-constraint}
\end{align}

together with any additional workflow-specific constraints declared by the
deployment contract.

This formulation subsumes the one-shot case. When the trajectory contains
one final accept-or-escalate decision, the only human cost is review, and
success is binary verdict correctness, Equations
\ref{eq:general-policy-objective}--\ref{eq:general-gate-constraint}
reduce to the reliability--autonomy problem of
Section~\ref{sec:qualification-cost}.

Two evaluation regimes must be distinguished.

\paragraph{Post-hoc policy replay.}
If oversight changes only whether an already-completed output is accepted or
escalated, multiple policies can be evaluated from the same saved trials.
Confidence-threshold routing for a completed evidence-grounded report is
the canonical example.

\paragraph{Policy-in-the-loop evaluation.}
If approval, clarification, retry, intervention, or escalation changes what
the agent subsequently observes or what actions remain available, the policy
changes the trajectory distribution itself. The candidate policy must then
be executed as part of the evaluation. Approval-before-commit, recovery
after a failed write, and interactive user workflows are examples.

EFE does not infer policy-in-the-loop outcomes from a trajectory generated
under another policy unless the required counterfactual is supported by the
record and evaluation design. This distinction prevents the qualification
layer from treating unsupported counterfactual simulations as measured
deployment performance.

For these more general workflows, the output may be a multidimensional
frontier over reliability, critical risk, autonomous action, human
intervention, and operating cost rather than a single scalar
cost-of-reliability curve.

% ------------------------------------------------------------------
\subsection{Statistical Qualification Protocol}
\label{sec:qualification-statistics}
% ------------------------------------------------------------------

Qualification concerns the performance of a deployment policy on future
cases, not merely its empirical score on a benchmark sample. EFE therefore
separates \emph{policy selection} from \emph{policy qualification}.

\paragraph{Development and qualification sets.}
Task instances used to select confidence thresholds, escalation rules,
approval policies, calibration maps, or other deployment-policy parameters
belong to a development set. Once selected, the agent configuration and
deployment policy are frozen and evaluated on a held-out qualification set.

The qualification set must not be used to search over thresholds and then
also be treated as an unbiased estimate of the selected threshold's
reliability. If a policy is modified in response to qualification results,
the modified policy requires a new held-out evaluation or another valid
qualification procedure.

\paragraph{Reliability bounds.}
Let $\widehat{R}(\pi)$ denote the observed reliability of a fixed deployment
policy on the qualification set. EFE reports an uncertainty interval rather
than using $\widehat{R}$ alone. For a required target $Y$, qualification
requires a one-sided lower confidence bound

\begin{equation}
R_{\mathrm{LCB}}(\pi)
\geq Y
\label{eq:reliability-lcb}
\end{equation}

at the confidence level declared by the benchmark or deployment contract.

For simple binary outcomes, this bound may be computed directly using an
appropriate binomial interval. For derived metrics, repeated observations,
or clustered task structures, EFE uses an uncertainty procedure consistent
with the sampling design, such as a task-level or cluster bootstrap. The
method and confidence level are part of the evaluation configuration.

\paragraph{Critical-failure bounds.}
For each gate $g$ with tolerated violation probability $\epsilon_g$, let
$p_g$ denote the true violation rate. Qualification requires an appropriate
one-sided upper confidence bound

\begin{equation}
p_{g,\mathrm{UCB}}
\leq
\epsilon_g.
\label{eq:violation-ucb}
\end{equation}

For event-disqualifying gates, an observed prohibited event causes immediate
failure regardless of the aggregate rate.

When no violations are observed in $n$ independent trials, the exact
one-sided $(1-\alpha)$ binomial upper bound is

\begin{equation}
p_{g,\mathrm{UCB}}
=
1-\alpha^{1/n}.
\label{eq:zero-event-bound}
\end{equation}

Equation~\ref{eq:zero-event-bound} makes explicit why ``no failures
observed'' is not equivalent to ``zero deployment risk.'' Certifying a
smaller tolerated failure probability requires correspondingly more
evidence.

\paragraph{Risk-class-dependent evidence requirements.}
EFE does not prescribe one universal minimum sample size for every workflow.
The required evidence depends on the consequence class, target reliability,
allowed critical-failure rate, heterogeneity of the workflow, and precision
required of the deployment decision. Higher-consequence workflows should
therefore declare tighter confidence requirements or lower tolerated
critical-failure rates and supply enough qualification trials to make those
requirements statistically testable.

If the evaluation sample is too small to establish the required bound, the
appropriate result is \emph{insufficient evidence for qualification}, not an
assumption that the requirement has been satisfied.

\paragraph{Repeated-trial reliability.}
For stochastic agents, the task specification may require multiple
independent attempts on the same task instance. EFE preserves both
per-attempt performance and per-instance consistency. Measures such as
avg@$k$, pass$^k$, critical-failure frequency, and agreement on incorrect
outcomes characterize different aspects of operational reliability and
should not be collapsed into a single mean score.

When repeated attempts on the same instance are used in statistical
inference, the dependence among those attempts must be respected; for
example, bootstrap resampling can occur at the task-instance level rather
than treating every attempt as an independent new task.

\paragraph{Shift and threshold validity.}
A deployment threshold is qualified only for the evaluation distribution
and workflow slices on which its validity has been established. Where
important deployment subpopulations or known shifts are represented, EFE
reports reliability and hard-gate outcomes separately for those slices.
Strong aggregate performance does not establish qualification for a
subpopulation with insufficient coverage or a materially different failure
distribution.

\paragraph{Requalification.}
Qualification is tied to the evaluation configuration defined in
Section~\ref{sec:standard-record}. Material changes to any component that
can affect behavior or measurement may trigger requalification, including:

\begin{itemize}
    \item the foundation model or model version;
    \item the agent harness, prompts, scaffolding, memory, or orchestration;
    \item tools, permissions, or action authority;
    \item environment or system-of-record interfaces;
    \item governing policies or policy corpus;
    \item deployment or oversight policy;
    \item task or production-data distribution;
    \item evaluator, grader, or hard-gate logic; or
    \item the benchmark release itself.
\end{itemize}

Some evaluator changes can be handled through regrading when the saved trial
record contains all information required by the new evaluator. Changes that
alter agent behavior, available information, authority, or the trajectory
require new execution.

% ------------------------------------------------------------------
\subsection{Deployment-Profile Generation}
\label{sec:qualification-profile}
% ------------------------------------------------------------------

The final qualification output is the EFE deployment profile. It records the
bounded operating envelope supported by the evidence rather than a global
claim about the agent.

For each qualified workflow or workflow slice, the profile reports:

\begin{itemize}
    \item the evaluated agent, environment, benchmark, policy, and grader
    versions;
    \item hard-gate pass or fail status;
    \item the qualified workflow scope;
    \item the consequence and reversibility class;
    \item the authority granted to the agent;
    \item actions permitted autonomously;
    \item actions requiring approval, clarification, or escalation;
    \item the target and achieved reliability, with statistical uncertainty;
    \item autonomous coverage or the corresponding multi-stage autonomy
    measures;
    \item residual risk by observed failure class;
    \item required monitoring, audit, and recovery provisions;
    \item expected human-review or approval burden; and
    \item expected model, oversight, recovery, and total operating cost.
\end{itemize}

The profile must distinguish three kinds of quantities:

\begin{enumerate}
    \item \textbf{measured quantities}, obtained directly from benchmark
    trials, such as task outcomes, confidence, state changes, violations,
    trajectories, and resource use;

    \item \textbf{deployment assumptions}, such as human-review accuracy,
    reviewer cost, approval latency, or recovery cost; and

    \item \textbf{derived quantities}, such as system reliability,
    autonomous coverage, escalation burden, and oversight-adjusted operating
    cost.
\end{enumerate}

Keeping these categories separate allows the same benchmark evidence to be
reinterpreted under a different enterprise reliability target or human-cost
model without changing the underlying measured results.

The deployment profile therefore answers the operational question posed by
EFE:

\begin{quote}
\textbf{Where can this agent operate, under what authority and oversight,
with what residual risk, and at what total cost?}
\end{quote}

Qualification remains conditional on the evaluated configuration. A
materially changed model, harness, environment, authority boundary, policy
corpus, deployment policy, or benchmark distribution may invalidate all or
part of the profile and require requalification.

==> old/metrics_bk_0830.tex <==
\section{Oversight Policy Optimization and Deployment Qualification}
\label{sec:qualification}

We formulated EFE deployment qualification as a constrained
oversight-policy optimization problem in Section~\ref{sec:overview}.
We now develop the quantities and qualification procedures needed to solve
that problem.

The key distinction is between \emph{agent performance} and
\emph{deployed-system reliability}.
An oversight policy changes how agent work is combined with human review or
intervention.
Its value therefore depends not only on how often the agent succeeds, but
also on whether the available routing signals identify cases where human
oversight is most valuable, how effective that oversight is, and what it
costs.

We first develop the trajectory-invariant terminal accept-or-escalate case, for which many candidate policies can be evaluated from the same saved execution evidence.
We then return to the general trajectory-dependent setting, in which a candidate policy must be executed or simulated because intervention changes the trajectory itself.


% ------------------------------------------------------------------
\subsection{Qualification Quantities}
\label{sec:qualification-quantities}
% ------------------------------------------------------------------
For agent $m$, workflow $w$, and oversight policy $\pi$, let
$u^\pi \in \{0,1\}$ denote the workflow-specific success event defined in
Section~\ref{sec:overview-setting}. 
Thus, $u^\pi$ records whether an individual workflow execution under
policy $\pi$ satisfies the pre-specified success criterion.

% We define the reliability of the resulting human--AI system as

% \begin{equation}
% R_{m,w}(\pi)
% =
% \mathbb{E}\!\left[u^\pi\right],
% \label{eq:deployment-reliability}
% \end{equation}

% where the expectation is over task instances and any stochasticity in agent
% execution, the environment, and interacting actors.
% $R_{m,w}(\pi)$ is therefore the probability that an execution under policy
% $\pi$ satisfies the workflow-specific success criterion. Deployment qualification is an aggregate statistical claim about this
% reliability, not an outcome assigned to any individual task instance.

We define the reliability of the resulting human--AI system as
\begin{equation}
R_{m,w}(\pi)
=
\mathbb{E}_{x\sim \mathcal{D}_w}
\left[
u^\pi(x)
\right],
\label{eq:deployment-reliability}
\end{equation}
where \(u^\pi(x)\in\{0,1\}\) denotes whether execution on workflow instance
\(x\) satisfies the workflow-specific success criterion. The expectation is
over workflow instances \(x\) drawn from the population represented by
\(\mathcal{D}_w\) and, when execution is stochastic, over the induced randomness in
agent execution, the environment, oversight process, and interacting actors.
Since \(u^\pi(x)\) is binary, \(R_{m,w}(\pi)\) is the probability that an
execution under policy \(\pi\) satisfies the workflow-specific success
criterion on a randomly drawn workflow instance. Deployment qualification is
an aggregate statistical claim about this reliability, not an outcome
assigned to any individual task instance.

Let $K_w(Z^\pi)$ denote the operating cost incurred by a trajectory.
This may include agent execution as well as human review, approval, intervention or recovery. The expected operating cost is

\begin{equation}
C_{m,w}(\pi)
=
\mathbb{E}\!\left[K_w(Z^\pi)\right].
\label{eq:deployment-cost}
\end{equation}

Conceptually, this cost can be decomposed into agent and human components,

\begin{equation}
C_{m,w}(\pi)
=
C_{\mathrm{agent}}(m,w,\pi)
+
C_{\mathrm{human}}(m,w,\pi),
\label{eq:cost-decomposition}
\end{equation}


although both terms may depend on $\pi$.
For example, an intervention may increase human effort while shortening,
extending, or restarting the subsequent agent trajectory.

Equations~\ref{eq:deployment-reliability} and
\ref{eq:deployment-cost} provide the two canonical quantities used in the
optimization objective of Equation~\ref{eq:efe-overview-objective}.
They are properties of the deployed human--AI system under a specified
policy, not intrinsic properties of the agent alone.


% ------------------------------------------------------------------
\subsection{Terminal Accept-or-Escalate Oversight}
\label{sec:accept-escalate}
% ------------------------------------------------------------------

We first consider the trajectory-invariant setting illustrated by
CliniCARE-Bench.
In terminal accept-or-escalate oversight, the agent completes its work before
the routing decision is made.
At runtime, the completed execution provides the result and an observable
confidence or other routing signal $s_i$; the oversight policy then determines
whether the result is accepted autonomously or routed to human review.

To optimize and qualify such a policy, EFE first executes the agent on a
representative evaluation set under autonomous execution.
For each task instance $x_i$, this produces a saved trajectory $Z_i$ and
routing signal $s_i$.
The workflow evaluator then determines the corresponding autonomous-success
indicator

\begin{equation}
u_i \in \{0,1\}.
\end{equation}

Thus, $(Z_i,s_i,u_i)$ are evaluation data used for policy qualification;
at deployment time, the routing decision is made from observable information
such as $s_i$, while $u_i$ is generally unknown.

Because the terminal routing decision occurs only after $Z_i$ has been
generated, the trajectory is invariant to the candidate routing policy.
EFE can therefore evaluate many accept-or-escalate policies by replaying the
same saved evaluation runs rather than re-executing the agent for every
candidate policy.

For a scalar routing signal $s_i$, consider a threshold policy $\pi_\tau$
that accepts the completed result autonomously when $s_i \geq \tau$ and
routes it to human review otherwise.
We assume that larger values of $s_i$ indicate greater likelihood of
successful autonomous execution, so that $s_i$ provides a meaningful ordering
of cases for selective routing. The formal routing assumption is given in
Appendix~\ref{app:routing-monotonicity}.

% For a scalar routing signal, consider a threshold policy $\pi_\tau$ that
% accepts the completed result autonomously when

% \begin{equation}
% s_i \geq \tau
% \end{equation}

% and routes it to human review otherwise.
% The signal need not be a calibrated probability; for threshold-based routing,
% it need only provide a useful ordering of cases.

% Consider a threshold policy $\pi_\tau$ that accepts a completed result
% autonomously when

% \begin{equation}
% s_i \geq \tau
% \end{equation}

% and routes it to human review otherwise.
Its autonomous coverage is

\begin{equation}
c(\tau)
=
\Pr(s \geq \tau),
\label{eq:coverage}
\end{equation}

and its corresponding human-review rate is

\begin{equation}
e(\tau)
=
1-c(\tau).
\label{eq:review-rate}
\end{equation}

Coverage is useful in this terminal setting because it is simply the
complement of review burden; it is not required as a universal EFE
deployment metric.

Among autonomously accepted cases, define

\begin{equation}
a(\tau)
=
\Pr(u=1 \mid s\geq\tau),
\label{eq:selective-success}
\end{equation}

the success probability of work accepted without review.

Let $a_h(\tau)$ denote the probability that a case routed by policy
$\pi_\tau$ is successfully resolved by the declared human-review path.
The reliability of the deployed human--AI system is then

\begin{equation}
R(\tau)
=
c(\tau)a(\tau)
+
\bigl(1-c(\tau)\bigr)a_h(\tau).
\label{eq:terminal-reliability}
\end{equation}

The first term corresponds to work accepted autonomously; the second
corresponds to work routed to human review.

The review-path performance $a_h(\tau)$ can be either measured from the review process or introduced as a deployment
assumption.
It is important to note that because routing deliberately selects a non-random subset of cases,
$a_h(\tau)$ may vary with the policy.
When a constant review-success assumption $a_h$ is available,
Equation~\ref{eq:terminal-reliability} reduces to

\begin{equation}
R(\tau)
=
c(\tau)a(\tau)
+
\bigl(1-c(\tau)\bigr)a_h.
\label{eq:terminal-reliability-constant-review}
\end{equation}

This formulation makes clear why autonomous benchmark performance does not
determine deployment reliability.
Two agents with similar autonomous success rates may require very different
amounts of human review if their routing signals differ in their ability to
identify likely failures.


% ------------------------------------------------------------------
\subsection{Cost at a Target Reliability}
\label{sec:cost-reliable-deployment}
% ------------------------------------------------------------------

In terminal accept-or-escalate deployment, the agent has already executed
before the routing decision is made.
Let $k_m$ denote its expected execution cost per case and let $k_h$ denote
the incremental cost of the declared human-review path.
Under a constant-cost approximation,

\begin{equation}
C(\tau)
=
k_m
+
k_h\,e(\tau)
=
k_m
+
k_h\bigl(1-c(\tau)\bigr).
\label{eq:terminal-cost}
\end{equation}

For target reliability $Y$, qualification therefore selects

\begin{equation}
\tau^\star(Y)
=
\arg\min_{\tau}
C(\tau)
\qquad
\text{subject to}
\qquad
R(\tau)\geq Y,
\label{eq:threshold-optimization}
\end{equation}

together with any additional workflow-specific risk constraint.

When $k_m$ and $k_h>0$ are constant, minimizing operating cost is equivalent
to minimizing review burden, or equivalently maximizing autonomous coverage,
among policies that satisfy the reliability requirement.
Writing

\begin{equation}
e^\star(Y)
=
e\!\left(\tau^\star(Y)\right),
\end{equation}

the corresponding cost of reliable deployment is

\begin{equation}
C^\star(Y)
=
k_m+k_h e^\star(Y).
\label{eq:cost-of-reliable-deployment}
\end{equation}

This quantity provides a direct economic comparison between systems:
how much operating cost is required for each system to satisfy the same
workflow-specific reliability target.

The constant-cost model is useful for exposition but is not required by EFE.
Review effort may vary substantially across cases, and different policies may
trigger different forms of review, correction, or escalation.
When case-level costs are available, qualification estimates
$C(\pi)$ directly from the costs induced by the candidate policy rather than
assigning a single $k_h$ to every reviewed case.


% ------------------------------------------------------------------
\subsection{Quality of the Routing Signal}
\label{sec:routing-quality}
% ------------------------------------------------------------------

The value of terminal oversight depends on whether the routing signal
identifies cases for which autonomous execution is likely to fail.
A useful routing signal should therefore rank lower-success cases below
higher-success cases, so that increasing the acceptance threshold
preferentially removes higher-risk cases from autonomous handling.

A natural diagnostic is the selective-risk curve,
\begin{equation}
r(\tau)
=
\Pr(u=0 \mid s\geq\tau),
\label{eq:selective-risk}
\end{equation}
or equivalently $r(c)$ when operating points are indexed by autonomous
coverage. Sweeping the routing threshold traces the risk--coverage
relationship: a stronger routing signal achieves lower selective risk at the
same autonomous coverage.

We summarize this curve using the area under the risk--coverage curve,
\begin{equation}
\mathrm{AURC}
=
\int_0^1 r(c)\,dc,
\label{eq:aurc}
\end{equation}
with lower values indicating more effective selective routing. AURC captures
the average selective risk incurred across coverage levels and is therefore a
direct measure of the risk--coverage tradeoff induced by the routing signal.

% Because raw AURC depends not only on routing quality but also on the base
% autonomous success rate $a_0=\Pr(u=1)$, we also report a baseline-adjusted
% quantity, excess AURC:
% \begin{equation}
% \mathrm{E\text{-}AURC}
% =
% \mathrm{AURC}
% -
% \mathrm{AURC}_{\mathrm{oracle}}(a_0).
% \label{eq:eaurc}
% \end{equation}
% Here, $\mathrm{AURC}_{\mathrm{oracle}}(a_0)$ is the AURC achieved by an oracle
% routing signal that accepts all successful executions before any failed
% executions. For a base autonomous success rate $a_0$, this oracle value is
% \begin{equation}
% \mathrm{AURC}_{\mathrm{oracle}}(a_0)
% =
% 1-a_0+a_0\ln a_0.
% \label{eq:oracle-aurc}
% \end{equation}
% Thus, E-AURC measures the gap between the observed routing signal and the best
% possible ordering at the same base autonomous success rate. Lower E-AURC
% indicates routing behavior closer to the oracle.

Because AURC depends not only on routing quality but also on the base autonomous success rate $a_0=\Pr(u=1)$, we also report the AUROC of confidence against correctness, which measures only how well the reported confidence separates successful from unsuccessful executions. This gives a measure of routing quality that is independent of the base success rate.

For EFE, the practical value of the routing signal is ultimately determined
by the deployment policy it supports. At a fixed reliability target $Y$, better
routing reduces the human-review burden, and therefore the operating cost,
required to satisfy the reliability constraint. We therefore report AURC,
which reflects the absolute risk--coverage tradeoff, alongside AUROC, which
compares routing quality after accounting for differences in base autonomous
success rates.

% % ------------------------------------------------------------------
% \subsection{Statistical and Risk-Sensitive Qualification}
% \label{sec:statistical-qualification}
% % ------------------------------------------------------------------

% Policy optimization on an evaluation sample does not establish that the
% selected policy will satisfy its reliability target on future cases.
% EFE therefore separates \emph{policy selection} from
% \emph{policy qualification}.

% Parameters of the oversight policy---for example, the routing threshold
% $\tau$---are selected using development data.
% The resulting policy $\widehat{\pi}$ is then frozen and evaluated on a
% held-out qualification set.

% Let $R_{\mathrm{LCB}}(\widehat{\pi})$ denote a one-sided lower confidence
% bound on the reliability of the fixed policy.
% Qualification at target $Y$ requires

% \begin{equation}
% R_{\mathrm{LCB}}(\widehat{\pi})
% \geq Y.
% \label{eq:reliability-lcb}
% \end{equation}

% For independent binary outcomes, an appropriate binomial confidence interval
% may be used.
% For repeated runs, clustered task instances, or other structured evaluation
% designs, the uncertainty estimator must respect the corresponding sampling
% structure, for example through task-level bootstrap resampling.
% If the available sample cannot establish the required lower bound, the
% appropriate conclusion is insufficient evidence for qualification even when
% the observed point estimate exceeds $Y$.

% Reliability is the common EFE deployment constraint.
% Some workflows additionally require explicit control of failure severity.
% As introduced in Section~\ref{sec:overview-setting}, let

% \begin{equation}
% L_w(Z^\pi)\geq 0
% \end{equation}

% denote a workflow-specific deployment loss.
% Qualification may additionally require

% \begin{equation}
% \rho_w\!\left(L_w(Z^\pi)\right)
% \leq B_w,
% \label{eq:risk-qualification}
% \end{equation}

% where $\rho_w$ may, for example, be a chance constraint or a tail-risk
% functional such as conditional value-at-risk.
% Where this constraint is statistically estimated, qualification should
% similarly use an appropriate upper confidence bound on the relevant risk
% quantity rather than relying on its point estimate alone.

% The resulting qualification claim is necessarily conditional on both the
% evaluation population and the declared deployment assumptions.
% Material changes to the agent, workflow, evaluator, routing policy, review
% model, or represented task distribution may therefore require
% requalification.
% ------------------------------------------------------------------
\subsection{Statistical Qualification}
\label{sec:statistical-qualification}
% ------------------------------------------------------------------

Optimizing an oversight policy on an evaluation sample does not establish that
the selected policy will satisfy its reliability target on future cases.
EFE therefore separates \emph{policy selection} from
\emph{policy qualification}.

The evaluation sample $S_w$ is partitioned by disjoint index sets
$I_{\mathrm{dev}}, I_{\mathrm{qual}} \subseteq [N_w]$ into a development set
$S_{\mathrm{dev}} = \{x_i : i \in I_{\mathrm{dev}}\}$ and a held-out
qualification set $S_{\mathrm{qual}} = \{x_i : i \in I_{\mathrm{qual}}\}$.
All policy choices---including the routing rule and threshold---are made using
$S_{\mathrm{dev}}$.
The selected policy $\widehat{\pi}$ is then frozen before
$S_{\mathrm{qual}}$ is examined.

For terminal accept-or-escalate oversight, let
$\widehat{\tau}$ denote the threshold selected on the development set.
For each qualification case $i$, define

\begin{equation}
d_i
=
\mathbf{1}\{s_i \geq \widehat{\tau}\},
\label{eq:qualification-routing}
\end{equation}

where $d_i=1$ denotes autonomous acceptance and $d_i=0$ denotes human review.
The qualification set is therefore used only to estimate the operating
characteristics of this fixed routing policy, not to search for a better
threshold.


\paragraph{Measured human-review outcomes.}
When the outcome of the declared human-review path is observed for each
escalated case, let $h_i\in\{0,1\}$ denote whether that review path produces
a successful result.
The realized success of the deployed system on qualification case $i$ is

\begin{equation}
v_i
=
d_i u_i + (1-d_i)h_i,
\label{eq:qualification-case-success}
\end{equation}

and the empirical deployment reliability is

\begin{equation}
\widehat{R}(\widehat{\pi})
=
\frac{1}{N_{\mathrm{qual}}}
\sum_{i\in I_{\mathrm{qual}}} v_i,
\qquad
N_{\mathrm{qual}} = |I_{\mathrm{qual}}|.
\label{eq:qualification-reliability}
\end{equation}

In the terminal setting, $v_i$ is the realized policy-level success outcome
corresponding to the general success event $u_i^\pi$ in
Section~\ref{sec:qualification-quantities}; $u_i$ here denotes the success
of the autonomous execution before routing.

When every policy-level outcome is observed---including the outcome of each
executed human review---$v_i$ is a binary outcome and, for independent
qualification cases, a one-sided binomial lower confidence bound can be
computed directly.
At confidence level $1-\alpha$, EFE qualifies the policy only if

\begin{equation}
R_{\mathrm{LCB}}^{\,1-\alpha}(\widehat{\pi})
\geq Y.
\label{eq:reliability-lcb}
\end{equation}

Thus, a point estimate above the target is not sufficient: the held-out
evidence must be strong enough for the lower confidence bound itself to clear
the deployment requirement.


\paragraph{Human-review performance as a deployment assumption.}
In many evaluations, including retrospective benchmark analysis, the human
review path is not executed for every escalated case.
Instead, its success probability is supplied as a deployment assumption.
For a constant review-success assumption $a_h$, the qualification-set
reliability estimate becomes

\begin{equation}
\widehat{R}(\widehat{\pi};a_h)
=
\frac{1}{N_{\mathrm{qual}}}
\sum_{i\in I_{\mathrm{qual}}}
\left[
d_i u_i + (1-d_i)a_h
\right].
\label{eq:qualification-reliability-assumed-human}
\end{equation}

This quantity is no longer a simple binomial proportion, because reviewed
cases contribute an assumed success probability rather than an observed
binary outcome.
All statistical uncertainty is concentrated in the accepted cases.
Writing $n_{\mathrm{acc}}$ for the number of accepted qualification cases and
$\widehat{p}_{\mathrm{acc}}$ for the observed success rate among them, the
estimate decomposes as

\begin{equation}
\widehat{R}(\widehat{\pi};a_h)
=
\frac{n_{\mathrm{acc}}}{N_{\mathrm{qual}}}\,
\widehat{p}_{\mathrm{acc}}
+
\frac{N_{\mathrm{qual}}-n_{\mathrm{acc}}}{N_{\mathrm{qual}}}\,
a_h,
\label{eq:qualification-reliability-decomposition}
\end{equation}

in which only $\widehat{p}_{\mathrm{acc}}$ is estimated from observed
outcomes.
EFE therefore attaches statistical uncertainty only to the observed
component: a one-sided binomial lower confidence bound
$p_{\mathrm{acc,LCB}}^{\,1-\alpha}$ is computed from the
$n_{\mathrm{acc}}$ accepted cases, and the qualification criterion becomes

\begin{equation}
R_{\mathrm{LCB}}^{\,1-\alpha}(\widehat{\pi};a_h)
=
\frac{n_{\mathrm{acc}}}{N_{\mathrm{qual}}}\,
p_{\mathrm{acc,LCB}}^{\,1-\alpha}
+
\frac{N_{\mathrm{qual}}-n_{\mathrm{acc}}}{N_{\mathrm{qual}}}\,
a_h
\;\geq\;
Y.
\label{eq:reliability-lcb-assumed-human}
\end{equation}

No statistical confidence is attributed to the assumed term.
The resulting qualification statement is therefore explicitly conditional,
of the form ``qualified at target $Y$ under the declared review assumption
$a_h$.''
For policy families whose contributions do not admit this decomposition,
the same conditional bound is obtained by resampling qualification cases and
re-evaluating the fixed policy on each resample.
If $a_h$ is itself estimated from separate human-review data, uncertainty in
that estimate must also be propagated rather than treating $a_h$ as known
exactly; a conservative qualification replaces $a_h$ with a one-sided lower
confidence bound $a_{h,\mathrm{LCB}}$ in
Equation~\ref{eq:reliability-lcb-assumed-human}.

\paragraph{Break-even review assumption.}
Because $R_{\mathrm{LCB}}^{\,1-\alpha}(\widehat{\pi};a_h)$ is nondecreasing
in $a_h$, the dependence on the assumption can be summarized by a single
quantity: the weakest review assumption under which the policy still
qualifies,

\begin{equation}
a_h^{\min}(\widehat{\pi},Y)
=
\inf
\left\{
a_h\in[0,1]
:
R_{\mathrm{LCB}}^{\,1-\alpha}(\widehat{\pi};a_h)
\geq
Y
\right\}.
\label{eq:break-even-review-assumption}
\end{equation}

The deployment profile then states an auditable requirement on the human
process---the policy qualifies at target $Y$ provided the declared review
path succeeds at rate at least $a_h^{\min}$---rather than a conclusion
resting on an unexamined free parameter.
If no $a_h\in[0,1]$ satisfies the criterion, the policy is reported as not
qualified at target $Y$ under any review assumption.


\paragraph{Sampling unit.}
The resampling unit must match the unit that is intended to generalize.
If multiple stochastic runs are performed on the same task instance, those
runs are not treated as independent new cases.
EFE resamples at the task-instance level, carrying all repeated runs of an
instance together.
Analogously, if cases are naturally clustered by patient, customer, account,
or another sampling unit, qualification resamples at that cluster level.

A policy that fails the statistical criterion is reported as
\emph{not qualified at target $Y$} or \emph{insufficient evidence},
rather than being retuned on the qualification set.
Any change to $\widehat{\pi}$ after inspecting qualification results requires
a new held-out qualification evaluation.

% ------------------------------------------------------------------
\subsection{Risk-Sensitive Qualification}
\label{sec:risk-sensitive-qualification}
% ------------------------------------------------------------------

Reliability treats every unsuccessful execution as the same binary event.
For workflows in which failures differ materially in consequence, EFE may
add a workflow-specific loss

\begin{equation}
L_w(Z^\pi)\geq 0,
\end{equation}

and require

\begin{equation}
\rho_w\!\left(L_w(Z^\pi)\right)\leq B_w,
\label{eq:risk-qualification}
\end{equation}

where $B_w$ is the declared risk tolerance.
The risk functional $\rho_w$ is workflow-specific; examples include a bound
on the probability of a specified severe event or a tail-risk measure such
as conditional value-at-risk (CVaR).

This constraint is optional.
The common EFE qualification criterion remains reliability at minimum
operating cost; a separate risk constraint is introduced only when binary
success does not adequately represent the consequences of failure.

% ------------------------------------------------------------------
\subsection{Trajectory-Dependent Oversight}
\label{sec:trajectory-dependent-oversight}
% ------------------------------------------------------------------

The terminal formulation above is especially convenient because the routing
decision does not change the saved agent trajectory.
More general enterprise workflows allow intervention during execution.

Let $h_t$ denote the observable workflow history at decision point $t$, and
let

\begin{equation}
\pi(o_t\mid h_t)
\end{equation}

denote an oversight policy over intervention decisions $o_t$, such as
approval, correction or takeover.
Executing the workflow under $\pi$ induces a policy-dependent trajectory

\begin{equation}
Z_i^\pi
\sim
P(\,\cdot\mid m,x_i,E_w,\pi\,).
\label{eq:policy-dependent-trajectory}
\end{equation}

The qualification objective remains the one defined in
Equation~\ref{eq:efe-overview-objective}.
The difference is how the quantities in that objective are estimated.

For a trajectory-invariant terminal policy, candidate policies can be
evaluated by replaying the same saved trajectories under different routing
rules.
For a trajectory-dependent policy, changing $\pi$ changes what the agent,
oversight actor, or user subsequently observes and does.
Reliability, cost, and risk must therefore be estimated by executing or
simulating the candidate policy in the evaluation runtime.

Policy-in-the-loop evaluation may consequently change both sides of the
deployment tradeoff.
An intervention can improve the probability of successful completion, but
can also change agent execution length, human effort, recovery behavior, and
the distribution of subsequent outcomes.
These effects are captured by the same general quantities
$R_{m,w}(\pi)$, $C_{m,w}(\pi)$, and, when applicable,
$\rho_w(L_w(Z^\pi))$.

Thus, trajectory-invariant and trajectory-dependent workflows do not require
different deployment objectives.
They require different procedures for generating the evidence from which a
candidate oversight policy is optimized and qualified.

\paragraph{Empirical instantiation.}
Section~\ref{sec:empirical} applies the qualification methodology above to
CliniCARE-Bench.
The analysis is conducted on the benchmark's full four-way adjudication space
using a signal-based accept-or-escalate policy that is agnostic to the class
labels, with sensitivity analyses in
Appendix~\ref{app:clinicare-supplementary} and a cost-of-conflation control in
Appendix~\ref{app:conflation-control}.

% \subsection{Illustration with CliniCARE-Bench.}

% We use CliniCARE-Bench to illustrate how a routing signal is converted into
% an oversight policy and, ultimately, a qualified deployment operating point.
% The full benchmark uses a four-way adjudication space---\emph{Yes},
% \emph{No}, \emph{Indeterminate: Lack of Data}, and
% \emph{Indeterminate: Medically Ambiguous}.
% For clarity in the main-text analysis, we restrict the illustration to cases
% whose reference adjudication is definitive,

% \begin{equation}
% y_i^\star \in \{\mathrm{Yes},\mathrm{No}\}.
% \label{eq:clinicare-definitive-subset}
% \end{equation}

% We retain all agent predictions on these cases.
% In particular, if the agent returns either indeterminate verdict when the
% reference adjudication is definitive, the execution is counted as
% unsuccessful rather than removed from the analysis.
% For this illustration, define

% \begin{equation}
% u_i
% =
% \mathbf{1}\{\widehat{y}_i = y_i^\star\},
% \label{eq:clinicare-binary-success}
% \end{equation}

% and let $s_i$ denote the case-level confidence or other scalar routing signal
% associated with the agent's completed adjudication.
% Thus, the CliniCARE illustration reduces to the pair $(s_i,u_i)$ required by
% the terminal accept-or-escalate formulation above.

% % TODO(EFE/CliniCARE): report the number of definitive-reference cases
% % retained in this analysis and their Yes/No composition.
% % TODO(EFE/CliniCARE): confirm the exact semantics and range of the
% % case-level routing signal used for each evaluated system.

% Figure~\ref{fig:clinicare-routing} shows the resulting selective-routing
% behavior.
% Sweeping the threshold $\tau$ trades autonomous coverage against failure risk
% among autonomously accepted cases.

% % TODO(EFE/CliniCARE): insert empirical risk--coverage figure.
% % Recommended figure:
% %   Panel (a): selective risk r(c) versus autonomous coverage c
% %   for selected representative systems, with optional random/oracle
% %   reference curves.
% %
% % TODO(EFE/CliniCARE): report AURC and selective success at representative
% % coverage levels, e.g. c = 0.25, 0.50, 0.75.

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figures/clinicare_routing.pdf}
%     \fbox{
%         \parbox[c][1.55in][c]{0.92\linewidth}{
%         \centering
%         \textbf{TODO: CliniCARE selective-routing results}\\[4pt]
%         Panel (a): selective risk vs.\ autonomous coverage\\
%         Panel (b): human-review burden vs.\ target reliability
%         }}
%     \caption{
%     \textbf{Illustrative deployment qualification on definitive-reference
%     CliniCARE-Bench cases.}
%     Panel (a) evaluates whether the case-level routing signal concentrates
%     autonomous failures at lower scores.
%     Panel (b) translates this routing behavior into the human-review burden
%     required to satisfy increasing reliability targets.
%     The complete four-way analysis, including both valid indeterminate
%     outcomes, is reported in Appendix~\ref{app:clinicare-fourway-routing}.
%     }
%     \label{fig:clinicare-routing}
% \end{figure}

% To translate selective routing into deployment reliability, let $a_h$ denote
% the assumed probability that a case routed to the declared human-review path
% is successfully resolved.
% For each candidate threshold,

% \begin{equation}
% R(\tau;a_h)
% =
% c(\tau)a(\tau)
% +
% \left[1-c(\tau)\right]a_h.
% \label{eq:clinicare-reliability}
% \end{equation}

% For target reliability $Y$, the development data are used to select the
% highest-coverage threshold satisfying the reliability requirement,

% \begin{equation}
% \widehat{\tau}(Y)
% =
% \arg\max_{\tau} c(\tau)
% \qquad
% \text{subject to}
% \qquad
% R(\tau;a_h)\geq Y.
% \label{eq:clinicare-threshold-selection}
% \end{equation}

% The selected threshold is then frozen and evaluated on the held-out
% qualification set using the statistical procedure in
% Section~\ref{sec:statistical-qualification}.

% % TODO(EFE/CliniCARE): pre-specify the primary human-review assumption a_h.
% % Until a directly measured review-path estimate is available, report
% % sensitivity over a declared range rather than presenting a_h as measured.
% %
% % TODO(EFE/CliniCARE): report, for representative Y values:
% %   - selected threshold \hat{\tau}(Y)
% %   - held-out autonomous coverage
% %   - human-review burden
% %   - achieved reliability \hat{R}
% %   - one-sided reliability lower confidence bound
% %   - qualification pass/fail.
% %
% % TODO(EFE/CliniCARE): insert one concrete comparison between two systems
% % with similar autonomous success but materially different review burden
% % at the same reliability target.

% The purpose of this analysis is not to redefine CliniCARE-Bench as a binary
% benchmark, but to provide a transparent empirical instance of the EFE
% qualification machinery.
% The full CliniCARE task retains four-way adjudication, process-aware
% evaluation, and explicit abstention behavior; we analyze these additional
% structures in Appendix~\ref{app:clinicare-fourway-routing}.



==> old/overview_bk_0810.tex <==

% ==================================================================
\section{Enterprise's First Exam at a Glance}
\label{sec:overview}
% ==================================================================

\subsection{The EFE System}
\label{sec:overview-system}

Figure~\ref{fig:efe-overview} presents the overall EFE architecture. An
enterprise workflow is encoded through the EFE open standard, executed and
evaluated through the implemented platform, and translated through oversight
simulation into a deployment profile.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/EFE.png}
    \caption{
        \textbf{Enterprise's First Exam.}
        EFE converts an authentic enterprise workflow into a versioned
        deployment specification, executes agents in controlled environments,
        evaluates their outcomes and trajectories, simulates candidate
        oversight policies, and returns a deployment profile. \PSEBench{} and
        \CliniCARE{} are the first completed reference implementations. The
        open contribution program expands EFE across industries, workflows,
        environments, policies, assets, and evaluation methods.
    }
    \label{fig:efe-overview}
\end{figure}


\subsection{The Deployment Profile}
\label{sec:overview-profile}

A conventional benchmark commonly produces a task score or leaderboard
ranking. EFE produces a deployment profile specifying:

\begin{itemize}
    \item the hard-gate result;
    \item the qualified workflow scope;
    \item the agent's permitted authority;
    \item the actions that may be performed autonomously;
    \item the actions requiring approval or escalation;
    \item the achievable reliability and autonomous coverage;
    \item the residual risks and known limitations;
    \item the expected human-oversight and total operating cost.
\end{itemize}

The deployment profile answers the operational question:

\begin{quote}
\textbf{Where can the agent operate, under what authority and oversight,
with what residual risk, and at what total cost?}
\end{quote}


\subsection{Available at Launch}
\label{sec:overview-status}

\begin{table}[t]
    \centering
    \caption{EFE components available at launch.}
    \label{tab:launch-status}
    \begin{tabular}{
        >{\raggedright\arraybackslash}p{0.43\textwidth}
        >{\raggedright\arraybackslash}p{0.20\textwidth}
        >{\raggedright\arraybackslash}p{0.27\textwidth}
    }
        \toprule
        \textbf{Component} & \textbf{Status} & \textbf{Role} \\
        \midrule
        EFE open standard
        & Implemented
        & Defines EFE-compatible tasks and deployment contracts \\

        Evaluation platform
        & Implemented
        & Executes agents and records complete trajectories and state \\

        Evaluation engine
        & Implemented
        & Scores outcomes, processes, safety, and reliability \\

        Oversight simulator
        & Implemented
        & Evaluates autonomy, escalation, reliability, and cost policies \\

        Deployment-profile generator
        & Implemented
        & Produces qualified scope, authority, residual risk, and oversight \\

        \PSEBench{}
        & Completed
        & Seed benchmark and reference implementation \\

        \CliniCARE{}
        & Completed
        & Seed benchmark and reference implementation \\

        Open contribution program
        & Open
        & Expands domain, workflow, environment, and evaluation coverage \\
        \bottomrule
    \end{tabular}
\end{table}

==> old/overview_bk_0817.tex <==
% real workflow → deployment specification → controlled evaluation → oversight policy → deployment profile → expansion loop.

% ==================================================================
\section{Enterprise's First Exam at a Glance}
\label{sec:overview}
% ==================================================================

Enterprise deployment is not determined by model capability alone. The same
agent may be appropriate for one workflow but not another, or may be safe
only under a particular authority boundary and oversight policy. EFE
therefore evaluates the joint system

\begin{equation}
\text{Agent}
\times
\text{Workflow}
\times
\text{Deployment Policy}.
\end{equation}

Figure~\ref{fig:efe-overview} summarizes the resulting architecture. EFE
begins with an authentic enterprise workflow: who is responsible for the
work, what information and systems are available, which policies govern the
task, what actions may be taken, and how humans participate today. The EFE
open standard turns this workflow into an explicit deployment specification.
Agents are then evaluated against that specification in controlled
environments, with both their outcomes and the process by which they reach
those outcomes observed. Finally, EFE asks how the measured system could
actually be operated---what may be automated, what requires approval or
escalation, what reliability can be achieved, and what residual human effort
and cost remain.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/EFE.png}
\caption{
\textbf{Enterprise's First Exam.}
EFE begins with an authentic enterprise workflow and expresses it through an
open deployment standard covering autonomy surfaces, risk, authority, and
evaluation requirements. Agents are executed in controlled environments and
evaluated on outcomes, process, safety, and reliability. These measurements
are combined with candidate oversight policies to produce a deployment
profile describing the agent's qualified operating envelope. Seed benchmarks
such as \PSEBench{} and \CliniCARE{} instantiate the framework, while an open
contribution loop extends it to new workflows, environments, policies, and
evaluation methods.
}
\label{fig:efe-overview}
\end{figure}


\subsection{From Enterprise Workflow to Deployment Qualification}
\label{sec:overview-system}

The central design choice in EFE is to preserve the connection between an
evaluation task and the deployment setting it represents. A task is not
specified only by an instruction and a reference answer. It is situated
within an organizational role, information boundary, authority structure,
policy environment, consequence class, and human workflow.

The open standard captures this setting through four closely related
elements. \emph{Deployment tracks} describe the forms of autonomy exercised
by the workflow: evidence-grounded insight, state-changing action, and open
user interaction. Their associated \emph{risk surfaces} identify what can go
wrong. The \emph{deployment contract} specifies the agent's role, accessible
information and systems, permitted and prohibited actions, approval
boundaries, and escalation conditions. The \emph{evaluation profile} then
identifies the measurements and hard gates needed to judge the workflow.

This specification is deliberately independent of a particular model or
agent architecture. Different agents can therefore be evaluated against the
same workflow and authority boundary, and the same workflow specification
can be implemented on different compatible evaluation platforms.

Evaluation produces more than a final task score. EFE observes the work
product together with the evidence used, tool interactions, policy
application, approvals and escalations, and, for state-changing workflows,
the resulting enterprise state. These observations support distinct
measurements of outcome quality, process fidelity, safety, authority
compliance, reliability, and human-oversight requirements.

Deployment qualification then turns those measurements into an operating
policy. Non-negotiable safety and authority requirements are treated as hard
gates. For the remaining cases, EFE characterizes the tradeoff among
reliability, autonomous coverage, human intervention, and operating cost.
The objective is not to maximize autonomy, but to determine the scope of
autonomy that is justified by the evidence.


\subsection{The Deployment Profile}
\label{sec:overview-profile}

The primary output of EFE is therefore not a leaderboard position or a
context-free judgment that an agent is ``enterprise ready.'' It is a
\emph{deployment profile}: a bounded description of how the evaluated system
can be used.

A deployment profile specifies:

\begin{itemize}
    \item the workflow or workflow slices for which the evidence supports
    deployment;
    \item the authority granted to the agent;
    \item actions that may be performed autonomously and actions that require
    approval, clarification, or escalation;
    \item hard safety, policy, privacy, and authority constraints;
    \item achievable reliability and autonomous coverage;
    \item residual risks and known failure modes;
    \item required monitoring, review, and recovery mechanisms; and
    \item expected human-oversight and total operating cost.
\end{itemize}

The profile is conditional on the evaluated agent, workflow, environment,
policies, authority boundary, and deployment assumptions. It therefore
answers a more operational question than conventional benchmark accuracy:

\begin{quote}
\textbf{Where can this agent operate, under what authority and oversight,
with what residual risk, and at what total cost?}
\end{quote}

This framing also makes comparison among systems deployment-dependent.
A system with the highest average task score need not support the best
deployment policy: another system may separate reliable from unreliable
cases more effectively, remain within authority boundaries more consistently,
or require less human oversight to reach the same operating target.


\subsection{An Open and Extensible Evaluation Ecosystem}
\label{sec:overview-ecosystem}

No fixed benchmark can represent the full diversity of enterprise work.
EFE is therefore designed as an extensible evaluation ecosystem rather than
a closed collection of tasks.

The open standard provides the common representation through which new
workflows can enter the framework. Enterprises and domain experts can
contribute workflow definitions, policies, governed assets, task instances,
and reference work products; evaluation researchers can contribute new
graders, reliability measures, adversarial scenarios, and oversight methods.
Sensitive enterprise assets need not be made public: common task semantics
and evaluation methodology can coexist with gated, private, or server-side
execution.

\PSEBench{} and \CliniCARE{} illustrate this architecture for
evidence-grounded healthcare workflows. The broader purpose of EFE is to
support the same progression across industries and autonomy surfaces: from
research and decision support, to state-changing enterprise operations, to
open user-facing agents.

As this ecosystem grows, EFE is intended to provide a common language for
connecting three communities that are often separated: those who understand
the work, those who build and evaluate agents, and those responsible for
deploying them. The long-term goal is not a single universal exam, but a
shared framework through which increasingly capable agents can be evaluated
against the workflows, constraints, and operating policies under which
organizations actually intend to use them.

==> old/platform.tex <==

% ==================================================================
\section{The EFE Reference Evaluation Platform}
\label{sec:platform}

The EFE open standard specifies \emph{what} must be represented in an
enterprise-agent evaluation: the workflow, deployment tracks and risk
surfaces, authority boundary, consequence and reversibility, applicable
evaluation primitives, and deployment assumptions. The EFE reference
platform operationalizes that standard by turning a compatible
specification into reproducible agent executions, auditable trial records,
and ultimately a deployment profile.

Rather than introducing a new execution harness, EFE builds on the
Harbor evaluation framework and the executable-task design developed for
Terminal-Bench~\citep{harbor2026,merrill2026terminalbench}. Harbor provides
the underlying abstractions for tasks, datasets, agents, environments,
trials, verifiers, and jobs, together with containerized execution and
parallel evaluation. Terminal-Bench demonstrates how difficult agent tasks
can be packaged with controlled environments and executable verification.
Agents' Last Exam (ALE) provides a complementary reference design for
heterogeneous professional workflows, separating the task specification,
agent harness, and execution environment and evaluating the resulting
artifacts against hidden references or structured criteria
\citep{sun2026ale}.

EFE adds a layer that these execution frameworks do not attempt to provide:
an explicit enterprise deployment contract, governed information and action
boundaries, enterprise-state capture, policy and authority evaluation,
human-oversight simulation, and translation from benchmark measurements
into a conditional deployment qualification.

\subsection{Design Goals and Layering}
\label{sec:platform_goals}

The reference implementation follows four design principles.

\paragraph{Build on a reusable execution substrate.}
Environment provisioning, agent invocation, trial scheduling, resource
isolation, artifact collection, and low-level verifier execution are
delegated to Harbor wherever possible. EFE therefore does not require a
new agent harness or a new container runtime. A Harbor-compatible agent can
be evaluated without being rewritten specifically for EFE.

\paragraph{Keep the standard implementation-neutral.}
Harbor is the reference execution substrate, not part of the normative EFE
standard. The canonical EFE task and deployment specification is defined
independently of a particular execution engine. Other platforms may
implement the same specification provided that they preserve the required
environment, authority, logging, evaluation, and versioning semantics.

\paragraph{Evaluate the deployed system, not only the model.}
EFE qualification is conditional on the workflow and deployment policy.
The platform therefore records the model, agent harness, task specification,
environment version, policy corpus, authority configuration, grader
versions, and oversight assumptions associated with every evaluation run.
Changing any of these components may change the resulting deployment
profile.

\paragraph{Preserve enough evidence to re-audit and re-grade a run.}
Final task scores alone are insufficient for enterprise qualification.
EFE preserves the artifacts, relevant agent trajectory, environment events,
state transitions, policy decisions, and grader outputs required to
reconstruct the evaluation and, where possible, re-evaluate a completed
trial without rerunning the agent.

Conceptually, the platform evaluates

\begin{equation}
\mathcal{D}
\times
\mathcal{A}
\times
\mathcal{E}
\times
\Pi
\longrightarrow
\mathcal{T}
\longrightarrow
\mathcal{Q},
\label{eq:efe_platform}
\end{equation}

where $\mathcal{D}$ is an executable EFE deployment specification,
$\mathcal{A}$ is an agent configuration consisting of a harness and
foundation model, $\mathcal{E}$ is a governed execution environment,
$\Pi$ is the deployment or oversight policy under evaluation,
$\mathcal{T}$ is the resulting set of trial records, and
$\mathcal{Q}$ is the EFE deployment profile. This extends the familiar
task--agent--environment decomposition used in executable agent
benchmarks~\citep{merrill2026terminalbench,sun2026ale} with the deployment
policy and enterprise-governance semantics needed for qualification.

\subsection{Executable Task Packages and the Benchmark Registry}
\label{sec:platform_tasks}

The canonical EFE task record defined in Section~\ref{sec:standard}
is compiled into an executable task package. The package separates
agent-visible material from evaluator-only material and associates each
concrete task instance with the workflow template, deployment contract,
risk class, active evaluation primitives, environment version, and
reference artifacts that govern its evaluation.

This design builds directly on Harbor's task abstraction and the
Terminal-Bench convention of pairing an instruction and controlled
environment with executable verification
\citep{harbor2026,merrill2026terminalbench}. EFE augments that package with
enterprise-specific metadata rather than replacing the underlying task
format.

The task registry maintains four separately versioned objects:

\begin{enumerate}
    \item \textbf{workflow templates}, which describe reusable enterprise
    activities and their deployment semantics;
    \item \textbf{task instances}, which instantiate a template with
    concrete inputs, initial state, hidden references, and evaluation
    conditions;
    \item \textbf{benchmark releases}, which contain validated collections
    of templates and instances; and
    \item \textbf{evaluation configurations}, which bind a benchmark
    release to an agent, environment, policy corpus, graders, and
    deployment assumptions.
\end{enumerate}

This distinction is important for reproducibility. A change to a policy
document, an environment image, a grader, or the agent harness does not
silently overwrite an earlier result; it produces a new evaluation
configuration whose provenance remains attached to the resulting profile.

The registry also stores validation status and task lineage. Reference
solutions or expert work products may be used to verify task solvability
and grader correctness without being exposed to the evaluated agent.
Consistent with both Terminal-Bench and ALE, hidden evaluation material is
kept outside the agent-visible workspace
\citep{merrill2026terminalbench,sun2026ale}.

\subsection{Governed Environment Runtime and State Management}
\label{sec:platform_environment}

Harbor provides the base environment abstraction, including containerized
execution, resource constraints, network controls, multi-container tasks,
and isolated verifier environments~\citep{harbor2026}. EFE extends this
notion of an environment from a computational sandbox to a
\emph{governed enterprise environment}.

For an EFE task, the environment must reproduce not only the software
needed to complete the task but also the information and action boundary
of the organizational role being evaluated. At a high level, we represent
an environment as

\begin{equation}
\mathcal{E}
=
(S_0,\mathcal{O},\mathcal{A},\mathcal{P},\mathcal{H}),
\end{equation}

where $S_0$ is the reproducible initial enterprise state,
$\mathcal{O}$ is the observable information and tool surface,
$\mathcal{A}$ is the set of actions exposed by the environment,
$\mathcal{P}$ is the policy and authority enforcement layer, and
$\mathcal{H}$ is the human or user interaction channel when one is present.

Depending on the workflow, the environment may expose files, databases,
search indexes, internal APIs, enterprise applications, browser or GUI
interfaces, policy corpora, communication channels, or simulated users.
State-changing workflows may additionally contain systems of record,
transactional services, approval queues, or downstream services whose
state can be inspected after the run.

The environment enforces the deployment contract independently of the
agent's own instructions. In particular, EFE distinguishes actions that are
permitted autonomously, actions that require approval, and actions that are
prohibited. An agent claiming that an operation is permitted is not
sufficient evidence of authorization; the execution boundary records and,
where required, blocks the operation according to the task's declared
authority configuration.

For stateful tasks, the platform records a reproducible initial snapshot and
the resulting state transition. This enables evaluation of the enterprise
state itself rather than relying only on the agent's final natural-language
response. It also permits tests of duplicate execution, retries, stale
state, partial failure, rollback, and compensating actions.

Track-specific requirements emerge naturally from this common environment
model. Evidence-grounded workflows emphasize controlled information access
and provenance. State-changing workflows add mutable enterprise state and
authority enforcement. Open user-facing workflows additionally expose an
interaction channel through which a live or simulated user can supply new,
incomplete, contradictory, or adversarial information during execution.

\subsection{Agent Integration Layer}
\label{sec:platform_agents}

EFE does not prescribe the internal architecture of the evaluated agent.
The system under evaluation may use a proprietary or open-source harness,
arbitrary prompting and context-management strategies, native tools,
subagents, memory, browser or GUI control, shell execution, MCP services,
or other orchestration mechanisms.

This follows the modular agent interface used by Harbor, which supports
multiple integrated and externally supplied agent implementations
\citep{harbor2026}, and the separation in ALE between the agent
(harness plus foundation model) and the task/environment
\citep{sun2026ale}. The purpose of the EFE integration layer is therefore
not to translate every agent into a fixed vocabulary such as
\texttt{read\_file}, \texttt{search}, or \texttt{call\_tool}. Doing so
would alter the harness being evaluated and could erase meaningful
differences among agent systems.

Instead, EFE normalizes the \emph{evaluation boundary}. Each adapter must
support the lifecycle needed to configure and launch the agent, provide it
with the declared environment, terminate it under well-defined timeout and
resource conditions, identify the exact harness and model configuration,
and export the artifacts and execution telemetry required by the
evaluation.

Authority is enforced at the environment boundary rather than through an
EFE-specific agent API. Thus, two agents may interact with the same
enterprise workflow using different native tool systems while remaining
subject to the same data-access, action, approval, and logging constraints.

\subsection{Canonical Trial Record: Trajectories, Artifacts, and State}
\label{sec:platform_trial_record}

A Harbor \emph{trial} is one agent attempt on one task, while a job
collects multiple trials~\citep{harbor2026}. EFE retains these execution
semantics and augments the resulting record with the information needed for
enterprise audit and deployment qualification.

Each EFE trial record identifies at minimum:

\begin{itemize}
    \item the workflow template, task instance, and benchmark release;
    \item the model and agent-harness configuration;
    \item the environment and policy versions;
    \item agent-visible inputs and retrieved evidence;
    \item tool calls, environment observations, and material intermediate
    actions;
    \item intermediate and final work products;
    \item proposed and committed state-changing operations;
    \item protected environment events and before-and-after state;
    \item approval requests and approval outcomes;
    \item abstentions, clarifications, escalations, and their timing;
    \item resource use, latency, and model cost; and
    \item all verifier and grader outputs used to construct the final
    evaluation result.
\end{itemize}

Where the agent exposes a structured trajectory, EFE uses Harbor's Agent
Trajectory Interchange Format (ATIF) as the base representation rather than
introducing a competing agent-log format~\citep{harbor2026}. ATIF captures
messages, tool calls, observations, model and token metadata, costs, and
subagent structure. EFE associates this agent trajectory with additional
enterprise-side records that should not be controlled by the evaluated
agent, including system-of-record mutations, authorization decisions,
approval events, and trusted state snapshots.

This distinction between the \emph{agent trace} and the
\emph{environment record} is important. An agent-produced explanation of
what it did is not itself an audit trail. Deployment evaluation relies on
the externally recorded evidence of what the environment exposed, which
actions were attempted, which actions were committed, and how enterprise
state changed.

\subsection{Pluggable Verifiers and Evaluation Primitives}
\label{sec:platform_evaluation}

The evaluation engine maps the trial record onto the evaluation primitives
declared by the EFE task specification. Because enterprise work products
are heterogeneous, no single grader is appropriate for every task.

EFE follows a deterministic-first verification principle. Terminal-Bench
uses executable tests to determine whether the required terminal state has
been achieved~\citep{merrill2026terminalbench}. ALE similarly uses
artifact- and state-specific evaluators and deliberately prefers
deterministic verification when a checkable criterion can be constructed,
reserving model-based judgment for outputs that cannot credibly be reduced
to programmatic tests~\citep{sun2026ale}. EFE adopts the same principle.

The reference evaluator supports several composable verifier families:

\begin{enumerate}
    \item \textbf{Outcome and artifact verifiers} evaluate whether the
    required deliverable is correct and complete.
    
    \item \textbf{Final-state verifiers} inspect the resulting enterprise
    state, including records, transactions, submissions, and other
    state-changing effects.
    
    \item \textbf{Evidence-grounding verifiers} test whether consequential
    claims are supported by the evidence retrieved during the run and
    whether required provenance is present.
    
    \item \textbf{Policy and authority verifiers} evaluate whether the
    agent used the governing policy correctly and remained inside its
    granted role and action boundary.
    
    \item \textbf{Trajectory and process verifiers} inspect required or
    prohibited steps, approval behavior, escalation behavior, recovery
    behavior, and trace completeness.
    
    \item \textbf{Safety and interaction verifiers} evaluate privacy,
    adversarial robustness, policy compliance under pressure, unsafe
    actions, and other interaction-specific risks.
    
    \item \textbf{Expert or model-assisted evaluators} score criteria for
    which deterministic verification is not credible, using narrow,
    versioned rubrics and preserving the evaluated artifact and grader
    configuration for later audit.
\end{enumerate}

Evaluators may return continuous scores, categorical outcomes, structured
failure labels, or hard-gate violations. These signals remain separate in
the canonical record even when an aggregate benchmark score is also
reported. In particular, a high mean task score cannot compensate for a
violation of a non-negotiable authority, safety, privacy, or auditability
gate.

Verifier code and hidden references should, when necessary, execute in an
isolated evaluator context inaccessible to the agent. Harbor directly
supports separation between the agent environment and verifier environment,
including transfer of selected artifacts for grading~\citep{harbor2026}.
EFE uses this separation for confidential reference work products, hidden
policies, proprietary grading logic, and other evaluator-only assets.

Preserving artifacts separately from graders also permits
\emph{regrading}. If an evaluation rubric or deterministic verifier is
corrected, an existing artifact or state snapshot can be rescored when the
new grader does not require information that was absent from the original
trial. The new score is recorded under a new grader version rather than
silently replacing the historical result.

\subsection{Repeated Trials and Statistical Aggregation}
\label{sec:platform_reliability}

Enterprise qualification concerns a distribution of outcomes, not a single
successful rollout. The platform therefore supports repeated independent
trials of the same agent configuration on the same task instance as well
as evaluation over collections of instances. Harbor's trial and job
abstractions provide the underlying scheduling and parallel execution
mechanism~\citep{harbor2026}.

Repeated trials allow EFE to distinguish mean capability from operational
reliability. Depending on the task, aggregation may include success
probability, repeated-trial pass rates, variation in continuous outcome
quality, critical-failure frequency, escalation frequency, resource use,
and confidence intervals around deployment-relevant quantities.

Aggregation follows the hierarchy of the EFE standard. Trials are first
associated with task instances, instances with workflow templates, and
templates with benchmark releases and coverage metadata. The platform
therefore retains both aggregate results and the failure distribution by
workflow, risk surface, consequence class, and evaluation primitive.

This is especially important for qualification because rare critical
failures can be hidden by a high average score. Hard-gate failures and
consequence-weighted failure classes are therefore retained explicitly and
are not averaged away during benchmark aggregation.

\subsection{Oversight Simulation}
\label{sec:platform_oversight}

Raw benchmark performance does not by itself determine how an agent should
be deployed. EFE therefore places an oversight simulator above the
execution and evaluation layers.

The simulator combines trial-level measurements with candidate deployment
policies and operating assumptions. These may include confidence or
uncertainty signals, escalation decisions, approval requirements, human
review accuracy, reviewer time and cost, model cost, recovery cost, and
target reliability. For the one-shot accept-or-escalate setting of
Section~\ref{sec:qualification}, this reduces to evaluating the
reliability--autonomy frontier and selecting the minimum-cost policy that
satisfies the target reliability and all hard gates.

The stateful and interactive cases require a distinction between two forms
of oversight simulation.

\paragraph{Post-hoc policy replay.}
When the oversight decision changes only whether an existing result is
accepted or escalated, the platform can evaluate multiple policies from
the same set of saved trials. Confidence-threshold policies for
verdict-oriented evidence tasks are the canonical example.

\paragraph{Policy-in-the-loop evaluation.}
When an approval, clarification, intervention, or escalation changes what
the agent observes or what actions remain possible, the deployment policy
changes the trajectory itself. In this setting EFE executes the candidate
policy as part of the trial rather than assuming that the effect can be
reconstructed from a trajectory generated under another policy. Examples
include approval-before-commit workflows, recovery after failed writes,
and interactive tasks in which a human response changes subsequent agent
behavior.

This distinction prevents the oversight simulator from making unsupported
counterfactual claims from logged trajectories. Post-hoc simulation is
used where the required counterfactual is identifiable from the stored
record; otherwise qualification requires policy-in-the-loop trials.

The result is not necessarily a single globally optimal policy. The
simulator can expose a frontier over autonomous coverage, reliability,
critical risk, human-review burden, and operating cost, from which an
enterprise selects an operating point consistent with its deployment
requirements.

\subsection{Deployment-Profile Generation}
\label{sec:platform_profile}

The final stage converts evaluation results and oversight analysis into an
EFE deployment profile. The profile is conditional on the evaluated agent
configuration, workflow, environment, authority boundary, policy corpus,
benchmark release, reliability requirement, and operating assumptions.

For each qualified workflow or workflow slice, the profile reports:

\begin{itemize}
    \item hard-gate pass or fail status;
    \item the qualified workflow scope;
    \item the authority granted to the agent;
    \item actions permitted autonomously;
    \item actions requiring approval, clarification, or escalation;
    \item achievable reliability and autonomous coverage;
    \item residual risks and observed failure classes;
    \item required monitoring, audit, and recovery provisions; and
    \item expected human-oversight and total operating cost.
\end{itemize}

Thus the primary output of the platform is not a context-free claim that
an agent is ``enterprise ready.'' It is a bounded operating envelope:

\begin{quote}
\emph{Where can this agent operate, under what authority and oversight,
with what residual risk, and at what total cost?}
\end{quote}

A materially changed model, harness, environment, policy corpus, authority
configuration, or benchmark release may invalidate part of that envelope
and trigger requalification.

\subsection{Reference Implementation and Compatibility}
\label{sec:platform_compatibility}

EFE is designed as a qualification layer above existing agent-evaluation
infrastructure rather than as a replacement for it. In the reference
implementation, Harbor provides the execution substrate for provisioning
environments, integrating heterogeneous agents, running trials and jobs,
executing verifiers, and collecting artifacts and trajectories
\citep{harbor2026}. Terminal-Bench supplies an important reference for
self-contained, executable, verifiable task construction
\citep{merrill2026terminalbench}. ALE demonstrates how the separation among
task specification, agent harness, and environment extends to heterogeneous
professional software workflows and heterogeneous artifacts
\citep{sun2026ale}.

EFE adds the enterprise semantics above this substrate: deployment tracks
and risk surfaces, role and authority, governed assets, consequence and
reversibility, enterprise-state transitions, policy and process evaluation,
repeated-trial qualification, oversight economics, and deployment-profile
generation.

This layering is deliberate. Improvements in the underlying execution
infrastructure---new sandbox providers, agent integrations, trajectory
formats, or verifier mechanisms---can be adopted without changing the EFE
deployment standard. Conversely, an organization may implement the EFE
standard on a different execution substrate as long as it preserves the
specified task semantics, authority enforcement, evidence capture,
evaluation primitives, reproducibility, and deployment-profile outputs.
The open standard therefore defines interoperability at the
\emph{qualification} layer, while Harbor serves as the reference
implementation of the \emph{execution} layer.

==> old/platform_bk_0810.tex <==
\section{The Implemented EFE Platform - OLD}
\label{sec:platform}

\subsection{Platform Architecture and Implementation Status}
\label{sec:platform-architecture}

The implemented platform operationalizes the abstraction

\begin{equation}
    \text{Task Specification}
    \times
    \text{Agent Harness}
    \times
    \text{Environment}.
    \label{eq:platform-abstraction}
\end{equation}

% TODO:
% Insert the platform architecture figure.
%
% Suggested flow:
% Contributor portal
% -> task registry and review
% -> secure asset and policy vault
% -> environment orchestrator
% -> agent adapter
% -> trajectory, artifact, and state store
% -> evaluation engine
% -> oversight simulator
% -> deployment-profile generator.


\subsection{Task Registry}
\label{sec:platform-registry}

The task registry stores versioned workflow templates, task instances,
policies, reference artifacts, evaluation rubrics, benchmark releases, and
validation status.


\subsection{Secure Asset and Policy Vault}
\label{sec:platform-vault}

The vault manages enterprise data, policy documents, hidden references, and
other governed assets. It supports public, gated, private, and server-side
evaluation modes.


\subsection{Environment Orchestration}
\label{sec:platform-environments}

The environment orchestrator creates a reproducible initial state, exposes
approved tools and data, records changes, isolates concurrent runs, and
resets state between repeated trials.


\subsection{Normalized Agent Adapters}
\label{sec:platform-adapters}

The platform exposes capability-oriented operations rather than prescribing
an agent architecture. Supported operations may include:

\begin{itemize}
    \item \texttt{observe};
    \item \texttt{read\_file};
    \item \texttt{search};
    \item \texttt{query\_database};
    \item \texttt{call\_tool};
    \item \texttt{propose\_write};
    \item \texttt{commit\_write};
    \item \texttt{ask\_user};
    \item \texttt{escalate};
    \item \texttt{finish}.
\end{itemize}


\subsection{Trajectory, Artifact, and State Store}
\label{sec:platform-store}

The platform records immutable:

\begin{itemize}
    \item retrieved sources;
    \item evidence-to-claim mappings;
    \item tool calls and tool outputs;
    \item intermediate and final artifacts;
    \item proposed and committed writes;
    \item before-and-after state;
    \item approval requests;
    \item escalations and escalation rationales.
\end{itemize}


\subsection{Evaluation Engine}
\label{sec:platform-evaluation}

The evaluation engine supports:

\begin{itemize}
    \item deterministic outcome grading;
    \item structured policy and authority checks;
    \item evidence-grounding evaluation;
    \item rubric-based expert or model-assisted grading;
    \item final-state inspection;
    \item trajectory and process evaluation;
    \item repeated-trial aggregation;
    \item human-review effort estimation.
\end{itemize}


\subsection{Oversight Simulator}
\label{sec:platform-simulator}

The oversight simulator evaluates candidate autonomy, approval, and
escalation policies under different reliability targets, human-review
accuracies, and operating costs.


\subsection{Deployment-Profile Generator}
\label{sec:platform-generator}

The deployment-profile generator converts benchmark results, hard-gate
outcomes, and oversight simulations into an operational deployment envelope.

% TODO:
% Insert one complete example profile produced by the implemented platform.


\subsection{Implementation-Status Summary}
\label{sec:platform-status}

\begin{table}[t]
    \centering
    \caption{Implementation status of the EFE platform.}
    \label{tab:implementation-status}
    \begin{tabular}{
        >{\raggedright\arraybackslash}p{0.34\textwidth}
        >{\raggedright\arraybackslash}p{0.18\textwidth}
        >{\raggedright\arraybackslash}p{0.38\textwidth}
    }
        \toprule
        \textbf{Platform component}
        & \textbf{Status}
        & \textbf{Current capability} \\
        \midrule
        Task registry
        & Implemented
        & Versioned templates, instances, policies, and references \\

        Secure asset and policy vault
        & Implemented
        & Controlled access to governed inputs and policy corpora \\

        Environment orchestration
        & Implemented
        & Controlled execution and repeatable task initialization \\

        Agent adapters
        & Implemented
        & Normalized execution across supported agent systems \\

        Trajectory and state store
        & Implemented
        & Immutable evidence, action, artifact, and state capture \\

        Evaluation engine
        & Implemented
        & Outcome, process, grounding, safety, and reliability grading \\

        Oversight simulator
        & Implemented
        & Reliability, autonomy, escalation, and cost analysis \\

        Deployment-profile generator
        & Implemented
        & Conditional deployment qualification and residual-risk reporting \\
        \bottomrule
    \end{tabular}
\end{table}


==> old/reference_bench.tex <==
% ==================================================================
\section{Seed Benchmarks and Reference Implementations}
\label{sec:seed-benchmarks}
% ==================================================================

We instantiate EFE on two completed healthcare benchmarks,
\PSEBench{}~\citep{han2026psebench} and
\CliniCARE{}~\citep{chatrath2026clinicare}. The purpose of this section is
not to reproduce the benchmark papers, but to show how independently
developed evaluations can be represented through the EFE standard,
executed as governed agent workflows, and translated into
deployment-relevant measurements.

The two benchmarks provide complementary reference implementations.
\PSEBench{} evaluates policy-grounded patient-safety-event triage in a
controlled environment with by-construction ground truth, including cases
that require active information seeking or escalation because the governing
policy remains ambiguous. \CliniCARE{} evaluates retrospective clinical
audit over real-patient-derived longitudinal EHR data, where agents must
retrieve heterogeneous evidence, apply governing standards, produce cited
adjudications, and expose a replayable investigation trace. Both are
evidence-grounded workflows, but they stress different parts of the EFE
evaluation surface.

% ==================================================================
\subsection{\PSEBench}
\label{sec:psebench}
% ==================================================================

\subsubsection{Enterprise Workflow and Deployment Question}
\label{sec:pse-workflow}

\PSEBench{} evaluates patient-safety event triage: determining whether a
reported clinical event is reportable under a jurisdiction-specific
patient-safety policy~\citep{han2026psebench}. The benchmark is instantiated
on Minnesota's 29 Reportable Adverse Health Events (MN29) framework.
Operationally, a patient-safety reviewer receives an event narrative,
consults the governing statute and guidance, determines whether
decision-critical information is missing, and returns a reportability
assessment with its legal basis.

The workflow is naturally human-supervised. The evaluated agent does not
file a regulatory report or modify a clinical record. Its role is to produce
a policy-grounded triage recommendation for a patient-safety professional
who remains responsible for the consequential organizational decision.

The corresponding EFE deployment question is therefore:

\begin{quote}
\textbf{For which patient-safety events can the agent produce a sufficiently
accurate, policy-grounded triage recommendation autonomously, and which
events must be escalated for additional information or expert review?}
\end{quote}

This distinction is important because a system may correctly identify many
reportable events while still be unsuitable for deployment if it commits
when required information is missing, fails to recognize regulatory
ambiguity, or cannot substantiate its decision from the governing policy.

\subsubsection{Mapping to the EFE Standard}
\label{sec:pse-standard}

Under the EFE standard, \PSEBench{} is primarily a
\textbf{Track~1: evidence-grounded insight} workflow. Its interaction with
the benchmark's information provider is an evidence-acquisition interface,
not an open user-facing workflow, and the evaluated agent does not change
persistent enterprise state.

The primary risk surface is therefore \textbf{evidence and reasoning risk}.
The deployment contract can be summarized as follows:

\begin{itemize}
    \item \textbf{Role:} patient-safety event triage reviewer or assistant;
    \item \textbf{Intended user:} patient-safety expert or quality manager;
    \item \textbf{Information access:} the event narrative, MN29 statute and
    official guidance, and case-specific facts made available through the
    governed information interface;
    \item \textbf{Autonomous actions:} inspect evidence, consult policy,
    request missing factual information, and draft a triage recommendation;
    \item \textbf{Prohibited actions:} amend the clinical record, file the
    regulatory report, or otherwise commit the downstream organizational
    action;
    \item \textbf{Expected work product:} a structured verdict
    (\emph{Reportable}, \emph{Non-Reportable}, or \emph{Uncertain}),
    the applicable clause, governing legal evidence, and rationale;
    \item \textbf{Escalation conditions:} unresolved decision-critical
    information or irreducible policy silence, contradiction, or ambiguity.
\end{itemize}

Because the work product can influence a consequential reporting decision
but remains subject to human action, we treat the benchmark as an
illustrative \textbf{R1} workflow under the consequence classification of
Section~\ref{sec:standard-risk}.

The principal EFE evaluation primitives exercised by \PSEBench{} are
outcome correctness, evidence and policy grounding, abstention and
escalation, auditability of the information-seeking trajectory, and
human-review and oversight cost. The benchmark's native metrics instantiate
these primitives through verdict accuracy, clause accuracy, legal-evidence
citation, boundary-condition coverage, missing-information detection,
targeted information seeking, and uncertainty detection.

\subsubsection{Benchmark Construction and Validation}
\label{sec:pse-construction}

The full construction methodology is described in
\citet{han2026psebench}; we summarize only the elements relevant to EFE
conformance.

\PSEBench{} represents regulatory decision logic through human-audited
\emph{clause cards}. Each card factorizes a portion of the MN29 policy into
an event type, boundary conditions, factual event elements, governing legal
basis, intended verdict, and instantiation constraints. The released
specification contains 146 complete-case cards, 66 missing-information
variants, and 11 uncertain cards.

Cases are generated in two verified stages. Structured event facts are first
instantiated under the clause-card constraints. A narrative is then produced
from those facts, and a second verifier checks that the narrative preserves
the decision-critical information without introducing facts that would
change the intended legal classification. Missing-information variants
systematically withhold identified decision-critical fields, while uncertain
variants represent cases in which the facts are complete but the governing
policy remains irreducibly ambiguous.

The resulting benchmark contains 5,074 cases: 3,455 complete cases,
1,362 missing-information cases, and 257 uncertain cases. Each case retains
structured ground truth for the verdict, event type, governing legal basis,
decision boundary conditions, and, for missing-information cases, the
withheld factual fields.

Two patient-safety experts additionally reviewed a stratified sample of
90 generated cases. They agreed with the constructed ground truth on
28/30 complete-case verdicts, 29/30 missing-case indeterminacies, and
30/30 uncertain-case ambiguities, while rating the narratives highly for
clinical realism. This validation complements the benchmark's
by-construction verification rather than replacing it.

\subsubsection{Evaluation Protocol and Baseline Systems}
\label{sec:pse-protocol}

The evaluated agent is placed in a two-role environment. It receives the
event narrative and governing policy and may either issue an \texttt{ASK}
action for a specific missing fact or terminate with an \texttt{ANSWER}.
The information provider is a stateless, controlled fact interface whose
responses are constrained to the structured ground truth associated with
the case. The agent controls whether to ask, what to ask, and when to stop,
subject to a maximum of ten interaction turns. The full question--answer
trajectory and final structured response are retained for evaluation.

The benchmark evaluates 15 models spanning closed-source frontier,
open-weight frontier, smaller general-purpose, and medical-specialty
families. The information-provider model and LLM-based grader are held fixed
across evaluated systems so that observed differences reflect the evaluated
agent rather than changes in the environment or grader. Full model
configurations, prompts, and metric definitions are reported in the
\PSEBench{} paper.

For EFE, we treat the benchmark's measured verdict, grounding,
information-seeking, and uncertainty metrics as the primary observations.
Any mapping from these measurements to human-review cost is performed by
the EFE oversight model and is reported separately below.

\subsubsection{Benchmark Results}
\label{sec:pse-results}

The main deployment-relevant finding is that \textbf{verdict accuracy does
not determine triage readiness}. The strongest systems achieve over 90\%
overall verdict accuracy, but their behavior diverges substantially on
grounding, information seeking, and escalation.

For example, GPT-5.5 and GPT-5 achieve 94.6\% and 90.2\% verdict accuracy,
respectively, while their uncertainty-detection F1 scores differ much more
sharply, 79.7\% versus 12.8\%. Gemini~3.1~Pro reaches 95.3\% verdict
accuracy and 74.0\% uncertainty-detection F1. Across the broader model set,
uncertainty detection is the most polarized capability: many systems that
perform reasonably on complete cases rarely return \emph{Uncertain} on
irreducible policy gray zones.

Performance also deteriorates as the workflow requires more than static
classification. The strongest systems remain highly accurate on complete
cases but decline on missing-information and uncertain cases. Several
systems either commit without requesting decision-critical facts or ask
questions that do not target the withheld information. Evidence-grounding
scores likewise trail headline verdict accuracy, showing that a correct
classification does not necessarily imply a policy-faithful or auditable
decision.

From the EFE perspective, these are distinct deployment failures:
\emph{wrong outcome}, \emph{unsupported decision}, \emph{failure to gather
necessary information}, and \emph{failure to escalate}. Reporting them
separately is therefore more informative than reducing the benchmark to a
single leaderboard score.

\subsubsection{Oversight Economics}
\label{sec:pse-economics}

\PSEBench{} also provides a controlled illustration of the EFE
reliability--autonomy formulation in Section~\ref{sec:qualification}.
The benchmark directly measures base verdict performance and whether
systems recognize cases designed to require escalation. EFE uses these
measurements to ask how much human review would be required to attain a
specified system-level reliability.

It is important to distinguish the quantities involved. Verdict accuracy
and uncertainty-detection performance are \emph{measured benchmark
quantities}. Human-review accuracy, reviewer cost, and model inference cost
are \emph{deployment assumptions}. The resulting escalation rate and
cost-of-reliability curve are therefore \emph{modeled EFE outputs}, not
direct measurements made by \PSEBench{}.

For the illustrative analysis in Section~\ref{sec:cost-reliability}, we use
human-review accuracy $a_h=0.99$ and human-review cost
$k_h=\$25$ per escalated case. Because \PSEBench{} does not natively provide
a calibrated scalar confidence for every case, its uncertainty-detection
score is used only as a proxy for the quality with which a system separates
cases that should be deferred. The resulting economic analysis should
therefore be interpreted as an illustration of the EFE mapping rather than
as a production cost estimate.

The qualitative result is robust to the particular dollar assumption:
systems with similar inference cost can require very different amounts of
human review when their escalation behavior differs. As the target
reliability approaches the assumed human-review ceiling, the required
coverage by human reviewers rises sharply. Thus, for this workflow,
improving the ability to identify cases requiring review can matter more to
deployment economics than reducing token cost.

\subsubsection{Representative Deployment Profiles}
\label{sec:pse-profiles}

A representative EFE deployment profile for \PSEBench{} does not grant
unrestricted autonomous reporting authority. The qualified action is the
production of a triage recommendation.

For a strong system, the profile may permit autonomous preparation of
recommendations on well-supported cases while requiring escalation when
decision-critical facts remain unresolved, when the policy is ambiguous, or
when the agent cannot ground its conclusion in the governing clause. Systems
with weak information-seeking or uncertainty-detection behavior require a
broader review policy even when their aggregate verdict accuracy is high.

The benchmark therefore demonstrates the central EFE distinction between
\emph{capability} and \emph{deployable scope}: high classification accuracy
can qualify an agent to assist the workflow without qualifying it to resolve
every case autonomously.


% ==================================================================
\subsection{\CliniCARE: Seed Benchmark and Reference Implementation}
\label{sec:clinicare}
% ==================================================================

\subsubsection{Enterprise Workflow and Deployment Question}
\label{sec:clinicare-workflow}

\CliniCARE{} evaluates evidence-grounded retrospective clinical audit over
longitudinal patient records~\citep{chatrath2026clinicare}. These workflows
ask questions such as whether a protocol was followed, whether a clinical
event occurred within a specified interval, or whether the available record
supports a quality or operational conclusion.

The agent is not given a preassembled case summary. It must determine what
evidence is needed, retrieve it across heterogeneous structured records and
free-text notes, reconstruct the relevant timeline, perform explicit
computations where necessary, identify and apply the governing clinical or
operational standard, and produce a cited adjudication.

The corresponding EFE deployment question is:

\begin{quote}
\textbf{Which retrospective clinical-review cases can an agent adjudicate
with a sufficiently correct, grounded, policy-compliant, and auditable
investigation, and which cases require human review?}
\end{quote}

The unit of evaluation is therefore not medical knowledge in isolation, but
the defensibility of the full evidence-acquisition and adjudication process.

\subsubsection{Mapping to the EFE Standard}
\label{sec:clinicare-standard}

\CliniCARE{} is also primarily a
\textbf{Track~1: evidence-grounded insight} workflow, with
\textbf{evidence and reasoning risk} as its primary risk surface.

Its EFE deployment contract is:

\begin{itemize}
    \item \textbf{Role:} retrospective clinical audit or quality reviewer;
    \item \textbf{Intended user:} a clinical quality, safety, or operational
    reviewer;
    \item \textbf{Information access:} a patient-scoped longitudinal EHR,
    governed clinical tools, a sandbox for explicit computation, and a
    fixed policy corpus;
    \item \textbf{Autonomous actions:} retrieve records, construct a
    timeline, compute derived quantities, retrieve governing policy, and
    draft a cited adjudication;
    \item \textbf{Prohibited actions:} modify the patient record, initiate
    treatment, contact the patient, or otherwise take prospective clinical
    action;
    \item \textbf{Expected work product:} a cited report with one of four
    verdicts---\emph{Yes}, \emph{No}, \emph{Indeterminate: Lack of Data},
    or \emph{Indeterminate: Medically Ambiguous};
    \item \textbf{Escalation conditions:} insufficient evidence to resolve
    the question or residual medical ambiguity after the relevant evidence
    has been reviewed.
\end{itemize}

As with \PSEBench{}, this is an illustrative \textbf{R1} deployment because
the agent produces decision support rather than committing a clinical or
administrative action.

\CliniCARE{} exercises a broader set of Track~1 EFE primitives:
outcome correctness, patient-evidence grounding, policy grounding,
calibrated abstention, auditability, process adherence, repeated-trial
reliability, human-review effort, and resource and operating cost.

\subsubsection{Benchmark Construction and Validation}
\label{sec:clinicare-construction}

The complete construction protocol is given in
\citet{chatrath2026clinicare}. \CliniCARE{} contains 25 clinician-developed
and validated scenarios spanning 14 medical specialties and ten recurring
reasoning capabilities. Each scenario specifies a natural-language clinical
query, operational four-way adjudication criteria, required evidence and
grounding, governing documents where applicable, and a process rubric.

Each scenario is instantiated on 30 patient records, yielding 750 cases over
MIMIC-IV, MIMIC-IV-Note, and MIMIC-IV-ED. Cases are deliberately sampled
across definitive and indeterminate regimes to exercise missing evidence,
conflicting documentation, temporal ambiguity, and other difficult audit
conditions; the resulting distribution is an evaluation distribution rather
than an estimate of clinical prevalence.

Reference verdicts are constructed through independent adjudication by
three frontier model--harness configurations operating with the complete
scenario specification. The three systems agree unanimously on 556 cases,
split 2--1 on 183, and produce three distinct verdicts on 11; the latter are
sent for direct clinical adjudication.

Clinical review is used both to validate the scenario specifications and to
calibrate the reference-label procedure. Two clinicians independently vet
every scenario. On a separate 75-case verdict-calibration sample, the
reference verdict agrees with the clinician verdict on 64 of 70 cases with
a defined label, or 91\% agreement ($\kappa=0.87$); agreement is perfect on
the unanimous-ensemble subset and lower on non-unanimous cases. A
double-reviewed subset further shows that the difficult cases are also those
on which independent clinical judgment is less reproducible. These
measurements support the reference-labeling protocol while also defining its
limitations; the full 750 cases were not exhaustively independently
adjudicated by clinicians.

\subsubsection{Evaluation Protocol and Baseline Systems}
\label{sec:clinicare-protocol}

Agents interact with the longitudinal record through a governed,
patient-scoped tool layer rather than unrestricted access to the underlying
database. The primary environment exposes clinically meaningful retrieval
operations over encounters, notes, laboratory values, vital signs,
medications, microbiology, procedures, imaging, and orders. A capped,
read-only SQL fallback covers gaps in the higher-level tools; a sandbox
supports explicit computation; and policy-document tools expose a fixed
corpus with document- and line-level provenance. Every retrieval,
computation, and policy access is logged.

The main evaluation contains sixteen complete system configurations:
production Claude Code, Codex, and Gemini CLI systems on their native model
families, together with six open-weight models evaluated through the
model-agnostic opencode harness. Web search and external fetch are disabled,
so all systems operate only on the governed patient record and policy corpus.
Each system is evaluated once on each of the 750 cases for the primary
leaderboard.

A frozen 148-case development subset is used separately for paired
ablations and repeated-run reliability experiments. Selected systems are
executed independently three times on this subset to measure avg@$k$,
pass$^k$, pass@$k$, verdict agreement, and stable wrong answers. The
development subset is not used to rank systems because it deliberately
oversamples the two indeterminate classes.

Every parseable report also includes a stated confidence, allowing EFE to
evaluate calibration and selective autonomy. Resource measurements include
turns, tool calls, token use, and execution cost, with accounting differences
across harness families retained rather than treated as perfectly
comparable.

\subsubsection{Outcome, Grounding, Process, and Abstention Results}
\label{sec:clinicare-results}

The sixteen systems achieve four-way verdict accuracies between 65.3\% and
76.1\%, with macro-F1 between 0.555 and 0.701. More importantly for EFE,
the additional evaluation primitives reveal differences that aggregate
accuracy obscures.

\paragraph{Outcome versus process.}
Defect-free accuracy credits a correct verdict only when the observable
investigation also avoids all scenario-specific prohibited shortcuts.
Across the sixteen systems it falls 4.8--14.8 percentage points below raw
report-present accuracy and changes the system ordering. Process-adherence
scores similarly separate systems with comparable final-verdict
performance. A correct outcome is therefore not sufficient evidence of a
defensible clinical investigation.

\paragraph{Abstention.}
All sixteen systems under-abstain. On cases whose reference verdict requires
deferral, over-commitment ranges from 21.3\% to 55.3\%, whereas
over-abstention on reference-definitive cases ranges from 7.3\% to 16.5\%.
The dominant failure is therefore committing to an answer when the record
does not support one, rather than excessive caution.

\paragraph{Patient-evidence grounding.}
Record-level citation validity is high, but substantive support and evidence
coverage vary materially. Record-identifier precision lies between 0.985 and
1.000, while claim-level support and required-evidence coverage remain
lower and vary across harnesses. In particular, retrieving a source does not
guarantee that the final report establishes the required finding, reinforcing
the EFE distinction between tool activity and grounded completion.

\paragraph{Policy grounding.}
Systems generally cite real and relevant governing policy documents but do
so incompletely. Policy-citation resolution ranges from 0.954 to 1.000 and
document precision from 0.764 to 0.899, while governing-document recall
ranges from 0.407 to 0.703. Thus a report may cite a valid applicable
standard while omitting other standards necessary for a complete
adjudication.

\paragraph{Repeated-run reliability.}
On the three-attempt development experiment, pass$^3$ falls
8.3--12.6 points below avg@3 across the evaluated systems. Much of the
remaining agreement is agreement on the same incorrect verdict rather than
random run-to-run variation. Repetition alone therefore does not make a
system reliable: some errors are stable.

Together these results show why EFE preserves outcome, grounding, process,
abstention, and repeated-trial reliability as separate primitives rather than
collapsing them into one clinical-agent score.

\subsubsection{Reliability--Autonomy and Oversight Analysis}
\label{sec:clinicare-economics}

Unlike \PSEBench{}, \CliniCARE{} obtains an explicit per-case confidence
from each system. This allows the EFE oversight analysis to use the
measured ordering of cases directly rather than substituting an aggregate
uncertainty metric.

For each system, cases are ranked by stated confidence and the autonomy
threshold is swept from selective handling of the highest-confidence cases
to full autonomy. This produces the risk--autonomy curve defined in
Section~\ref{sec:qualification}. The curve answers a deployment question
that full-cohort accuracy cannot: whether the system knows sufficiently well
\emph{which} cases it is likely to resolve correctly.

The benchmark's calibration results already show that this property is
distinct from accuracy. Expected calibration error ranges from 0.046 to
0.262 across the sixteen systems and orders systems differently from
four-way accuracy. The final EFE cost-of-reliability analysis should
therefore be computed from the case-level confidence and correctness records,
using the deployment assumptions specified in
Section~\ref{sec:cost-reliability}, rather than inferred from aggregate
accuracy.

As with \PSEBench{}, the distinction between observation and assumption is
explicit: verdicts, confidence, traces, and resource use are measured;
human-review accuracy and cost are deployment assumptions; reliability,
autonomous coverage, and oversight-adjusted cost are derived quantities.
This keeps the deployment profile auditable and allows the same benchmark
results to be reevaluated under a different enterprise cost or reliability
target.

\subsubsection{Representative Deployment Profiles}
\label{sec:clinicare-profiles}

The current results do not support a context-free claim that any evaluated
system can autonomously perform retrospective clinical audit. Even the
strongest full-cohort system resolves only about three quarters of cases
correctly, every evaluated system over-commits on cases requiring
abstention, and correct verdicts can contain process defects.

A representative EFE deployment profile would therefore qualify
\CliniCARE{} systems for a bounded \emph{draft-for-review} role rather than
unrestricted autonomous adjudication. The agent may retrieve the record,
construct the evidence trail, apply governing standards, and prepare a
reviewable conclusion. Autonomous acceptance can then be restricted to
workflow slices and confidence regions that satisfy the chosen reliability
and hard-gate requirements, while cases with missing evidence, residual
medical ambiguity, process defects, or insufficient grounding remain
human-reviewed.

The appropriate boundary is system- and target-dependent. A system with
slightly lower aggregate accuracy can support a better operating policy if
its confidence more effectively separates reliable from unreliable cases or
if its investigation is more grounded and auditable. The deployment profile
therefore retains these dimensions rather than selecting the system from
accuracy alone.


% ==================================================================
\subsection{What the Two Seed Benchmarks Demonstrate}
\label{sec:cross-benchmark}
% ==================================================================

\subsubsection{End-to-End Validation of EFE}
\label{sec:cross-validation}

Together, \PSEBench{} and \CliniCARE{} exercise the complete EFE path from
workflow specification to deployment analysis. Table~\ref{tab:seed-efe}
summarizes the mapping.

\begin{table}[t]
\centering
\caption{The two seed benchmarks as reference implementations of EFE.}
\label{tab:seed-efe}
\small
\begin{tabular}{
>{\raggedright\arraybackslash}p{0.34\textwidth}
>{\raggedright\arraybackslash}p{0.27\textwidth}
>{\raggedright\arraybackslash}p{0.29\textwidth}
}
\toprule
\textbf{EFE component} & \textbf{\PSEBench{}} & \textbf{\CliniCARE{}} \\
\midrule

Workflow specification
& Patient-safety event triage
& Retrospective clinical audit \\

Governed context
& Event narrative, MN29 policy, controlled information provider
& Longitudinal EHR, clinical tools, computation, policy corpus \\

Primary deployment track
& Evidence-grounded insight
& Evidence-grounded insight \\

Primary risk surface
& Evidence and reasoning
& Evidence and reasoning \\

Observable trajectory
& ASK/ANSWER sequence, retrieved facts, final report
& Retrievals, computations, policy accesses, final report \\

Outcome evaluation
& Verdict and target-clause correctness
& Four-way adjudication correctness \\

Grounding / process evaluation
& Legal evidence, boundary conditions, information seeking
& Patient evidence, policy grounding, MUST-DO/MUST-NOT process rubric \\

Abstention / escalation
& Missing-information and policy-ambiguity handling
& Lack-of-data and medical-ambiguity verdicts \\

Reliability evidence
& Controlled escalation diagnostics
& Confidence calibration and repeated trials \\

EFE output
& Reliability/oversight mapping and bounded triage role
& Reliability/autonomy mapping and bounded audit role \\

\bottomrule
\end{tabular}
\end{table}

The benchmarks deliberately differ in how ground truth is obtained.
\PSEBench{} emphasizes controllability: policy logic is factorized before
case generation, producing rich by-construction annotations and explicit
missing-information and gray-zone variants. \CliniCARE{} emphasizes
ecological validity: the environment contains real longitudinal EHR records,
and reference adjudications are generated through a model-assisted procedure
calibrated against clinical review. Their agreement on the need to evaluate
more than final-answer accuracy is therefore informative because it arises
under substantially different benchmark-construction regimes.

\subsubsection{Task Accuracy Is Not Deployment Qualification}
\label{sec:cross-accuracy}

Both benchmarks demonstrate that aggregate task accuracy is insufficient for
deployment qualification.

In \PSEBench{}, systems with strong verdict accuracy differ sharply in
whether they request missing information and recognize policy ambiguity. In
\CliniCARE{}, defect-free accuracy reorders systems relative to raw verdict
accuracy because some correct conclusions are reached through prohibited or
insufficiently defensible processes.

EFE therefore treats task correctness as one input to qualification rather
than as the qualification itself.

\subsubsection{Accuracy and Escalation Quality Jointly Determine Value}
\label{sec:cross-escalation}

Base task performance determines how much work a system could in principle
handle. Escalation quality determines whether human review can be allocated
to the cases where it is most valuable.

\PSEBench{} exposes this distinction directly through missing-information
and uncertainty-detection behavior. \CliniCARE{} exposes it through
four-way abstention labels, directional over-commitment and over-abstention,
and per-case confidence.

Consequently, two systems with similar aggregate accuracy can support
different autonomous coverage at the same reliability target. This is why
the EFE unit of evaluation is
\emph{agent $\times$ workflow $\times$ deployment policy}, rather than the
agent alone.

\subsubsection{Human Review Versus Model Cost}
\label{sec:cross-cost}

For the clinical-review workflows and cost assumptions studied here, the
dominant variable in the EFE operating-cost model is human review rather
than model inference. The reason is not that model cost is universally
negligible, but that review of a consequential clinical or patient-safety
case is substantially more expensive than a single model execution under
the assumptions used in our analysis.

The economically important agent property is therefore the fraction of
cases that can be handled autonomously while satisfying the required
reliability and hard gates. Better task performance lowers the amount of
review needed; better confidence discrimination lowers it further by
directing review toward the cases most likely to fail.

This conclusion is specific to the studied workflows, pricing assumptions,
and review model and should not be generalized to enterprise tasks with
different model, latency, human-labor, or failure costs.

\subsubsection{Deployment Rankings Depend on the Operating Target}
\label{sec:cross-target}

Neither benchmark implies a universal ordering of systems for deployment.
The preferred system and policy can change with:

\begin{itemize}
    \item the required reliability;
    \item tolerance for particular critical failure classes;
    \item human-review accuracy;
    \item human-review and approval cost;
    \item the quality of the system's confidence or escalation signal; and
    \item the autonomous coverage required for the deployment to be
    economically useful.
\end{itemize}

EFE therefore reports an operating envelope or frontier rather than a single
context-free ``enterprise readiness'' rank.

\subsubsection{Boundaries of the Current Evidence}
\label{sec:cross-boundaries}

The two seed benchmarks provide completed reference implementations of EFE
for healthcare-related evidence-grounded workflows. They demonstrate
governed information access, policy-grounded reasoning, trajectory capture,
outcome and process evaluation, abstention and escalation, repeated or
confidence-based reliability analysis, and translation into bounded
deployment policies.

They do not yet empirically validate the full scope of EFE.
Neither benchmark grants an evaluated agent consequential state-changing
authority, so they do not test the complete Track~2 surface of transactional
correctness, approval-before-commit, idempotency, rollback, or downstream
state propagation. Nor do they evaluate an open user-facing workflow in
which uncontrolled user interaction itself is the principal risk surface.

The current evidence should therefore be read as an end-to-end validation of
the EFE architecture for evidence-grounded enterprise workflows, not as
empirical validation of every deployment track defined by the standard.
Future reference benchmarks can extend the same specification and platform
to state-changing and open-interaction workflows without changing the core
EFE abstraction.

% ==================================================================
% TEMPORARY AUTHOR TODO -- REMOVE ENTIRE BOX BEFORE SUBMISSION
% ==================================================================

\begin{efetodo}{Submission Blocker: Complete the Empirical EFE Qualification Analysis}

\textbf{Goal.}
Turn the current benchmark results into an actual EFE deployment
qualification result. The final paper should show, quantitatively, how
measured agent behavior maps to autonomous coverage, human-review burden,
reliability, cost, and a representative deployment profile.

\vspace{4pt}
\textbf{\textcolor{todored}{Phase 0 --- Freeze the deployment question}}

\begin{itemize}
    \item \todocritical{
    Use \CliniCARE{} as the primary quantitative demonstration of the
    reliability--autonomy and oversight-economics framework.}

    \item \todocheck{
    Deployment setting:
    the agent performs retrospective clinical audit and produces a draft
    adjudication; sufficiently reliable cases may be accepted without
    additional review, while the remaining cases are escalated to a human
    reviewer.}

    \item \todocritical{
    Freeze the primary autonomous-success definition before looking at the
    qualification results. Recommended:
    \[
    \text{deployment success}
    =
    \text{correct verdict}
    \land
    \text{no disqualifying process defect}.
    \]
    Also retain verdict correctness alone as a secondary analysis.}

    \item \todocheck{
    Do not change the success definition after examining which systems benefit
    from it.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todoorange}{Phase 1 --- Construct the case-level analysis table}}

\begin{itemize}
    \item \tododata{
    Produce one row for every evaluated
    \texttt{system $\times$ case}.}

    \item \tododata{
    Include at least:
    \texttt{system\_id},
    \texttt{case\_id},
    \texttt{scenario\_id},
    \texttt{reference\_verdict},
    \texttt{predicted\_verdict},
    \texttt{verdict\_correct},
    \texttt{confidence},
    \texttt{process\_defect},
    \texttt{deployment\_success},
    \texttt{reference\_requires\_abstention},
    \texttt{agent\_abstained},
    \texttt{overcommit},
    \texttt{overabstain},
    evidence-grounding metrics,
    policy-grounding metrics,
    and measured model cost.}

    \item \tododata{
    Export the underlying unrounded case-level data and all derived summary
    tables to CSV/JSON so every reported result can be regenerated.}

    \item \todocritical{
    Use case-level outputs as the source of truth; do not reconstruct
    qualification results from rounded leaderboard numbers.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todored}{Phase 2 --- Resolve development versus qualification data}}

\begin{itemize}
    \item \todocritical{
    Verify whether the current 148-case \CliniCARE{} development subset is
    disjoint from the 750-case primary evaluation set.}

    \item \todocritical{
    If the 148 cases are contained in the 750, they cannot be used both to
    select the deployment threshold and to estimate held-out qualification
    reliability.}

    \item \tododata{
    Establish a fixed, reproducible development/qualification split.
    Preferred simple design:
    select the routing policy on development data, freeze it, and report its
    performance on disjoint qualification data.}

    \item \todocheck{
    Record the split definition and random seed/version in the evaluation
    configuration.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todoblue}{Phase 3 --- Compute the CliniCARE risk--autonomy results}}

\begin{itemize}
    \item \todoanalysis{
    For each system, rank cases by the stated per-case confidence and sweep
    the autonomy threshold $\tau$.}

    \item \todoanalysis{
    At every operating point compute:
    \[
    c(\tau),\qquad
    r(c),\qquad
    a(c),\qquad
    e(c)=1-c.
    \]
    }

    \item \todoanalysis{
    Compute the curve using the primary deployment-success definition and
    separately using verdict correctness alone.}

    \item \todoanalysis{
    Compute AURC, oracle AURC, and E-AURC as defined in
    Section~\ref{sec:qualification-diagnostics}.}

    \item \todoanalysis{
    Add an oracle ordering that escalates autonomous failures first.}

    \item \todoanalysis{
    Select only 3--4 systems for the main figure:
    (i) strongest overall system,
    (ii) a system with similar task accuracy but meaningfully different
    confidence discrimination,
    (iii) one weaker representative system,
    and (iv) the oracle.}

    \item \todopaper{
    Produce one main-paper figure:
    \textbf{risk versus autonomous coverage}.
    The figure should make visible that similar aggregate accuracy can imply
    different useful autonomy.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todoblue}{Phase 4 --- Produce actual qualification policies}}

\begin{itemize}
    \item \todoanalysis{
    Pre-specify representative deployment reliability targets, e.g.
    \[
    Y \in \{0.90,\,0.95,\,0.97\}.
    \]
    Adjust only if there is a substantive deployment reason.}

    \item \todoanalysis{
    Specify human-review assumptions used for the primary analysis,
    including $a_h$ and $k_h$. Clearly label them as deployment assumptions,
    not benchmark measurements.}

    \item \todoanalysis{
    For each representative system and target $Y$, compute:
    \begin{itemize}
        \item qualified autonomous coverage $c^\star(Y)$;
        \item escalation rate $1-c^\star(Y)$;
        \item empirical deployment reliability;
        \item one-sided lower confidence bound on reliability;
        \item model cost per case;
        \item human-review cost per case;
        \item total oversight-adjusted cost;
        \item oracle escalation rate and oracle cost;
        \item excess cost due to imperfect discrimination.
    \end{itemize}
    }

    \item \todoanalysis{
    If no threshold satisfies the statistical qualification requirement for
    a target, report \emph{not qualified} or \emph{insufficient evidence};
    do not extrapolate.}

    \item \todopaper{
    Produce one compact main-paper table with columns of the form:
    \[
    \text{System}
    \;|\;
    \text{Target}
    \;|\;
    \text{Coverage}
    \;|\;
    \text{Review}
    \;|\;
    \text{Reliability [LCB]}
    \;|\;
    \text{Cost}
    \;|\;
    \text{Qualified?}.
    \]
    }
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todoblue}{Phase 5 --- Statistical qualification}}

\begin{itemize}
    \item \todoanalysis{
    Select routing thresholds using development data only. Freeze the
    threshold before evaluating qualification data.}

    \item \todoanalysis{
    Report a one-sided lower confidence bound
    $R_{\mathrm{LCB}}(\pi)$ for the selected deployment policy, consistent
    with Section~\ref{sec:qualification-statistics}.}

    \item \todoanalysis{
    Use task/case-level bootstrap or another procedure consistent with the
    sampling design. Do not treat repeated executions of the same case as
    independent cases.}

    \item \todoanalysis{
    Where sample size is insufficient to establish the target reliability,
    explicitly report \emph{insufficient evidence for qualification}.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todogreen}{Phase 6 --- Generate one real deployment profile}}

\begin{itemize}
    \item \todopaper{
    Select one representative \CliniCARE{} system and instantiate an actual
    EFE deployment profile from the measured results.}

    \item \todopaper{
    The profile should report at least:
    \begin{itemize}
        \item workflow and deployment track;
        \item consequence class;
        \item qualified authority;
        \item actions permitted autonomously;
        \item target deployment reliability;
        \item achieved reliability and uncertainty bound;
        \item autonomous coverage;
        \item human-review coverage;
        \item mandatory escalation conditions;
        \item hard-gate results;
        \item residual failure modes; and
        \item expected oversight-adjusted operating cost.
    \end{itemize}
    }

    \item \todopaper{
    Replace the current hypothetical language in
    Section~\ref{sec:clinicare-profiles} with this measured deployment
    profile.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todoorange}{Phase 7 --- Handle PSEBench separately}}

\begin{itemize}
    \item \todocritical{
    Do not construct a confidence-threshold risk--autonomy curve from
    aggregate uncertainty-detection F1.}

    \item \tododata{
    Check whether the raw \PSEBench{} outputs contain a meaningful per-case
    confidence, logit, or other pre-specified routing score.}

    \item \todoanalysis{
    If a valid per-case routing signal exists, run the same held-out
    selective-deployment analysis used for \CliniCARE{}.}

    \item \todopaper{
    If no valid per-case routing signal exists, use \PSEBench{} as the
    complementary demonstration of escalation competence:
    report verdict accuracy together with missing-information detection,
    targeted information seeking, grounding, and uncertainty detection.}

    \item \todopaper{
    Explicitly state that \PSEBench{} demonstrates information-acquisition
    and escalation behavior but is not used to estimate the full
    confidence-threshold EFE risk--autonomy frontier.}
\end{itemize}


\vspace{4pt}
\textbf{\textcolor{todogreen}{Phase 8 --- Rewrite the paper around the completed results}}

\begin{itemize}
    \item \todopaper{
    Replace Section~\ref{sec:clinicare-economics} with the actual
    risk--autonomy, statistical qualification, and cost results. Remove the
    sentence saying that the final analysis ``should therefore be computed.''}

    \item \todopaper{
    Replace Section~\ref{sec:clinicare-profiles} with the measured
    representative deployment profile.}

    \item \todopaper{
    Revise Section~\ref{sec:pse-economics} so that it makes only the
    quantitative claims supported by the available PSEBench routing signal.}

    \item \todopaper{
    Update Section~\ref{sec:cross-validation} to say that the two benchmarks
    provide end-to-end validation of EFE for
    \emph{evidence-grounded workflows}, not all three deployment tracks.}

    \item \todopaper{
    Update Sections~\ref{sec:cross-accuracy},
    \ref{sec:cross-escalation}, and \ref{sec:cross-cost} with the final
    measured cross-system findings.}

    \item \todopaper{
    Recheck the abstract and Introduction so that every claim about autonomous
    coverage, escalation burden, reliability, or operating cost is directly
    supported by the final analysis.}

    \item \todocritical{
    REMOVE THIS ENTIRE TODO BOX BEFORE SUBMISSION.}
\end{itemize}

\end{efetodo}

==> old/reference_bench_bk_0810.tex <==
\section{ Seed Benchmark and Reference Implementation}
\label{sec:psebench}
% ==================================================================
\subsection{\PSEBench}
\subsubsection{Enterprise Workflow and Deployment Question}
\label{sec:pse-workflow}

% TODO:
% Describe the patient-safety event-review workflow, intended reviewer,
% organizational decision, governing policies, and deployment question.


\subsubsection{Mapping to the EFE Standard}
\label{sec:pse-standard}

% TODO:
% Report:
% - context metadata;
% - deployment tracks;
% - active risk surfaces;
% - deployment contract;
% - risk class;
% - evaluation primitives;
% - canonical record.


\subsubsection{Benchmark Construction and Validation}
\label{sec:pse-construction}

% TODO:
% Import concise finalized material from the completed PSEBench paper:
% - source data;
% - task and case creation;
% - expert involvement;
% - reference construction;
% - adjudication;
% - grader validation;
% - benchmark size and splits.


\subsubsection{Evaluation Protocol and Baseline Systems}
\label{sec:pse-protocol}

% TODO:
% Specify:
% - final benchmark version;
% - model and agent configurations;
% - repeated runs;
% - confidence elicitation;
% - token-cost assumptions;
% - human-review assumptions.


\subsubsection{Benchmark Results}
\label{sec:pse-results}

% TODO:
% Present measured task-level and primitive-level results before presenting
% derived economic quantities.


\subsubsection{Oversight Economics}
\label{sec:pse-economics}

% TODO:
% Present cost-of-reliability curves and distinguish:
% - measured benchmark quantities;
% - assumed human parameters;
% - modeled or simulated economic mappings.
%
% Verify and regenerate all table values from unrounded escalation rates.


\subsubsection{Representative Deployment Profiles}
\label{sec:pse-profiles}

% TODO:
% Show deployment-profile cards for representative systems.


% ==================================================================
\subsection{\CliniCARE: Seed Benchmark and Reference Implementation}
\label{sec:clinicare}

\subsubsection{Enterprise Workflow and Deployment Question}
\label{sec:clinicare-workflow}

CliniCARE-Bench evaluates the defensibility of evidence-grounded
retrospective clinical adjudication over longitudinal records, rather than
medical-knowledge recall in isolation.


\subsubsection{Mapping to the EFE Standard}
\label{sec:clinicare-standard}

% TODO:
% Report:
% - clinical-review role;
% - Track 1 deployment surface;
% - longitudinal evidence environment;
% - policy grounding;
% - expected work product;
% - authority boundary;
% - verdict and abstention schema;
% - escalation conditions;
% - risk class;
% - evaluation primitives.


\subsubsection{Benchmark Construction and Validation}
\label{sec:clinicare-construction}

% TODO:
% Summarize the completed benchmark:
% - 25 scenarios;
% - candidate-case generation;
% - 750 cases;
% - independent multi-model oracle ensemble;
% - physician review;
% - adjudication process;
% - evidence and policy requirements;
% - final benchmark version.


\subsubsection{Evaluation Protocol and Baseline Systems}
\label{sec:clinicare-protocol}

% TODO:
% Specify:
% - systems evaluated;
% - confidence elicitation;
% - held-out evaluation;
% - tie handling;
% - repeated trials;
% - human-review assumptions.


\subsubsection{Outcome, Grounding, Process, and Abstention Results}
\label{sec:clinicare-results}

% TODO:
% Report:
% - verdict performance;
% - required-evidence coverage;
% - evidence grounding;
% - policy grounding;
% - process adherence;
% - abstention behavior;
% - repeated-trial reliability;
% - efficiency.


\subsubsection{Reliability--Autonomy and Oversight Analysis}
\label{sec:clinicare-economics}

% TODO:
% Insert final risk--autonomy and cost-of-reliability results.
% Remove all ``preliminary'' and ``early task set'' language.


\subsubsection{Representative Deployment Profiles}
\label{sec:clinicare-profiles}

% TODO:
% Show representative operating policies and identify cases that remain
% unsuitable for autonomous handling.


% ==================================================================
\subsection{What the Two Seed Benchmarks Demonstrate}
\label{sec:cross-benchmark}
% ==================================================================

\subsubsection{End-to-End Validation of EFE}
\label{sec:cross-validation}

% TODO:
% Add a benchmark-by-EFE-component matrix showing:
% - canonical task specification;
% - governed enterprise context;
% - controlled execution;
% - trajectory capture;
% - outcome evaluation;
% - process evaluation;
% - abstention and escalation;
% - oversight simulation;
% - deployment-profile output.


\subsubsection{Task Accuracy Is Not Deployment Qualification}
\label{sec:cross-accuracy}

Two systems with similar aggregate task accuracy may support substantially
different deployment policies if their errors are distributed differently
across confidence-ranked cases.


\subsubsection{Accuracy and Escalation Quality Jointly Determine Value}
\label{sec:cross-escalation}

Base task performance determines the starting point for deployment.
Confidence discrimination determines how efficiently human oversight can be
allocated to the cases most likely to fail.


\subsubsection{Human Review Versus Model Cost}
\label{sec:cross-cost}

Under the clinical-review workflows and human-review assumptions studied in
\PSEBench{} and \CliniCARE{}, human oversight dominates differences in
per-case model inference cost.

% Important:
% State this as a result under the studied workflows and assumptions,
% not as a universal fact for all enterprise deployments.


\subsubsection{Deployment Rankings Depend on the Operating Target}
\label{sec:cross-target}

The preferred system and policy may change with:

\begin{itemize}
    \item the target reliability;
    \item the critical-risk tolerance;
    \item human-review accuracy;
    \item human-review cost;
    \item acceptable autonomous coverage.
\end{itemize}


\subsubsection{Boundaries of the Current Evidence}
\label{sec:cross-boundaries}

The two seed benchmarks provide completed, end-to-end demonstrations of EFE
for healthcare-related evidence-grounded workflows. They do not yet
empirically validate every state-changing or open-interaction capability
supported by the broader standard and platform.


==> old/sections/00_abstract.tex <==
\begin{abstract}


AI-agent benchmarks increasingly test professional, computer-use, and economically valuable work, asking whether an agent \emph{can} complete a task. Enterprise deployment turns on a different question: whether an organization can safely \emph{employ} an agent within a defined role, authority boundary, oversight policy, and cost budget. We introduce \textbf{Enterprise's First Exam (EFE)}, a reliability-oriented framework that qualifies agents for deployment on authentic enterprise workflows. EFE makes four contributions. First, it reframes enterprise evaluation around safe employment rather than task completion. Second, it provides a multi-axis task taxonomy, spanning industry context, work activity, autonomy tier, role and authority, workflow state and work product, consequence and reversibility, and reliability primitives, that guides test coverage across three cumulative deployment tiers: evidence-grounded insight, state-changing workflows, and open user-facing tasks. Third, it defines a single headline metric, the \emph{total cost of safe task completion}, by treating an agent's accept-or-escalate decision as selective prediction with human deferral, together with discrimination diagnostics (AURC and excess-AURC). Fourth, it delivers an evaluation platform comprising task specification, agent harness, and environment, with an oversight simulator that returns a deployment profile in place of a single global score. Applying the metric to a 15-model patient-safety leaderboard and a clinical-audit benchmark, we find that per-token price is negligible against the cost of human review, that the dominant cost driver is a model's calibrated ability to recognize which cases it should escalate, and that as agents improve, the human-oversight cost of meeting a fixed reliability target falls. We close with a call for participation and a phased plan to release EFE as a community benchmark.
\end{abstract}

==> old/sections/00_abstract_0728.tex <==
\begin{abstract}
Existing AI-agent benchmarks focus on testing whether an agent can \emph{complete} professional or economically valuable work. Enterprise deployment requires a broader determination: whether an organization can \emph{safely employ} an agent within a defined role, authority boundary, oversight policy, reliability requirement, and operating budget. We introduce Enterprise’s First Exam (EFE), \emph{an open standard and evaluation platform for qualifying AI agents for enterprise deployment.} 
% emily: need more iteration here to highlight contribution. currently it is too generic.
EFE specifies enterprise tasks across professional context, work activity, autonomy surface, role and authority, workflow state, consequence and reversibility, and reusable reliability primitives. It combines versioned task specifications, controlled execution environments, normalized agent adapters, immutable trajectory and state records, evaluation engines, and an oversight simulator that returns a deployment profile rather than a single global score. 

We launch EFE with two seed benchmarks, PSEBench and CliniCARE-Bench, which serve as reference implementations of the standard and demonstrate the platform end to end. Across these benchmarks, we demonstrate how deployment-relevant quantities, including autonomous coverage, escalation burden, residual risk, and the human-oversight cost required to meet a target reliability. The results show that human review, rather than token price, dominates the economics of reliable deployment, and that an agent’s ability to identify which cases require escalation is a primary determinant of its safe operating cost. We release EFE as an extensible platform and standard and invite contributions of additional enterprise workflows, environments, policies, assets, and evaluation methods.

\end{abstract}

==> old/sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Enterprise teams adopt agents along a reliability gradient. They start where the blast radius is smallest: read-only agents that retrieve and synthesize information. They then move toward agents that write back into systems of record. Finally, they deploy agents that hold open conversations with users to complete tasks. Each step unlocks more value and widens the evaluation surface. A read-only research agent may produce a wrong or incomplete insight, but a human reviewer can still catch the error before acting. A workflow automation agent may update the wrong enterprise record, and that update may propagate downstream. A user-facing agent may be steered by a confused, demanding, or adversarial user in real time.

Recent benchmarks increasingly evaluate this kind of professional work. Computer-use and long-horizon agent exams ask whether a generalist agent can complete authentic professional workflows \citep{agentslastexam}, economically-grounded evaluations ask whether a model's work product is as good as an expert's \citep{gdpval}, and profession-aligned evaluations ask whether a domain agent creates measurable business value \citep{xbench}, often organized by a taxonomy of work activities \citep{workactivitytax}. These are valuable, but they answer whether an agent \emph{can do the work}. An enterprise deployment decision turns on a different question, and a different unit of analysis.

\begin{quote}
\textit{Professional-work benchmarks ask whether an agent can do the work. Enterprise's First Exam asks whether an organization can safely employ the agent, under a specified operating policy, at an acceptable total cost.}
\end{quote}

We introduce \textbf{Enterprise's First Exam}, a reliability-oriented evaluation and \emph{deployment-qualification} framework for enterprise AI agents. It is not another general professional-work benchmark, but a gating layer built on top of authentic professional tasks and workflows. The term ``First Exam'' is intentional, as it is not a final exam for full autonomy, but the first deployment gate an agent must pass before it can be trusted in enterprise use with bounded human oversight. Passing the exam does not mean the agent requires no supervision. It means the agent has reached a minimum reliability threshold, its remaining risks are measurable, and the required human-oversight policy can be specified. The framework preserves three \textbf{cumulative deployment tiers}:

\emily{currently we treat:
Tier 1: read and synthesize;
Tier 2: write enterprise state;
Tier 3: interact openly with a user, as cumulative levels. But these are partly independent surfaces: A customer-facing informational agent may be open and interactive but read-only.
A background payment or clinical-ordering agent may have no user conversation but be far riskier than many Tier-3 agents.
An interactive support agent may propose a write but never commit it.
Interaction openness and mutation authority are different dimensions. replacing “three cumulative tiers” with three deployment surfaces: [Surface	Possible levels]
1) Evidence access	retrieve, synthesize, infer; 
2) Action authority	recommend, propose, approve, commit; 3) Interaction openness	fixed request, controlled dialogue, open user interaction}


\begin{itemize}[leftmargin=1.4em]
  \item \textbf{Tier 1: Evidence-Grounded Insight Agents} are read-only agents that retrieve, analyze, and synthesize enterprise information into decision-support artifacts, such as due-diligence reports, patient-safety reviews, and contract analyses.
  \item \textbf{Tier 2: State-Changing Workflow Agents} extend Tier 1 by writing back into enterprise systems of record, such as creating cases, updating CRM or ERP records, filing prior-authorization requests, resolving IT tickets, or reconciling vendor statements.
  \item \textbf{Tier 3: Open User-Facing Task-Completion Agents} complete tasks through open-ended interaction with users while following policy and protecting users.
\end{itemize}

Each tier expands the agent's \textbf{autonomy surface}, increases the \textbf{consequence of failure}, and changes the \textbf{economics of evaluation and oversight}. Passing the exam does not grant unlimited autonomy. Instead, it produces a \emph{deployment profile}, denoting which tier of work the agent is qualified for, what risks remain, what human-oversight policy is required, which actions can be autonomous, which require approval, what monitoring and audit trails are needed, and how the human-oversight cost should decline as the agent improves. This makes Enterprise's First Exam both a benchmark and a deployment governance framework.

The Enterprise's First Exam contributes:
\begin{enumerate}[leftmargin=1.6em]
  \item A \textbf{positioning of enterprise evaluation} relative to professional-work, economically-valuable-task, and profession-aligned benchmarks (\cref{sec:positioning}), reframing agent evaluation as a deployment-qualification and economics problem rather than a task-completion problem.
  \item A \textbf{multi-axis task taxonomy} for enterprise exams (\cref{sec:taxonomy}): industry and professional context, work activity, deployment and autonomy tier, role and authority, workflow state and work product, consequence and reversibility, and reliability primitives, together with a canonical task record that makes each task reproducible and its deployment envelope explicit.
  \item A \textbf{headline metric}, the total cost of safe task completion, derived from selective prediction with human deferral, with an oracle lower bound and discrimination diagnostics; and empirical instantiations on a patient-safety leaderboard and a clinical-audit benchmark (\cref{sec:calibration}).
  \item An \textbf{evaluation platform:} task specification $\times$ agent harness $\times$ environment, with an \emph{oversight simulator} and a \emph{deployment-profile output} in place of a single global score (\cref{sec:platform}), and a \textbf{call for participation} and phased release plan for a community benchmark (\cref{sec:call}).
\end{enumerate}

\begin{quote}
\textit{Enterprise readiness is not merely task completion. It is grounded, auditable, policy-compliant, safe, and cost-effective task completion under realistic enterprise constraints.}
\end{quote}


==> old/sections/02_related_work.tex <==
\section{Related Work and Positioning}
\label{sec:related}

\subsection{Positioning among evaluation families}
\label{sec:positioning}

Enterprise's First Exam should not be positioned as another general professional-work benchmark. It should be a deployment-qualification framework layered on authentic professional tasks and workflows. \Cref{tab:positioning} locates it relative to adjacent evaluation families, whereas each of those measures some facet of whether the work is good, useful, or completable, EFE measures whether the agent can be safely employed under a specified operating policy at an acceptable total cost.

\begin{table}[h]
\centering
\small
\begin{tabularx}{\textwidth}{L{2.6cm} Y L{3.0cm} L{3.2cm}}
\toprule
\textbf{Evaluation} & \textbf{Primary question} & \textbf{Unit of evaluation} & \textbf{Distinctive output} \\
\midrule
\textbf{Enterprise's First Exam (ours)} & Can this agent be deployed safely, under what authority and oversight, and at what operating cost? & Agent $\times$ workflow $\times$ deployment policy & Deployment profile: qualified autonomy tier, residual risks, escalation rate, and oversight cost \\
Agents' Last Exam \citep{agentslastexam} & Can a generalist computer-use agent complete authentic, long-horizon professional work? & Executable professional workflow & Artifact or state-completion score \\
GDPval / GDPEval \citep{gdpval} & Is the model-generated work product as good as an expert's? & Professional request and deliverable & Human-expert comparative quality and potential time or cost savings \\
Profession-aligned evaluation \citep{xbench} & Does a domain-specific agent create measurable professional productivity or business value? & Live demand from a particular profession & Profession-specific score and technology--market-fit signal \\
\bottomrule
\end{tabularx}
\caption{Positioning of Enterprise's First Exam relative to adjacent evaluation families.}
\label{tab:positioning}
\end{table}

\paragraph{What EFE adopts from adjacent benchmarks.} From long-horizon computer-use exams \citep{agentslastexam}, EFE adopts authentic professional projects, an expert advisory committee, separation of the task specification from the agent harness and execution environment, staged review gates from sourcing through quality control, preserved hidden references and full agent trajectories, and private or server-side evaluation instances. From economically-grounded evaluation \citep{gdpval}, it adopts recruiting experienced professionals, collecting both the request and an expert work product, measuring human completion time and estimated labor cost, and comparing agent artifacts against expert artifacts using multiple independent reviews where deterministic grading is not credible. From profession-aligned evaluation \citep{xbench, workactivitytax}, it adopts mapping the real business process, estimating how professionals allocate time across work activities, prioritizing workflows with clear demand and measurable value, and refreshing tasks as the professional environment changes.

\paragraph{What is unique to EFE.} On top of this synthesis, EFE adds policy, authority, escalation, blast radius, repeated-trial reliability, and oversight economics. Its headline question is: \emph{what is the minimum-cost deployment policy that meets a required reliability level?} The remainder of this section reviews the reliability-estimation literature that our headline metric consumes.

\subsection{Confidence and Uncertainty Estimation for LLMs}

The signal our calibration map ingests comes from work on self-assessed
correctness. \citet{kadavath2022language} show that large models are well
calibrated on multiple-choice and true/false questions in the right format, and elicit \emph{P(True)} (propose an answer, then score its correctness) as well as \emph{P(IK)} (does the model know?). Their finding that P(IK) is poorly calibrated on new tasks is not a footnote for us but a \emph{priced input}: exactly the cross-task calibration gap they report is what our safety margin $\delta(\varepsilon)$ converts into additional escalation cost. \citet{ren2023selfeval} are closest in spirit: token-level self-evaluation with an explicit ``none of the above'' abstention, benchmarked for selective generation. But their unit is the quality of one generation on TruthfulQA/TL;DR and their output is a selective-generation curve; we lift the same signal into an agentic, write-capable setting and replace the curve with a single cost-optimal operating point tied to a human-review price $k_h$. Sampling-based estimators, such as semantic entropy \citep{kuhn2023semantic} and confidence-weighted self-consistency  \citep{taubenfeld2025confidence}, are not merely ``expensive'' in our setting: they are \emph{structurally incompatible} with our economic metric, since every additional sample multiplies the per-case token cost $k_m$ that the framework is built to minimize, ruling them out as the operative online signal even where they are most accurate offline. Verbalized-confidence work \citep{lin2022teaching, tian2023just} and the finding that verbalized scores can beat RLHF-model logits are, for us, evidence about \emph{which source} of $s_i$ is best, a choice we leave open; we instead price the downstream cost of a miscalibrated signal (\cref{sec:calibration}). The remaining estimators, spanning relative confidence preferences \citep{shrivastava2025relative}, input-clarification ensembling \citep{hou2024decomposing}, functional-level UQ \citep{niu2024functional}, and logit-layer selection studies \citep{ma2025inferring}, all target the accuracy of the estimate itself; none attach a cost to being wrong about one's own confidence, which is our central quantity.

\subsection{Calibration of Language Models}

Every method in this line \emph{improves} calibration; EFE, by contrast,
\emph{monetizes the residual}. \citet{guo2017calibration} showed modern networks
are overconfident and that temperature scaling corrects it;
\citet{braverman2020calibration} study calibration drift over long generations;
\citet{jiang2021know} and \citet{chen2023close} characterize when QA calibration
holds, while \citet{tian2023just} warn that RLHF degrades it. We take all of this
as given and assume calibration is imperfect. Post-hoc correctors
(adaptive temperature scaling, \citealp{xie2024adaptive}; graph-based
calibration, \citealp{li2024graph}) and training-time correctors
(calibration-tuning to know what a model does not know,
\citealp{kapoor2024calibration}; listener-aware LACIE,
\citealp{stengeleskin2024lacie}), along with sequence-likelihood calibration
(SLiC, \citealp{zhao2022slic}; SLiC-HF, \citealp{zhao2023slichf}) and the caution
that likelihood over-optimizes in direct alignment algorithms
\citep{shi2024understanding}, are all interchangeable instantiations of our map
$g$. Our contribution is orthogonal and, to our knowledge, new: a mapping from
residual calibration error to a \emph{deployment price}, via the threshold
inflation $\tau^\star + \delta(\varepsilon)$ and the resulting increase in
escalation rate. Where these papers report a better ECE, we report
what that ECE is worth in review dollars at reliability $Y$.

\subsection{Selective Prediction, Abstention, and Deferral}

Our accept-or-escalate rule is selective prediction with human deferral, but prior
work optimizes the wrong objective for enterprise deployment. Conformal methods
give distribution-free \emph{coverage} guarantees: \citet{kumar2023conformal} for
multiple-choice QA, and \citet{su2024api} crucially without logit access. Yet
coverage is not what an operator pays for; we instead choose the operating point
that satisfies a reliability constraint at least cost,
minimizing $k_m + k_h\,(1-c)$ subject to $R(c) \ge Y$.
(\citeauthor{su2024api}'s logit-free result matters specifically because
enterprises run closed models where $s_i$ from an API is all that exists.) The
\citet{ren2023robots} robots-that-ask-for-help framework aligns a planner's
uncertainty to a human-help threshold via conformal prediction, mirroring our gate
for a single embodied agent; we generalize deferral to a portfolio priced across
three deployment tiers and, unlike any of this work, decompose the error budget
into \textbf{under-escalation} (a confident wrong verdict that forces the gate
upward and raises cost globally) versus \textbf{over-escalation} (deferring
answerable cases and wasting human time), two economically distinct failures that
a single coverage or risk number cannot separate.

\subsection{Truthfulness, Faithfulness, and Hallucination}

This line supplies methods to detect or improve truthfulness; EFE takes a
deliberately stricter stance for a deployment gate. SelfCheckGPT
\citep{manakul2023selfcheckgpt} detects hallucination from sampled-response
consistency, Inference-Time Intervention \citep{li2023inference} steers activations
toward truthful directions, and probing work argues that LLMs know more than they
show \citep{orgad2024llms} via internal signals. These are valuable, but each
relies on a \emph{model-internal} or self-consistency signal, whereas our Grounding
primitive demands \emph{external, human-auditable} traceability of every claim to
evidence that genuinely supports it, a bar that an internal truthfulness signal
does not clear in a regulated setting. The reason we insist on this is sharpened by
faithfulness research: work measuring faithfulness in chain-of-thought reasoning
\citep{lanham2023measuring} and showing that language models do not always say what
they think \citep{turpin2023language} establishes that a plausible rationale need
not be the decision's true cause. We therefore define auditability as verifiable
evidence-and-action traceability rather than as trust in the agent's narrated
explanation.


==> old/sections/03_organizing_principle.tex <==
\section{The Organizing Principle: Autonomy Surface, Failure Consequence, and Oversight Economics}
\label{sec:principle}

The tiers are cumulative: Tier 2 inherits the relevant requirements of Tier 1 and adds write-action safety, and Tier 3 inherits the relevant requirements of Tiers 1 and 2 and adds open-interaction robustness, adversarial safety, and repeated-trial reliability.

\paragraph{Autonomy surface.} In Tier 1, the agent reads: it retrieves, analyzes, summarizes, and synthesizes, and it does not change enterprise state. In Tier 2, the agent writes: it updates records, creates tickets, files submissions, routes approvals, or triggers workflow transitions. In Tier 3, the agent converses and negotiates the task itself: it must infer intent, collect missing information, handle corrections, apply policy, use tools, and complete the task through open interaction. The autonomy surface grows from \emph{retrieve and synthesize} $\rightarrow$ \emph{change system state} $\rightarrow$ \emph{negotiate and complete a task with a live user}.

\paragraph{Failure consequence.} In Tier 1, the main failure is a misleading or incomplete insight, often recoverable because a human reviewer can catch the issue before acting. In Tier 2, the main failure is an incorrect write that has already changed the enterprise system of record. In Tier 3, the agent faces uncontrolled input from users who may be confused, emotional, demanding, adversarial, or malicious, and may be pressured into policy violations, unsafe actions, or privacy leakage. The failure consequence grows from \emph{misleading insight} $\rightarrow$ \emph{incorrect system mutation} $\rightarrow$ \emph{unsafe or policy-violating user interaction}.

\paragraph{Oversight economics.} Oversight economics has two linked components. \emph{Offline evaluation cost} is paid before deployment (benchmark construction, expert annotation, rubric design, repeated trials, red-teaming, trace review, safety validation) and answers whether the agent is good enough to enter deployment and under what constraints. \emph{Online human-oversight cost} is paid after deployment (human review, approval before high-risk actions, escalation handling, auditing, correction, monitoring) and answers how much supervision is required to use the agent safely in production. Offline evaluation determines whether the agent passes the gate, while online oversight determines the cost of employing it afterwards. \Cref{tab:gate} traces this logic across agent quality levels. As quality rises, the agent passes the gate with progressively less oversight, shifting from heavy human review toward exception-based review and lowering the total cost of safe task completion.

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{
    >{\RaggedRight\arraybackslash}p{2.7cm}
    >{\RaggedRight\arraybackslash}p{3.5cm}
    >{\RaggedRight\arraybackslash}p{3.0cm}
    >{\RaggedRight\arraybackslash}X}
\toprule
\textbf{Agent quality} & \textbf{Exam result} & \textbf{Required oversight} & \textbf{Deployment implication} \\
\midrule
Low quality            & Fails gate                     & Not deployable          & No production use \\
\addlinespace
Minimum viable quality & Passes with high oversight     & Heavy human review      & Limited but safe deployment \\
\addlinespace
Improving quality      & Passes with moderate oversight & Confidence-gated review & Scalable supervised deployment \\
\addlinespace
High quality           & Passes with low oversight      & Exception-based review  & High automation ROI \\
\bottomrule
\end{tabularx}
\caption{Agent quality determines the exam result, the required oversight, and the deployment implication. The goal is not to maximize automation but to reduce the \textbf{total cost of safe task completion}. As the agent improves, the human-oversight cost should decline.}
\label{tab:gate}
\end{table}


==> old/sections/04_taxonomy.tex <==
\section{A Multi-Axis Taxonomy for Enterprise Exams}
\label{sec:taxonomy}

A single occupational taxonomy is insufficient, while the three deployment tiers alone are too coarse for coverage planning. Enterprise's First Exam therefore uses a \textbf{multi-axis task taxonomy}. Each task is tagged along seven axes, which together make coverage explicit, comparability possible, and the deployment envelope of each task unambiguous.

\subsection{Axis A: Industry and Professional Context}

This is the benchmark-coverage layer. Each task records its \emph{industry} (healthcare, financial services, life sciences, legal, insurance, retail, manufacturing, government, and others), \emph{function} (finance, compliance, operations, research, customer service, IT, procurement, risk), \emph{role or occupation} (financial analyst, clinical reviewer, claims examiner, procurement manager, compliance officer, and similar), and \emph{workflow family} (due diligence, patient-safety review, prior authorization, contract-leakage detection, claims adjudication, account reconciliation). This axis creates comparability with profession- and occupation-oriented benchmarks while preserving enterprise workflow specificity.

\subsection{Axis B: Work Activity}

Occupation alone is often too broad. A healthcare manager and a financial analyst may both perform investigation, analysis, inspection, record-keeping, and coordination. A cross-industry activity inventory provides a reusable layer between atomic capabilities such as retrieval and overly broad occupational labels: analysis and investigation, inspection and appraisal, advising and design, administration and coordination, procedure execution and troubleshooting, record-keeping, representation and user communication, rule enforcement and emergency response, and creative production.

\subsection{Axis C: Deployment and Autonomy Tier}

This is the primary Enterprise's First Exam axis. \Cref{tab:tiers} defines the three cumulative tiers by their autonomy surface, required end state, and defining risk. Tiers~1--3 are expanded in \cref{sec:tier1,sec:tier2,sec:tier3}.

\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{2.8cm} Z{3.4cm} Z{3.2cm} W}
\toprule
\textbf{Tier} & \textbf{Autonomy surface} & \textbf{Required end state} & \textbf{Defining risk} \\
\midrule
T1: Evidence-Grounded Insight & Read, retrieve, analyze, and synthesize & Reviewable decision-support artifact & Misleading, incomplete, contradicted, or unsupported insight \\
\addlinespace
T2: State-Changing Workflow & Update, submit, route, approve, or trigger & Correct system-of-record state & Incorrect, unauthorized, duplicated, or non-recoverable mutation \\
\addlinespace
T3: Open User-Facing Completion & Converse, clarify, negotiate, and act & Correct task completion with a live or simulated user & Policy violation, manipulation, privacy leakage, or unsafe interaction \\
\bottomrule
\end{tabularx}
\caption{The three cumulative deployment tiers (Axis C).}
\label{tab:tiers}
\end{table}

\subsection{Axis D: Role and Authority}

Every task specifies the agent's role and intended user, the allowed information and data sources, the allowed tools and systems, the decisions the agent may make autonomously, the actions requiring human approval, the actions prohibited entirely, the conditions requiring escalation, and the intended human reviewer or accountable owner. This axis distinguishes Enterprise's First Exam from benchmarks that evaluate only output quality, as a high-quality work product is not sufficient if the agent exceeded its authority.

\subsection{Axis E: Workflow State and Work Product}

Each task identifies where the agent enters the workflow and what it must leave behind. Common workflow stages are $\mathit{draft} \rightarrow \mathit{review} \rightarrow \mathit{revise} \rightarrow \mathit{verify} \rightarrow \mathit{route} \rightarrow \mathit{file} \rightarrow \mathit{commit} \rightarrow \mathit{monitor} \rightarrow \mathit{escalate}$. The scored object is the work product or final system state, not merely a natural-language answer. A report with an evidence trace, an updated enterprise record and state diff, a filed case or submission, a completed appointment or service interaction, or an escalation package usable by the next human owner.

\subsection{Axis F: Consequence and Reversibility}

Not every write carries equal risk. Each task is assigned a deployment-risk class (\cref{tab:risk}) that governs how severely errors are scored and what oversight the deployment profile prescribes.

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{1.4cm} Z{5.6cm} W}
\toprule
\textbf{Class} & \textbf{Description} & \textbf{Example} \\
\midrule
R0 & Informational and easily discarded & Internal research note \\
\addlinespace
R1 & Influences a decision but requires human approval & Due-diligence or patient-safety memo \\
\addlinespace
R2 & Reversible system mutation & Draft CRM update or ticket routing \\
\addlinespace
R3 & Consequential external action & Filing a claim or prior-authorization request \\
\addlinespace
R4 & High-impact or difficult-to-reverse action & Payment, denial, clinical commitment, or legal commitment \\
\bottomrule
\end{tabularx}
\caption{Deployment-risk classes (Axis F).}
\label{tab:risk}
\end{table}

\subsection{Axis G: Reliability Primitives}
\label{sec:primitives}

Each task selects the evaluation primitives that apply. These are the reusable evaluation engines an enterprise should build once and reuse across its agent portfolio:
\begin{enumerate}[leftmargin=1.8em]
  \item \textbf{Outcome correctness and completeness:} did the task reach the correct work product or final state?
  \item \textbf{Evidence grounding and citation support:} does every important claim trace to retrieved evidence, does the evidence genuinely support it, and does the agent distinguish fact, inference, assumption, and speculation?
  \item \textbf{Policy and authority compliance:} does the agent anchor its criteria, thresholds, and conclusions in the authoritative sources that govern the task (regulations, standard operating procedures, professional-society standards, contractual terms, or payer and compliance documents) rather than in recalled training data or a generic default, and does it stay within its granted authority?
  \item \textbf{Calibration, abstention, and escalation:} does the agent know what it does not know, ask for missing information rather than inventing it, and escalate when confidence is low, evidence is contradictory, or the task exceeds its authority? A reliable agent is evaluated not only on answering correctly but on abstaining correctly.
  \item \textbf{Write-operation correctness, recovery, and idempotency:} when the agent changes state, did it perform the correct action on the correct object with the correct values, and does it handle stale data, failed calls, partial completion, retries, and duplicate submissions safely?
  \item \textbf{Interaction and adversarial robustness:} does the agent hold its policy under crafted inputs, resisting prompt injection, jailbreaks, social engineering, and attempts to extract hidden instructions or sensitive data?
  \item \textbf{Auditability and trace completeness:} can a human reconstruct what the agent did, why, and on what evidence, from logged retrievals, tool calls, decisions, writes, and escalations?
  \item \textbf{Repeated-trial reliability:} does the agent succeed consistently across repeated trials, or pass once and fail the next time?
  \item \textbf{Human review effort:} how much reviewer time and correction does the agent's output require?
  \item \textbf{Total cost of safe completion:} the model cost plus the human-oversight cost required to reach a target reliability, formalized in \cref{sec:calibration}.
\end{enumerate}

\subsection{Canonical task record}
\label{sec:taskrecord}

The axes are captured in a versioned task record that pairs a reusable workflow template with concrete, gradeable instances. \Cref{lst:taskrecord} shows an illustrative record for a Tier-1 patient-safety review.

\begin{figure}[ht]
\begin{efecode}
task_id: healthcare.patient_safety.event_review.v1
coverage:
  industry: healthcare
  function: quality_and_safety
  role: patient_safety_reviewer
  work_activities: [investigation, analysis, inspection]
deployment:
  tier: T1
  risk_class: R1
  workflow_stage: draft_for_review
  autonomous_actions: [retrieve_records, construct_timeline, draft_findings]
  prohibited_actions: [amend_patient_record, contact_patient]
  escalation_conditions: [conflicting_medication_records, missing_policy,
                          potential_immediate_harm]
work_product:
  type: patient_safety_review
  required_components: [event_timeline, evidence_citations, policy_mapping,
                        contributing_factors, uncertainty_and_escalation]
evaluation:
  primitives: [outcome_quality, grounding, policy_compliance, calibration,
               auditability, oversight_cost]
  repeated_trials: 3
\end{efecode}
\caption{Illustrative canonical task record spanning the seven taxonomy axes.}
\label{lst:taskrecord}
\end{figure}


==> old/sections/05_headline_metric.tex <==
\section{Headline Metric: The Cost of Reliability}
\label{sec:calibration}

Enterprise readiness is not maximal autonomy, it is the \emph{minimization of the cost of meeting a reliability target}, and it answers the framework's headline question: what is the minimum-cost deployment policy that meets a required reliability level? We formalize this as a selective-prediction problem with deferral to a human, and derive a single per-case economic metric: the model (token) cost plus the human-oversight cost an agent still requires to reach a target reliability, $Y$. We develop the metric here in the Tier-1 setting of a verdict-and-evidence task, but it applies across tiers wherever an autonomous action can be gated behind a confidence threshold, and it is computed at scale by the oversight simulator of \cref{sec:platform}. Its headline form is
\begin{equation}
  C^\star(Y) \;=\; \underbrace{k_m}_{\text{always paid}}
  \;+\; \underbrace{k_h\,e^\star(Y)}_{\text{residual oversight}},
  \label{eq:headline}
\end{equation}
where $k_m$ is the model cost per case, $k_h$ the cost of one human review, and
$e^\star(Y)$ the escalation rate at the cost-optimal operating point derived below.
The all-human baseline reviews every case at cost $k_h$; a useful agent drives
$C^\star(Y)$ below it.

\subsection{Setup and the per-case decision pipeline}

Let the benchmark be a task set $T = \{(x_i, y_i)\}_{i=1}^{N}$ with inputs $x_i$
and gold labels $y_i$. For each case, a model produces a verdict and a scalar
confidence,
\begin{equation}
  m(x) = (\hat{y},\, s), \qquad s \in [0,1].
\end{equation}
This is the only contract the framework requires of the underlying benchmark: a
verdict whose correctness can be scored, and a confidence attached to it. The raw
score $s$ may come from logits, verbalized confidence, or any of the estimators
surveyed above; an optional calibration map $g$ fit on held-out data can produce a
calibrated confidence $g(s) \approx \Pr(\hat{y}=y \mid s)$, but the analysis below
depends only on the \emph{ordering} $s$ induces, not on its absolute values.

Given an escalation threshold $\tau \in [0,1]$, the system acts \emph{autonomously}
when $s \ge \tau$ and \emph{escalates} the case to a human otherwise:
\begin{equation}
  a_\tau(s) \;=\;
  \begin{cases}
    \textsc{autonomous}, & s \ge \tau,\\[2pt]
    \textsc{escalate},   & s < \tau.
  \end{cases}
\end{equation}
A human completes an escalated case with reliability $a_H$\textcolor{red}{AS: I think $a_H$ and $a_\tau$ are different usages of 'a'. We should use a different letter here. }  and review cost $k_h$;
the model incurs cost $k_m$ on \emph{every} case (it runs before we decide to
escalate), so an escalated case costs $k_m + k_h$ in total \textcolor{red}{AS: we should exclusively use either small h or capital H to denote H and not switch the scripts across notations }. We write
$a_0 = \Pr(\hat{y} = y)$ for the model's base (full-coverage) accuracy and assume
$k_h \gg k_m$\textcolor{red}{Here `a` seems to denote some `expectation` over model/system correctness in different autonomy regimes - which is fine but is different from previous definition of `a`. Alternately - perhaps a is just ill-defined earlier and we can add right detail}.

\paragraph{Goal.} For a given model, produce the \emph{cost-of-reliability curve}:
the $x$-axis is a target system reliability $Y$, and the $y$-axis is the minimum
expected cost per case at which the escalating system attains reliability $Y$.

\subsection{Risk--coverage, reliability, and cost}

It is convenient to parametrize by the coverage induced by $\tau$. Define
\begin{align}
  c(\tau)   &= \Pr(s \ge \tau)                          && \text{(coverage / autonomy rate),}\\
  e(\tau)   &= 1 - c(\tau) = \Pr(s < \tau)              && \text{(escalation rate),}\\
  r(c)      &= \Pr(\hat{y} \ne y \mid s \ge \tau)       && \text{(selective risk),}\\
  A_m(c)    &= \Pr(\hat{y} = y \mid s \ge \tau) = 1 - r(c) && \text{(selective accuracy).}
\end{align}
\textcolor{red}{AS: can we just use one term "autonomy rate" which is sufficient. Coverage is confusing.}
Coverage is the fraction of cases the model keeps; selective risk is the error
rate among those kept. Sweeping $\tau$ traces the \emph{risk--coverage curve},
plotted canonically as coverage against selective risk (lower is better). Since
$c$ is monotone in $\tau$, we freely write $r(c)$ and $A_m(c)$, reading the curve
off the top-$c$ fraction of cases ranked by confidence.

Autonomous cases are correct at rate $A_m$ \textcolor{red}{shouldn't this be same as earlier defined $a_0 = \Pr(\hat{y} = y)$}; escalated cases at rate $a_H$. \textcolor{red}{AS: can both correctness labels have same capitaliztion?}The
deployed system's reliability and expected per-case cost are therefore
\begin{align}
  R(c)    &= c\,A_m(c) + (1-c)\,a_H = c\,\bigl(1 - r(c)\bigr) + (1-c)\,a_H,
            \label{eq:reliability}\\
  \mathrm{Cost}(c) &= k_m + k_h\,\bigl(1 - c\bigr),
            \label{eq:cost}
\end{align}

so cost is strictly decreasing in coverage.

\begin{remark}[These identities hold for \emph{any} confidence signal]
Equations \eqref{eq:reliability}--\eqref{eq:cost} are measured quantities; they
are valid regardless of how good the confidence scores are. If the confidence is
uninformative, the risk--coverage curve is simply flat at the base error rate
$1 - a_0$ and escalation buys nothing --- but the identities still describe
reliability and cost correctly. What the quality of the confidence signal
controls is not the \emph{validity} of the analysis but the \emph{shape} of the
curve: how cheaply a given reliability target can be reached. We make this
precise in \cref{sec:oracle,sec:disc}.
\end{remark}

\subsection{The deliverable: the cost-of-reliability curve}

Minimizing cost \eqref{eq:cost} subject to a reliability constraint means \textcolor{red}{AS: maximizing the autonomy rate} using
the \emph{most} coverage (the least escalation) that still meets the target. For a
target $Y$,
\begin{equation}
  c^\star(Y) = \max\{\, c \in [0,1] : R(c) \ge Y \,\},
  \qquad
  C^\star(Y) = k_m + k_h\,\bigl(1 - c^\star(Y)\bigr),
  \label{eq:deliverable}
\end{equation}
and $e^\star(Y) = 1 - c^\star(Y)$ recovers \eqref{eq:headline}. Plotting
$C^\star(Y)$ against $Y$ is the cost-of-reliability curve. Two boundary regimes
bound it:
\begin{itemize}
  \item \textbf{Floor.} If $a_0 = R(1) \ge Y$, the model already meets the target
        at full coverage: $c^\star = 1$ and $C^\star = k_m$ (no escalation).
  \item \textbf{Ceiling.} $Y$ is attainable only up to the maximum of $R$
        (\cref{sec:ceiling}); beyond that the constraint set in
        \eqref{eq:deliverable} is empty.
\end{itemize}
It is convenient to report savings relative to the all-human baseline and the
dimensionless cost ratio $\rho = k_h/k_m$:
\begin{equation}
  S \;=\; k_h - C^\star \;=\; k_h\,c^\star(Y) - k_m,
  \qquad
  \frac{C^\star}{k_m} \;=\; 1 + \rho\,\bigl(1 - c^\star(Y)\bigr).
\end{equation}

\subsection{Ceiling and non-monotonicity}
\label{sec:ceiling}

Escalating a case helps reliability only when the model is less reliable than a
human on it. On the high-confidence cases the model handles \emph{better} than a
human, escalating both lowers reliability and wastes review cost. As a result
$R(c)$ is generally not monotone: as we escalate more, reliability first rises (we
hand off the cases the model gets wrong) and then falls (we start handing off
cases it would have gotten right). This is why the deliverable
\eqref{eq:deliverable} takes the \emph{largest} coverage meeting the target ---
that is the cheapest operating point. The reliability \emph{ceiling} is therefore
not $a_H$: keeping the high-confidence cases, where the model beats the human,
pushes attainable reliability above $a_H$. The best possible value, reached only
by a perfect signal (keep every correct verdict, escalate every wrong one), is
\begin{equation}
  R_{\max} = a_0 + a_H\,(1 - a_0) \;\ge\; a_H .
  \label{eq:ceiling}
\end{equation}
A real model's maximum lies between $a_H$ (uninformative confidence) and
\eqref{eq:ceiling} (perfect confidence).

\begin{lemma}[Perfectly calibrated special case]
\label{lem:mono}
Suppose the confidence is perfectly calibrated, $\Pr(\hat y = y \mid s) = s$, and
the gate escalates the lowest-confidence cases first. Then, writing reliability as
a function of the threshold, $R(\tau)$ is nondecreasing on $[0, a_H]$, since
$\tfrac{dR}{d\tau} = (a_H - \tau)\,f(\tau) \ge 0$ for $\tau \le a_H$. The deliverable
then reduces to the smallest threshold meeting the target,
$\tau^\star = \min\{\tau : R(\tau) \ge Y\}$.
\end{lemma}
\noindent
Intuitively, routing a borderline-confidence case to the more reliable human
raises system reliability until the threshold exceeds the human's own accuracy. The
general (possibly miscalibrated) case of \eqref{eq:deliverable} subsumes this
special case.

\subsection{The oracle floor and the discrimination gap}
\label{sec:oracle}

Suppose we had an \emph{oracle} that could escalate using true correctness rather
than confidence: a genie that knows which verdicts are wrong and escalates exactly
those. Its cost curve is a straight line in the target,
\begin{equation}
  C^\star_{\mathrm{oracle}}(Y)
    = k_m + k_h\,\frac{Y - a_0}{a_H},
  \qquad a_0 \le Y \le a_0 + a_H(1 - a_0).
  \label{eq:oracle-cost}
\end{equation}
This floor depends only on $a_0, a_H, k_m, k_h$ --- \emph{not} on the confidence
scores --- so it is the cheapest any confidence signal could possibly achieve. The
excess of the realized curve over it,
\begin{equation}
  \Delta(Y) = C^\star(Y) - C^\star_{\mathrm{oracle}}(Y) \;\ge\; 0,
\end{equation}
is the dollar cost of imperfect discrimination: a real system escalates its
lowest-confidence cases, only some of which are actually wrong, and wastes human
review on the correct ones it mistakenly defers.

\subsection{Discrimination metrics: AURC and E-AURC}
\label{sec:disc}

The quality of the confidence signal is a property of the \emph{ordering} it
induces, independent of the absolute values: any strictly monotone transformation
of $s$ leaves the ranking --- and hence $r(c)$, the entire risk--coverage curve,
and everything derived from it --- unchanged. It is thus a measure of
\emph{discrimination}, not calibration. The scalar summary is the area under the
(risk) risk--coverage curve,
\begin{equation}
  \mathrm{AURC} = \int_0^1 r(c)\,dc,
  \label{eq:aurc}
\end{equation}
with lower being better. Raw AURC confounds discrimination with base accuracy:
even a perfect ranking cannot drive risk to zero once coverage exceeds $a_0$. The
optimal ranking places all correct verdicts ahead of all incorrect ones, giving
\begin{equation}
  r^\star(c) =
  \begin{cases}
    0, & c \le a_0,\\[2pt]
    1 - \dfrac{a_0}{c}, & c > a_0,
  \end{cases}
  \qquad
  \mathrm{AURC}^\star = \int_{a_0}^{1}\!\Bigl(1 - \tfrac{a_0}{c}\Bigr)dc
    = (1 - a_0) + a_0 \ln a_0 .
\end{equation}
Subtracting this accuracy-determined floor isolates discrimination as the
\emph{excess} AURC,
\begin{equation}
  \text{E-AURC} = \mathrm{AURC} - \mathrm{AURC}^\star \;\ge\; 0,
  \label{eq:eaurc}
\end{equation}
which is zero if and only if the confidence perfectly separates correct from
incorrect verdicts. E-AURC is invariant to the risk-vs-accuracy orientation of the
plot (both curves shift together under $x \mapsto 1-x$); we report it in risk
units.

\begin{remark}[Two views of the same oracle]
The AURC-optimal ranking (correct ahead of incorrect) and the cost oracle of
\cref{sec:oracle} (escalate wrong verdicts first) are the \emph{same} ordering
projected onto different axes: selective risk in the AURC view, and review cost in
the economic view. E-AURC and the cost gap $\Delta(Y)$ are therefore two readings
of the same underlying discrimination deficit --- E-AURC target-agnostic and in
risk units, $\Delta(Y)$ evaluated at the operating point $c^\star(Y)$ and in
dollars. We report the realized $C^\star(Y)$ curve against the oracle floor as the
headline, and E-AURC as the single-number summary of the confidence signal's
discriminative quality.
\end{remark}

\subsection{Closed form under a Beta model}

To instantiate the curve analytically, model the per-case correctness probability
as $p \sim \mathrm{Beta}(\alpha,\beta)$ with mean $\mu = \alpha/(\alpha+\beta) = a_0$
(the base accuracy) and concentration $\nu = \alpha+\beta$ (calibration sharpness).
Under perfect calibration the gate escalates the lowest-$p$ cases first; writing
$I_x(a,b)$ for the regularized incomplete beta function (the $\mathrm{Beta}$ CDF),
the identity $\int_{\tau}^{1} p\,f(p;\alpha,\beta)\,dp = \mu\,(1 - I_\tau(\alpha+1,\beta))$
gives the closed forms
\begin{align}
  e(\tau) &= I_\tau(\alpha,\beta), \\
  R(\tau) &= \mu\,\bigl(1 - I_\tau(\alpha+1,\beta)\bigr) + a_H\,I_\tau(\alpha,\beta).
\end{align}
The resulting cost-of-reliability curve is convex and diverges as $Y \to a_H$; a
stronger, better-calibrated model (mass of $p$ concentrated near $1$) attains the
same $Y$ with smaller escalation, shifting its curve downward. This quantifies the
framework's central claim: \emph{as agent quality improves, the human-oversight
cost required for a fixed reliability target declines}.

\subsection{Empirical instantiation on PSEBench}
\label{sec:econ-pse}

We instantiate the model directly from measured benchmark results, using
PSEBench's 15-model leaderboard. PSEBench is a Tier-1 patient-safety-event review
benchmark; its leaderboard reports, per model, a verdict accuracy $M_1$ and an
uncertainty-detection $F_1$ score $M_7$ that quantifies how well the model
recognizes the cases it should escalate. We map these to the two ingredients the
cost model needs: $M_1$ fixes the base accuracy and $M_7$ fixes the
\emph{calibration quality} that governs how efficiently the model can defer.

Concretely, we draw per-case correctness $p \sim \mathrm{Beta}(\mu, \nu_0)$ with
$\mu = M_1$ and a fixed difficulty spread $\nu_0 = 8$. A perfectly calibrated agent
($q=1$) escalates its lowest-$p$ cases first, recovering the optimal gate
$R_{\mathrm{opt}}$ above; an uncalibrated agent ($q=0$) escalates at random,
$R_{\mathrm{rand}}(e) = (1-e)\mu + a_H e$. Setting the calibration quality to the
measured $q = M_7$ interpolates the two:
\begin{equation}
  R_q(e) = q\,R_{\mathrm{opt}}(e) + (1-q)\,R_{\mathrm{rand}}(e),
  \qquad e^\star = \min\{\,e : R_q(e) \ge Y\,\}.
  \label{eq:rq}
\end{equation}
Per-case token cost is computed from a shared PSEBench profile, roughly $6{,}000$
input tokens plus $4{,}000$ output tokens for reasoning models ($1{,}500$
otherwise), priced at each model's tier. Anthropic rates are list prices; OpenAI,
Google, open-weight, and medical-specialty rates are representative current
per-tier rates. We take the human reviewer accuracy $a_H = 0.99$ and review cost
$k_h = \$25$ per escalated case ($\approx$18 minutes of a patient-safety expert).

\begin{figure}[t]
  \centering
  \input{figures/cost-reliability-figure}
  \caption{Total cost per case versus target reliability $Y$ for representative
    PSEBench models ($a_H=0.99$, $k_h=\$25$). Cost rises convexly with the target
    and converges to the all-human baseline as $Y \to a_H$. GPT-5.5 and GPT-5 have
    identical token cost, yet GPT-5's collapsed uncertainty calibration
    ($M_7=12.8$ vs.\ $79.7$) forces far more escalation and a much higher curve.}
  \label{fig:cost}
\end{figure}

\begin{table}[t]
  \centering
  \small
  \input{pse-results}
  \caption{PSEBench economic results. \emph{Token \$/case} is the per-case
    inference cost at the shared token profile; \emph{esc.}\ is the escalation rate
    at the cost-optimal gate \eqref{eq:rq}; \emph{\$/case} is the total
    $\mathrm{Cost} = k_m + k_h\,e^\star$ at $k_h=\$25$. The all-human baseline
    is $\$25$/case.}
  \label{tab:pse-econ}
\end{table}

Three results stand out (\cref{tab:pse-econ,fig:cost})

\textcolor{red}{AS: Aren't points 1 and 2 the same points?}
\begin{enumerate}
  \item \textbf{Token cost is a rounding error.} Per-case inference cost spans
    only \$0.000--\$0.130 across all 15 models, at most $0.5\%$ of a \$25 human
    review. Per-token price is therefore not the operative economic variable, and
    the 40$\times$ spread in token rates barely perturbs the total.
  \item \textbf{The cost driver is escalation rate (i.e.\ accuracy and
    calibration).} GPT-5.5 and GPT-5 have \emph{identical} token cost (\$0.048), yet
    at $Y=98\%$ they cost \$7.45 and \$21.80 per case. The gap is entirely
    GPT-5's collapsed uncertainty awareness ($M_7$: $12.8$ vs.\ $79.7$), which
    forces it to escalate $87\%$ of cases rather than $30\%$. The leaderboard's
    $M_1$ and $M_7$ columns translate directly into dollars.
  \item \textbf{The human ceiling binds near the target.} As $Y \to a_H = 0.99$
    every model is pushed toward escalating everything; at $Y=98\%$ only the
    strongest few (Gemini 3.1 Pro, GPT-5.5, Claude Opus 4.7) stay materially below
    the all-human baseline, while the rest cluster at \$22--\$24. Relaxing the
    target to $95\%$ opens the frontier models dramatically: Gemini 3.1 Pro, whose
    $95.3\%$ base accuracy already clears the bar, needs \emph{zero} escalation at
    \$0.05/case. That gap is the measurable price of the reliability one demands.
\end{enumerate}

\paragraph{Calibration and the escalate class.}
Two error types govern the cost. \emph{Under-escalation}, a confident, incorrect
verdict on a case that should have been deferred (the \textsc{Escalate} /
\textsc{Uncertain} class), is a reliability failure that forces the gate upward and
raises cost globally. \emph{Over-escalation}, deferring cases the agent would have
answered correctly, is wasted human cost. Good calibration collapses both:
genuinely insufficient-evidence cases receive low confidence and route to a human
through the same gate. Calibration error $\varepsilon$ (e.g.\ expected calibration
error) acts as a safety margin: the operator must inflate the threshold to
$\tau^\star + \delta(\varepsilon)$ to remain robust, and that margin carries a
measurable price in additional escalation.

\subsection{Reliability curves on CliniCARE-Bench}
\label{sec:clinicare-reliability}

We use CliniCARE-Bench, our companion clinical-audit benchmark, to measure whether a model's self-reported confidence can guide escalation to human review. For each example, we record whether the predicted label matches the ground-truth label and extract the model's reported confidence. We then sort examples by confidence and vary the fraction handled autonomously. At coverage, $c$, selective risk, $r(c)$ is the error rate among the retained examples. This does not require fitting a calibration map, as the risk--coverage curve depends only on the ordering of confidence scores and is unchanged by any monotonic transformation. For tied confidence values, we use the tied group's mean correctness to avoid dependence on arbitrary within-tie ordering. We summarize each curve by its AURC \eqref{eq:aurc} and, subtracting the optimal-ranking floor $\mathrm{AURC}^\star = (1-a_0) + a_0 \ln a_0$, by its E-AURC \eqref{eq:eaurc}. Translating to cost via \eqref{eq:reliability} and \eqref{eq:cost} with $a_H = 0.99$ and $k_h = \$25$, we select, for a target reliability $Y$, the largest coverage satisfying $R(c) \ge Y$, which minimizes human-review cost.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{clinicare_bench_initial_conf.png}
    \caption{
        Preliminary CliniCARE-Bench cost-of-reliability and risk--coverage curves,
        assuming human-review accuracy $a_H=0.99$ and cost $k_h=\$25$ per case.
        These curves are computed on an early version of the task set and are
        intended to illustrate the methodology rather than to rank systems.
    }
    \label{fig:clinicare-reliability}
\end{figure}

\Cref{fig:clinicare-reliability} shows preliminary results. Among the systems
evaluated, the lowest E-AURC is $0.23$, followed by $0.27$, $0.28$, and $0.29$. One system's curve is nearly flat because it emits only four distinct confidence values and assigns $100\%$ confidence to most answers. Its current confidence output therefore provides little useful information for escalation, although this may be improved through prompting. For some policies, the highest-confidence subset also carries higher risk than the subset at roughly $20$--$30\%$ coverage, which may reflect poor confidence ranking, finite-sample noise, or residual task/label discrepancies in this early task set. The pattern nonetheless demonstrates that a model's confidence ordering, not its token price, determines how cheaply a clinical-audit agent can meet a target reliability.


==> old/sections/05_headline_metric_clean.tex <==
\section{Headline Metric: The Cost of Reliability}
\label{sec:calibration}

\emily{The headline metric is a Tier-1 special case, not yet a general enterprise metric.
The current formulation assumes: one final verdict; a gold correctness label; one scalar confidence score; one accept-or-defer decision;
a fixed-cost human who independently completes the case; symmetric errors summarized by accuracy. That works for a verdict-and-evidence task. It does not directly cover: multi-step workflow writes; multiple escalation points; partial human approval rather than complete handoff; different costs and harms for different actions; reversible versus irreversible failures; human verification of an existing artifact; interactive tasks where the state evolves during the conversation. we need someone to think about how to extend our formulation to handle it. or we can simply point out in the future work. }

Enterprise readiness is not maximal autonomy but the minimum-cost deployment policy
that attains a required reliability level $Y$. We formalize this as a selective-prediction problem
with deferral to a human and derive a single per-case economic metric, the model
(token) cost plus the human-oversight cost an agent still requires to reach $Y$. We
develop the metric in the Tier-1 setting of a verdict-and-evidence task, but it
applies across tiers wherever an autonomous action can be gated behind a confidence
threshold, and it is computed at scale by the oversight simulator of
\cref{sec:platform}. Its headline form is
\begin{equation}
  C^\star(Y) \;=\; \underbrace{k_m}_{\text{always paid}}
  \;+\; \underbrace{k_h\,e^\star(Y)}_{\text{residual oversight}},
  \label{eq:headline}
\end{equation}
where $k_m$ is the model cost per case, $k_h$ the cost of one human review, and
$e^\star(Y)$ the escalation rate at the cost-optimal operating point derived below.
The all-human baseline reviews every case at cost $k_h$; a useful agent drives
$C^\star(Y)$ below it.

\subsection{Setup and the per-case decision pipeline}

Let the benchmark be a task set $T = \{(x_i, y_i)\}_{i=1}^{N}$ with inputs $x_i$
and gold labels $y_i$. For each case, a model produces a verdict and a scalar
confidence,
\begin{equation}
  m(x) = (\hat{y},\, s), \qquad s \in [0,1].
\end{equation}
This is the only contract the framework requires of the underlying benchmark: a
verdict whose correctness can be scored, and a confidence attached to it. The raw
score $s$ may come from logits, verbalized confidence, or any of the estimators
surveyed above; an optional calibration map $g$ fit on held-out data can produce a
calibrated confidence $g(s) \approx \Pr(\hat{y}=y \mid s)$, but the analysis below
depends only on the \emph{ordering} that $s$ induces, not on its absolute values.

The deployment policy is a single threshold $\tau \in [0,1]$ on this confidence: the
system acts \emph{autonomously} when $s \ge \tau$ and \emph{escalates} the case to a
human when $s < \tau$. Everything below depends on $\tau$ only through the induced
autonomy rate $c(\tau) = \Pr(s \ge \tau)$, so we work directly with $c$.
A human completes an escalated case with accuracy $a_h$ and review cost $k_h$;
the model incurs cost $k_m$ on \emph{every} case, since it runs before we decide
to escalate, so an escalated case costs $k_m + k_h$ in total. We write
$a_0 = \Pr(\hat{y} = y)$ for the model's base (full-autonomy) accuracy and assume
$k_h \gg k_m$.

\paragraph{Goal.} For a given model, produce the \emph{cost-of-reliability curve}:
the $x$-axis is a target system reliability $Y$, and the $y$-axis is the minimum
expected cost per case at which the escalating system attains reliability $Y$.

\subsection{Autonomy, reliability, and cost}

We parametrize by the autonomy rate induced by $\tau$. Define
\begin{align}
  c(\tau)   &= \Pr(s \ge \tau)                          && \text{(autonomy rate),}\\
  e(\tau)   &= 1 - c(\tau) = \Pr(s < \tau)              && \text{(escalation rate),}\\
  r(c)      &= \Pr(\hat{y} \ne y \mid s \ge \tau)       && \text{(selective risk),}\\
  a(c)      &= \Pr(\hat{y} = y \mid s \ge \tau) = 1 - r(c) && \text{(selective accuracy).}
\end{align}
The autonomy rate $c$ is the fraction of cases the model handles itself; selective
risk is the error rate among those cases. Sweeping $\tau$ traces the
\emph{risk--autonomy curve}. Since $c$ is monotone in $\tau$, we freely write
$r(c)$ and $a(c)$, reading the curve off the top-$c$ fraction of cases ranked by
confidence. Selective accuracy is a function of the autonomy rate: at full autonomy
the system keeps every case, so $a(1) = a_0$; escalation trades away autonomy for
the chance to raise accuracy on the cases that remain.

Autonomous cases are correct at rate $a(c)$ and escalated cases at rate $a_h$. The
deployed system's reliability and expected per-case cost are therefore
\begin{align}
  R(c)    &= c\,a(c) + (1-c)\,a_h = c\,\bigl(1 - r(c)\bigr) + (1-c)\,a_h,
            \label{eq:reliability}\\
  \mathrm{Cost}(c) &= k_m + k_h\,\bigl(1 - c\bigr),
            \label{eq:cost}
\end{align}
so cost is strictly decreasing in the autonomy rate. We treat the human accuracy
$a_h$ as constant across escalated cases. This is a simplification: escalation
routes the hardest, lowest-confidence cases to the human, on which a reviewer may be
less accurate than on average, so $R(c)$ and the ceiling below are mildly optimistic.
Replacing $a_h$ with a case-dependent $a_h(c)$ leaves every identity that follows
unchanged in form.

\begin{remark}[These identities hold for \emph{any} confidence signal]
Equations \eqref{eq:reliability}--\eqref{eq:cost} are measured quantities; they
are valid regardless of how good the confidence scores are. If the confidence is
uninformative, the risk--autonomy curve is flat at the base error rate $1 - a_0$
and escalation buys nothing, yet the identities still describe reliability and cost
correctly. What the quality of the confidence signal controls is not the
\emph{validity} of the analysis but the \emph{shape} of the curve: how cheaply a
given reliability target can be reached, as quantified in
\cref{sec:oracle,sec:disc}.
\end{remark}

\subsection{The deliverable: the cost-of-reliability curve}

Minimizing cost \eqref{eq:cost} subject to a reliability constraint is exactly
\emph{maximizing the autonomy rate} that still meets the target, since less
escalation means lower cost. For a target $Y$,
\begin{equation}
  c^\star(Y) = \max\{\, c \in [0,1] : R(c) \ge Y \,\},
  \qquad
  C^\star(Y) = k_m + k_h\,\bigl(1 - c^\star(Y)\bigr),
  \label{eq:deliverable}
\end{equation}
and $e^\star(Y) = 1 - c^\star(Y)$ recovers \eqref{eq:headline}. Plotting
$C^\star(Y)$ against $Y$ gives the cost-of-reliability curve. Two boundary regimes
bound it:
\begin{itemize}
  \item \textbf{Floor.} If $a_0 = R(1) \ge Y$, the model already meets the target
        at full autonomy: $c^\star = 1$ and $C^\star = k_m$ (no escalation).
  \item \textbf{Ceiling.} $Y$ is attainable only up to the maximum of $R$
        (\cref{sec:ceiling}); beyond that the constraint set in
        \eqref{eq:deliverable} is empty.
\end{itemize}
We report savings relative to the all-human baseline and the dimensionless cost
ratio $\rho = k_h/k_m$:
\begin{equation}
  S \;=\; k_h - C^\star \;=\; k_h\,c^\star(Y) - k_m,
  \qquad
  \frac{C^\star}{k_m} \;=\; 1 + \rho\,\bigl(1 - c^\star(Y)\bigr).
\end{equation}

\subsection{Ceiling and non-monotonicity}
\label{sec:ceiling}

Escalating a case helps reliability only when the model is less reliable than a
human on it. On the high-confidence cases the model handles \emph{better} than a
human, escalating both lowers reliability and wastes review cost. As a result
$R(c)$ is generally not monotone: as we escalate more, reliability first rises (we
hand off the cases the model gets wrong) and then falls (we start handing off cases
it would have gotten right). This is why the deliverable \eqref{eq:deliverable}
takes the \emph{largest} autonomy rate meeting the target, which is the cheapest
operating point. The reliability \emph{ceiling} is therefore not $a_h$: keeping the
high-confidence cases, where the model beats the human, pushes attainable
reliability above $a_h$. The best possible value, reached only by a perfect signal
that keeps every correct verdict and escalates every wrong one, is
\begin{equation}
  R_{\max} = a_0 + a_h\,(1 - a_0) \;\ge\; a_h .
  \label{eq:ceiling}
\end{equation}
A real model's maximum lies between $a_h$ (uninformative confidence) and
\eqref{eq:ceiling} (perfect confidence).

\begin{lemma}[Perfectly calibrated special case]
\label{lem:mono}
Suppose the confidence is perfectly calibrated, $\Pr(\hat y = y \mid s) = s$, and
the policy escalates the lowest-confidence cases first. Then, writing reliability as
a function of the threshold, $R(\tau)$ is nondecreasing on $[0, a_h]$, since
$\tfrac{dR}{d\tau} = (a_h - \tau)\,f(\tau) \ge 0$ for $\tau \le a_h$. The deliverable
then reduces to the smallest threshold meeting the target,
$\tau^\star = \min\{\tau : R(\tau) \ge Y\}$.
\end{lemma}
\noindent
Routing a borderline-confidence case to the more reliable human raises system
reliability until the threshold exceeds the human's own accuracy. The general
(possibly miscalibrated) case of \eqref{eq:deliverable} subsumes this special case.

\subsection{The oracle floor and the discrimination gap}
\label{sec:oracle}

Suppose an \emph{oracle} could escalate using true correctness rather than
confidence, deferring exactly the verdicts that are wrong. Its cost curve is a
straight line in the target,
\begin{equation}
  C^\star_{\mathrm{oracle}}(Y)
    = k_m + k_h\,\frac{Y - a_0}{a_h},
  \qquad a_0 \le Y \le a_0 + a_h(1 - a_0).
  \label{eq:oracle-cost}
\end{equation}
This floor depends only on $a_0, a_h, k_m, k_h$, not on the confidence scores, so it
is the cheapest that any confidence signal could achieve. The excess of the realized
curve over it,
\begin{equation}
  \Delta(Y) = C^\star(Y) - C^\star_{\mathrm{oracle}}(Y) \;\ge\; 0,
\end{equation}
is the dollar cost of imperfect discrimination: a real system escalates its
lowest-confidence cases, only some of which are actually wrong, and wastes human
review on the correct ones it mistakenly defers.

\subsection{Discrimination metrics: AURC and E-AURC}
\label{sec:disc}

The quality of the confidence signal is a property of the \emph{ordering} it
induces, independent of the absolute values: any strictly monotone transformation
of $s$ leaves the ranking unchanged, and hence leaves $r(c)$, the entire
risk--autonomy curve, and everything derived from it unchanged. It is thus a measure
of \emph{discrimination}, not calibration. The scalar summary is the area under the
risk--autonomy curve (the classical risk--coverage curve, hence the acronym AURC),
\begin{equation}
  \mathrm{AURC} = \int_0^1 r(c)\,dc,
  \label{eq:aurc}
\end{equation}
with lower being better. Raw AURC confounds discrimination with base accuracy: even
a perfect ranking cannot drive risk to zero once the autonomy rate exceeds $a_0$. The
optimal ranking places all correct verdicts ahead of all incorrect ones, giving
\begin{equation}
  r^\star(c) =
  \begin{cases}
    0, & c \le a_0,\\[2pt]
    1 - \dfrac{a_0}{c}, & c > a_0,
  \end{cases}
  \qquad
  \mathrm{AURC}^\star = \int_{a_0}^{1}\!\Bigl(1 - \tfrac{a_0}{c}\Bigr)dc
    = (1 - a_0) + a_0 \ln a_0 .
\end{equation}
Subtracting this accuracy-determined floor isolates discrimination as the
\emph{excess} AURC,
\begin{equation}
  \text{E-AURC} = \mathrm{AURC} - \mathrm{AURC}^\star \;\ge\; 0,
  \label{eq:eaurc}
\end{equation}
which is zero if and only if the confidence perfectly separates correct from
incorrect verdicts. E-AURC is invariant to the risk-vs-accuracy orientation of the
plot (both curves shift together under $x \mapsto 1-x$); we report it in risk units.

\begin{remark}
The AURC-optimal ranking (correct ahead of incorrect) and the cost oracle of
\cref{sec:oracle} (escalate wrong verdicts first) are the \emph{same} ordering
projected onto different axes: selective risk in the discrimination view, and review
cost in the economic view. E-AURC and the cost gap $\Delta(Y)$ are therefore two
readings of the same discrimination deficit: E-AURC is target-agnostic and in risk
units, while $\Delta(Y)$ is evaluated at the operating point $c^\star(Y)$ and in
dollars. We report the realized $C^\star(Y)$ curve against the oracle floor as the
headline, and E-AURC as the single-number summary of the confidence signal's
discriminative quality.
\end{remark}

\subsection{Closed form under a Beta model}

To instantiate the curve analytically, model the per-case correctness probability
as $p \sim \mathrm{Beta}(\alpha,\beta)$. We use the mean-and-concentration
parametrization $\mathrm{Beta}(\mu,\nu)$, with mean $\mu = \alpha/(\alpha+\beta) = a_0$
(the base accuracy) and concentration $\nu = \alpha+\beta$ (the spread of per-case
difficulty), so that $\alpha = \mu\nu$ and $\beta = (1-\mu)\nu$. Under perfect
calibration the policy escalates the lowest-$p$ cases first; writing $I_x(a,b)$ for
the regularized incomplete beta function (the $\mathrm{Beta}$ CDF), the identity
$\int_{\tau}^{1} p\,f(p;\alpha,\beta)\,dp = \mu\,(1 - I_\tau(\alpha+1,\beta))$
gives the closed forms
\begin{align}
  e(\tau) &= I_\tau(\alpha,\beta), \\
  R(\tau) &= \mu\,\bigl(1 - I_\tau(\alpha+1,\beta)\bigr) + a_h\,I_\tau(\alpha,\beta).
\end{align}
The resulting cost-of-reliability curve is convex, and its slope grows without bound
as $Y$ approaches the model's attainable ceiling $\sup_c R(c)$ (at most
$R_{\max} = a_0 + a_h(1 - a_0)$), beyond which the target is infeasible; the cost
itself stays bounded by the all-human baseline $k_m + k_h$. A stronger model, with
more of the mass of $p$ near $1$, attains the same $Y$ with smaller escalation,
shifting its curve downward. Hence, as agent quality improves, the human-oversight
cost required for a fixed reliability target declines.

\subsection{Empirical instantiation on PSEBench}
\label{sec:econ-pse}

We instantiate the model directly from measured benchmark results, using PSEBench's
15-model leaderboard. PSEBench is a Tier-1 patient-safety-event review benchmark;
its leaderboard reports, per model, a verdict accuracy $M_1$ and an
uncertainty-detection $F_1$ score $M_7$ (both on a $0$--$100$ scale) that quantifies
how well the model recognizes the cases it should escalate. We map these to the two
ingredients the cost model needs: $M_1$ fixes the base accuracy, and we use the
uncertainty-detection $F_1$ as the \emph{calibration-quality} proxy $q = M_7/100$
that governs how efficiently the model can defer.

Concretely, we draw per-case correctness $p \sim \mathrm{Beta}(\mu, \nu_0)$ with
mean $\mu = M_1/100$ and a fixed difficulty spread $\nu_0 = 8$. A perfectly
calibrated agent ($q=1$) escalates its lowest-$p$ cases first, recovering the
perfectly-calibrated Beta gate above; expressed as a function of the escalation
rate $e$, we denote it $R_{\mathrm{opt}}(e)$. An uncalibrated agent ($q=0$)
escalates at random, $R_{\mathrm{rand}}(e) = (1-e)\mu + a_h e$. Setting the
calibration quality to the measured $q = M_7/100 \in [0,1]$ interpolates the two:
\begin{equation}
  R_q(e) = q\,R_{\mathrm{opt}}(e) + (1-q)\,R_{\mathrm{rand}}(e),
  \qquad e^\star = \min\{\,e : R_q(e) \ge Y\,\}.
  \label{eq:rq}
\end{equation}
The linear interpolation in \eqref{eq:rq} is a modeling choice, not a derived
identity: it is a one-parameter dial that reproduces the two endpoints ($q=1$
perfectly calibrated, $q=0$ uninformative) and reads $q$ off the leaderboard's
uncertainty-detection score, rather than a claim that real calibration mixes the two
gates exactly.
Per-case token cost is computed from a shared PSEBench profile, roughly $6{,}000$
input tokens plus $4{,}000$ output tokens for reasoning models ($1{,}500$
otherwise), priced at each model's tier. Anthropic rates are list prices; OpenAI,
Google, open-weight, and medical-specialty rates are representative current per-tier
rates. We take the human reviewer accuracy $a_h = 0.99$ and review cost
$k_h = \$25$ per escalated case ($\approx$18 minutes of a patient-safety expert).

\begin{figure}[t]
  \centering
  \input{figures/cost-reliability-figure}
  \caption{Total cost per case versus target reliability $Y$ for representative
    PSEBench models ($a_h=0.99$, $k_h=\$25$). Cost rises convexly with the target
    and climbs toward the all-human baseline as $Y$ approaches the model's
    reliability ceiling. GPT-5.5 and GPT-5 have
    identical token cost, yet GPT-5's collapsed uncertainty calibration
    ($M_7=12.8$ vs.\ $79.7$) forces far more escalation and a much higher curve.}
  \label{fig:cost}
\end{figure}

\begin{table}[t]
  \centering
  \small
  \input{pse-results}
  \caption{PSEBench economic results. \emph{Token \$/case} is the per-case
    inference cost at the shared token profile; \emph{esc.}\ is the escalation rate
    at the cost-optimal gate \eqref{eq:rq}; \emph{\$/case} is the total
    $\mathrm{Cost} = k_m + k_h\,e^\star$ at $k_h=\$25$. The all-human baseline
    is $\$25$/case.}
  \label{tab:pse-econ}
\end{table}

Three results follow (\cref{tab:pse-econ,fig:cost}).
\begin{enumerate}
  \item \textbf{The economic variable is human review, not tokens.} Per-case
    inference cost spans only \$0.000--\$0.130 across all 15 models, at most about
    $0.5\%$ of a \$25 human review. The roughly $40\times$ spread in per-token
    prices barely perturbs the total.
  \item \textbf{The bill is set by the escalation rate, which depends on both base
    accuracy and calibration quality.} GPT-5.5 and GPT-5 have \emph{identical} token
    cost (\$0.048), yet at $Y=98\%$ they cost \$7.45 and \$21.80 per case. The gap
    is driven by GPT-5's collapsed uncertainty calibration ($M_7$: $12.8$ vs.\
    $79.7$), which forces it to escalate about $87\%$ of cases rather than $30\%$.
    A model needs both a high $M_1$ and a high $M_7$ to escalate little; neither
    alone suffices, and the two leaderboard columns jointly fix the cost.
  \item \textbf{The human ceiling binds near the target.} As $Y \to a_h = 0.99$
    every model is pushed toward escalating everything, and at $Y=98\%$ only the
    strongest few (Gemini 3.1 Pro, GPT-5.5, Claude Opus 4.7) stay materially below
    the all-human baseline while the rest cluster at \$22--\$24. Relaxing the target
    from $98\%$ to $95\%$ brings the frontier models well below the all-human
    baseline: Gemini 3.1 Pro, whose $95.3\%$ base accuracy already clears the bar,
    needs \emph{zero} escalation at about \$0.05/case.
\end{enumerate}

\paragraph{Calibration and the escalate class.}
Two error types govern the cost. \emph{Under-escalation}, a confident and incorrect
verdict on a case that should have been deferred (the \textsc{Escalate} /
\textsc{Uncertain} class), is a reliability failure that forces the gate upward and
raises cost globally. \emph{Over-escalation}, deferring cases the agent would have
answered correctly, is wasted human cost. Good calibration collapses both:
genuinely insufficient-evidence cases receive low confidence and route to a human
through the same gate. Calibration error $\varepsilon$ (for example, expected
calibration error) acts as a safety margin: the operator must inflate the threshold
to $\tau^\star + \delta(\varepsilon)$ to stay robust, which adds escalation and thus
cost.

\subsection{Reliability curves on CliniCARE-Bench}
\label{sec:clinicare-reliability}

We use CliniCARE-Bench, our companion clinical-audit benchmark, to measure whether a
model's self-reported confidence can guide escalation to human review. For each
example, we record whether the predicted label matches the ground-truth label and
extract the model's reported confidence. We then sort examples by confidence and vary
the fraction handled autonomously. At autonomy rate $c$, selective risk $r(c)$ is the
error rate among the retained examples. This does not require fitting a calibration
map, as the risk--autonomy curve depends only on the ordering of confidence scores
and is unchanged by any monotonic transformation. For tied confidence values, we use
the tied group's mean correctness to avoid dependence on arbitrary within-tie
ordering. We summarize each curve by its AURC \eqref{eq:aurc} and, subtracting the
optimal-ranking floor $\mathrm{AURC}^\star = (1-a_0) + a_0 \ln a_0$, by its E-AURC
\eqref{eq:eaurc}. Translating to cost via \eqref{eq:reliability} and \eqref{eq:cost}
with $a_h = 0.99$ and $k_h = \$25$, we select, for a target reliability $Y$, the
largest autonomy rate satisfying $R(c) \ge Y$, which minimizes human-review cost.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{clinicare_bench_initial_conf.png}
    \caption{
        Preliminary CliniCARE-Bench cost-of-reliability and risk--autonomy curves,
        assuming human-review accuracy $a_h=0.99$ and cost $k_h=\$25$ per case.
        These curves are computed on an early version of the task set and are
        intended to illustrate the methodology rather than to rank systems.
    }
    \label{fig:clinicare-reliability}
\end{figure}

\Cref{fig:clinicare-reliability} shows preliminary results. Among the systems
evaluated, the lowest E-AURC is $0.23$, followed by $0.27$, $0.28$, and $0.29$. One
system's curve is nearly flat because it emits only four distinct confidence values
and assigns $100\%$ confidence to most answers; its current confidence output
therefore provides little useful information for escalation. For some policies, the highest-confidence subset also
carries higher risk than the subset at roughly $20$--$30\%$ autonomy, which may
reflect poor confidence ranking, finite-sample noise, or residual task/label
discrepancies in this early task set. The pattern nonetheless demonstrates that a
model's confidence ordering, not its token price, determines how cheaply a
clinical-audit agent can meet a target reliability.


==> old/sections/06_tier1.tex <==
\section{Tier 1: Evidence-Grounded Insight Agents}
\label{sec:tier1}

\subsection{Definition and core evaluation question}

Tier 1 agents are read-only agents. They search, retrieve, analyze, and synthesize fragmented enterprise information across documents, tables, APIs, spreadsheets, images, PDFs, logs, tickets, databases, and external sources, returning insights that supports a decision without changing the state of any system. This is the safest tier to deploy and the natural starting point for many enterprise agent programs. The worst-case failure is usually a wrong or incomplete insight a human reviewer can still catch before acting. Representative types include due-diligence, patient-safety event review, competitive and market intelligence, equity and credit research, regulatory and compliance monitoring, clinical evidence synthesis, contract and legal review, and supply-chain risk agents. The core question is: \emph{can the agent produce a trustworthy, evidence-grounded, decision-useful artifact from fragmented enterprise context?} The economic reliability metric of \cref{sec:calibration} was developed on exactly this setting.

\subsection{Evaluation criteria}

\paragraph{Insight grounding.} Every important conclusion should be traceable to evidence that genuinely supports it. Two failure modes are especially important: \emph{fabricated support} (the agent cites a source that does not say what it claims) and \emph{unsupported synthesis} (the agent draws a conclusion no source backs). Metrics include claim-level citation precision and recall, evidence sufficiency, unsupported- and contradicted-claim rates, source relevance, and correct handling of conflicting evidence.

\paragraph{Insight quality.} Research questions rarely have a single gold answer, so the output is evaluated against expert rubrics rather than exact match: completeness, factual accuracy, depth of analysis, decision relevance, risk prioritization, clarity of recommendations, and explicit assumptions and limitations.

\paragraph{Proactive information seeking.} A strong agent recognizes missing information and fills the gap rather than papering over it with plausible language: missing-information detection, correct follow-up question generation, appropriate tool or source selection, and avoidance of unsupported inference.

\paragraph{Escalation and abstention.} When the agent cannot verify a claim, faces genuine ambiguity, or lacks sufficient information, the correct behavior is to flag the issue for human review: abstention recall, over-abstention, escalation-rationale quality, low-confidence detection, and ambiguity handling. A calibrated agent earns trust by escalating the right cases.

\subsection{Relevant benchmark families}

Tier 1 is closest to deep research, retrieval-augmented generation, browsing, and evidence-synthesis benchmarks. Representative benchmarks include:

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{3.2cm} W Z{4.2cm}}
\toprule
\textbf{Benchmark} & \textbf{What it measures} & \textbf{Relevance} \\
\midrule
DeepResearch Bench \citep{deepresearchbench} & Long-form research report quality and citation-grounded synthesis & Direct analogue for insight quality and grounding \\
\addlinespace
DeepResearch Bench II \citep{deepresearchbench2} & Fine-grained rubric-based evaluation of expert-style reports & Useful for evaluating recall, analysis, and presentation \\
\addlinespace
DRBench \citep{drbench} & Enterprise deep research over public and private company context & Strong fit for enterprise read-only research \\
\addlinespace
BrowseComp \citep{browsecomp} & Persistent browsing and retrieval on verifiable hard-to-find answers & Tests search persistence and source discrimination \\
\addlinespace
MMDeepResearch-Bench \citep{mmdeepresearchbench} & Multimodal report generation and citation-grounded visual evidence use & Relevant when enterprise inputs include charts, images, and PDFs \\
\addlinespace
AbstentionBench \citep{abstentionbench} & Selective abstention on unanswerable, underspecified, ambiguous, or outdated queries & Direct analogue for escalation and uncertainty handling \\
\addlinespace
GAIA \citep{gaia} / FRAMES \citep{frames} & Multi-hop reasoning, tool use, retrieval, and synthesis & Useful for general evidence-seeking ability \\
\bottomrule
\end{tabularx}
\end{table}

Tier 1 establishes the foundation for enterprise trust: the agent must produce grounded insight before it is allowed to act.


==> old/sections/07_tier2.tex <==
\section{Tier 2: State-Changing Workflow Agents}
\label{sec:tier2}

\subsection{Definition and core evaluation question}

Tier 2 agents do everything Tier 1 agents do, then commit an action written back into an enterprise workflow system: they may update a record, create a ticket, resolve a case, file a submission, generate a quote, route an approval, or trigger a downstream process. The defining shift is consequence: a wrong insight in Tier 1 is recoverable because a human still stands between the agent and the system of record, whereas a wrong write in Tier 2 has already changed the world. Representative types include case and ticket resolution, CRM and CPQ update, IT service-management automation, claims-adjudication write-back, prior-authorization submission, procurement and supply-chain action, and finance close and reconciliation agents. The core question is: \emph{can the agent safely and correctly complete workflow actions in enterprise systems of record?} Tier 2 inherits all Tier 1 criteria---the reasoning preceding the write must still be grounded, complete, calibrated, and reviewable.

\subsection{Additional evaluation criteria}

\paragraph{Write-operation correctness.} The agent must perform the correct action on the correct object with the correct values; final text output is insufficient, so the benchmark inspects the final system state. Metrics include correct record selection, field update, workflow transition, and evidence association; duplicate-action and wrong-object mutation rates; and final-state match against expected state.

\paragraph{Reversibility and blast radius.} Not all writes are equal (Axis F): a reversible field update is lower risk than a bulk status change, payment instruction, claim denial, or irreversible submission. Metrics include action reversibility, downstream propagation risk, scope of affected records, financial exposure, customer or patient impact, and recovery complexity.

\paragraph{Recovery and idempotency.} Enterprise systems are stateful and failure-prone; agents must handle stale data, failed API calls, partial completion, retries, and duplicate submissions. Metrics include idempotency under retry, safe handling of API failure, partial-completion recovery, stale-state detection, rollback success, and compensating-action correctness.

\paragraph{Policy compliance and permissions.} The agent must act within role-based authority and standard operating procedure and obtain required approval before high-risk actions. Metrics include unauthorized-action, policy-violation, and approval-bypass rates; correct distinction between draft, submit, approve, and execute; correct use of role permissions; and completion conditioned on policy adherence. A useful headline metric is \emph{task completion under policy compliance}, which credits the agent only when it both finishes the task and breaks no rule.

\paragraph{Human-oversight cost for write operations.} Because a bad write is consequential, many writes require verification before commit. Metrics include human review time, review-artifact completeness, human correction rate and edit distance, reviewer confidence, escalation volume, and automation rate by confidence threshold. The goal is a confidence-gated pattern: commit autonomously on high-confidence, low-blast-radius actions, and route the rest to a human owner.

\subsection{Relevant benchmark families}

Tier 2 is closest to enterprise workflow, browser automation, API orchestration, and state-based task benchmarks:

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{3.4cm} W Z{4.0cm}}
\toprule
\textbf{Benchmark} & \textbf{What it measures} & \textbf{Relevance} \\
\midrule
CRMArena \citep{crmarena} / CRMArena-Pro \citep{crmarenapro} & CRM tasks across service, sales, and CPQ with workflow execution and confidentiality awareness & Strong fit for enterprise workflow and business-process agents \\
\addlinespace
AutomationBench \citep{automationbench} & Cross-application workflow orchestration through REST APIs, policy adherence, and end-state grading & Strong fit for multi-system write automation \\
\addlinespace
ST-WebAgentBench \citep{stwebagentbench} & Safety and trustworthiness of enterprise web agents & Relevant for write-operation risk and policy compliance \\
\addlinespace
WorkArena \citep{workarena} & Enterprise knowledge-work tasks in ServiceNow-style environments & Useful for browser-based workflow automation \\
\addlinespace
WebArena \citep{webarena} / VisualWebArena \citep{visualwebarena} & Web task completion in realistic environments & Useful for web-based state-changing tasks \\
\addlinespace
OSWorld \citep{osworld} & Desktop and web application tasks with execution-based evaluation & Useful for computer-use agents that manipulate real applications \\
\bottomrule
\end{tabularx}
\end{table}

Tier 2 marks the transition from insight to action. Recovery and idempotency are weakly served by existing public benchmarks, which focus on single-attempt final-state correctness; these dimensions are central to enterprise deployment and represent both a research gap and a place where domain-grounded evaluation is required.


==> old/sections/08_tier3.tex <==
\section{Tier 3: Open User-Facing Task-Completion Agents}
\label{sec:tier3}

\subsection{Definition and core evaluation question}

Tier 3 agents interact with users through open conversation to complete a task; the agent reads, may write, and must negotiate the task itself with a live or simulated user who may be confused, demanding, adversarial, emotional, or malicious, may provide incomplete information, change their mind, request a policy exception, or attempt manipulation. This is the hardest tier because the input is no longer controlled: the task emerges from a live exchange rather than being handed to the agent. Representative types include retail customer service, travel booking and modification, patient scheduling, telecom support, marketplace dispute, loan-application, government-service, employee help-desk, and technical-support agents. The core question is: \emph{can the agent complete user-facing tasks through open-ended conversation while following policy, protecting users, and resisting misuse?} The full Tier 3 setting combines all three risk surfaces: evidence risk, write-action risk, and open-interaction risk.

\subsection{Additional evaluation criteria}

\paragraph{Conversation robustness.} Maintain context across turns, handle corrections, recover from misunderstandings, and ask only necessary clarification questions: multi-turn task success, context retention, correction handling, clarification and conversation-length efficiency, and avoidance of repetitive loops.

\paragraph{Intent and slot completion.} Collect required information before acting without over-collecting sensitive data: intent-classification accuracy, required-field completion, unnecessary-question rate, sensitive-data minimization, and correct handling of inconsistent user-provided information.

\paragraph{Policy compliance under pressure.} Remain helpful while enforcing policy when users request exceptions or push the agent to bypass rules: policy-following accuracy, exception-handling correctness, improper-concession rate, correct-refusal rate, policy-explanation quality, and safe-escalation rate.

\paragraph{Guardrails against malicious use and jailbreaking.} Because the surface is open, Tier 3 evaluation must include a red-team track: jailbreak and prompt-injection resistance, sensitive-information and cross-user leakage rates, malicious-use refusal accuracy, hidden-policy leakage, and secure tool-use behavior. Defenses tuned for single-turn chatbots may not transfer to multi-step agents, so the guardrail must be evaluated in the agentic setting directly.

\paragraph{Repeated-trial reliability.} Open conversation introduces variance; an agent that resolves a task once but fails it on the next attempt is not deployable. A useful metric is $\mathrm{pass}^{k}$, the probability of succeeding on all $k$ independent trials, which exposes reliability a single pass rate hides.

\paragraph{User experience.} Enterprise deployment requires a good user experience: satisfaction, helpfulness, resolution clarity, escalation experience, friction and repetition rate, and trust and transparency.

\subsection{Relevant benchmark families}

Tier 3 is closest to conversational tool-use, customer-service, dual-control, and agent-safety benchmarks:

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{4.0cm} W Z{4.0cm}}
\toprule
\textbf{Benchmark} & \textbf{What it measures} & \textbf{Relevance} \\
\midrule
$\tau$-bench \citep{taubench} & Dynamic conversations between simulated users and tool-using agents with domain policy and final-state verification & Canonical benchmark for open conversational task completion \\
\addlinespace
$\tau^2$-bench \citep{tautwobench} & Dual-control setting where both user and agent act in a shared environment & Useful for support scenarios where the user must also take actions \\
\addlinespace
AgentHarm \citep{agentharm} & Harmful agentic requests and jailbreak robustness & Relevant for malicious-use and misuse evaluation \\
\addlinespace
ST-WebAgentBench \citep{stwebagentbench} & Trustworthiness and safety of web agents & Relevant for policy and safety under tool use \\
\addlinespace
SafeAgentBench \citep{safeagentbench} / Agent-SafetyBench \citep{agentsafetybench} & Tool-use harm and safety-policy enforcement & Relevant for broader agentic safety coverage \\
\bottomrule
\end{tabularx}
\end{table}

Tier 3 is the most complex class because the agent must combine reasoning, tool use, workflow execution, policy compliance, safety, and robust conversation under unpredictable user behavior.


==> old/sections/09_tiers_compound.tex <==
\section{How the Tiers Compound}
\label{sec:compound}

The three tiers are cumulative from an evaluation perspective (\cref{tab:compound}). A read-only research agent needs grounding and calibration; a write-back workflow agent needs write-risk scoring and verification; an open user-facing agent needs adversarial robustness and repeated-trial reliability on top of everything else.

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{Z{2.9cm} Z{3.2cm} Z{3.2cm} W}
\toprule
\textbf{Dimension} & \textbf{Tier 1: Insight} & \textbf{Tier 2: Workflow} & \textbf{Tier 3: Open task completion} \\
\midrule
Agent action & Read only & Read and write & Read, write, and converse \\
\addlinespace
Autonomy surface & Retrieve and synthesize & Commit workflow actions & Negotiate task with live user \\
\addlinespace
Worst-case failure & Misleading insight & Incorrect system mutation & Unsafe or policy-violating interaction \\
\addlinespace
Evaluation criteria & Grounding, abstention, insight quality & Write risk, permissions, human-review cost & Guardrails, jailbreak resistance, repeated-trial reliability \\
\addlinespace
Human-oversight cost & Low to medium; spot-check artifacts & Medium to high; verify before commit & High; review plus adversarial coverage \\
\addlinespace
Primary deployment question & Can we trust the answer? & Can we trust the action? & Can we trust the interaction? \\
\bottomrule
\end{tabularx}
\caption{The three tiers compound: each inherits the requirements of the tiers below it and adds a new risk surface.}
\label{tab:compound}
\end{table}

==> old/sections/10_platform.tex <==
\section{The Evaluation Platform}
\label{sec:platform}

The framework is realized by a backend platform whose core abstraction is
\begin{quote}
\textbf{task specification} $\times$ \textbf{agent harness} $\times$ \textbf{environment,}
\end{quote}
combined with hidden references, immutable execution traces, state inspection, and enterprise-specific oversight modeling. The platform is organized as a pipeline: a contributor portal feeds a task registry and review workflow; a secure asset and policy vault holds inputs and governing documents; an environment orchestrator instantiates the task; an agent adapter runs the system under test; a trajectory, artifact, and state store records everything; an evaluation engine scores the run; and an oversight simulator produces deployment profiles and leaderboards.

\subsection{Task realism and design principles}

The platform enforces the design principles that make a result a \emph{deployment} decision rather than a quality score. Tasks resemble real enterprise work, specifying a user goal, an enterprise role or persona, available systems and tools, relevant documents and data sources, the business policy, the expected output or final system state, the risk level, the required human-review behavior, and an evaluation rubric (Axes~A--G). The platform preserves evidence and action traces, such as retrieved sources, claims and supporting evidence, tool calls, API inputs and outputs, state changes, human-review requests, and escalation rationale. For Tier~2 and Tier~3 tasks, the final enterprise state is inspected directly against a hidden expected end state with state reset between trials. Scoring is risk-tiered by Axis~F, so a formatting slip is not scored like a wrong record update or a privacy leak.

\subsection{Agent adapter}

A single normalized run protocol supports API, browser, desktop, CLI, enterprise-product, and multi-agent systems, exposing capabilities rather than prescribing an architecture: \texttt{observe}, \texttt{read\_file}, \texttt{search}, \texttt{query\_database}, \texttt{call\_tool}, \texttt{propose\_write}, \texttt{commit\_write}, \texttt{ask\_user}, \texttt{escalate}, and \texttt{finish}. Crucially, \texttt{propose\_write} is distinct from \texttt{commit\_write}, which allows direct evaluation of approval-gated deployment policies: an agent can be scored on whether it correctly \emph{proposes} a high-risk write for human approval rather than committing it autonomously. Every write is stored as an immutable event capturing the actor, action, object, before/after state, authorization context, timestamp, and reversibility, so that unauthorized or non-recoverable mutations are detectable after the fact.

\subsection{Evaluation engine and hard deployment gates}

The evaluation engine supports multiple grader types within one task---deterministic assertions, structured field and database final-state comparison, citation-entailment and evidence-sufficiency checks, policy-rule checking, rubric-based expert grading, calibrated model-based judging, adversarial and prohibited-action checks, human review, and repeated-run statistics. Critically, Enterprise's First Exam includes \textbf{hard deployment gates}: an output may receive a strong quality score yet still \emph{fail the exam} because it fabricated evidence, violated policy, performed an unauthorized action, failed to escalate a high-risk ambiguity, omitted a required audit trail, or behaved unreliably across repeated attempts.

\subsection{Oversight simulator}
\label{sec:oversight}

The oversight simulator is the platform's most Enterprise's-First-Exam-specific service and the component that computes the metric of \cref{sec:calibration}. For every run it stores the agent's verdict or action, its confidence, whether escalation was requested, the ground-truth need for escalation, human review time, human correction type, human reviewer accuracy, and model and tool cost. From these it computes autonomous coverage, escalation rate, under-escalation and over-escalation rates, system reliability after human review, human minutes per 100 cases, cost per safely completed task, and cost at selected reliability targets such as $95\%$, $98\%$, and $99\%$. This turns the leaderboard's accuracy and calibration columns directly into the deployment economics of \cref{sec:econ-pse}.

\subsection{Deployment-profile output}
\label{sec:profile}

The benchmark deliberately avoids a single global score. A result instead resembles the profile in \cref{lst:profile}: a qualified tier and target reliability, the autonomous coverage and escalation rate that meet it, safety-critical counters (critical policy violations, unsupported-claim rate), repeated-trial reliability, human review time, total safe-completion cost, and an explicit envelope of permitted, approval-required, and not-qualified actions. This reframes evaluation from a static score into a dynamic deployment contract.

\begin{figure}[h]
\begin{efecode}
Qualified tier:            T1, supervised deployment
Target reliability:        98%
Autonomous coverage:       61%
Human escalation rate:     39%
Critical policy violations: 0
Unsupported-claim rate:    1.8%
Repeated-trial full-pass rate: 84%
Human review time:         6.2 minutes/case
Total safe-completion cost: $8.40/case

Permitted:        draft findings; create evidence tables; recommend follow-up
Approval required: final risk classification; external communication
Not qualified:    system-of-record write; autonomous case closure
\end{efecode}
\caption{Illustrative deployment-profile output in place of a single global score.}
\label{lst:profile}
\end{figure}



==> old/sections/11_call_for_participation.tex <==
\section{Call for Participation and Release Plan}
\label{sec:call}

Enterprise's First Exam is intended as a community benchmark and deployment-gating framework built from authentic enterprise workflows. Task completion alone does not establish that an agent is ready for deployment; organizations need to know whether an agent is grounded, policy-compliant, auditable, and reliable, what actions it may perform autonomously, when it must escalate, and how much human oversight is required. We therefore issue two calls.

\paragraph{Call A: domain and task contributors.} We invite domain experts, enterprise practitioners, and organizations to contribute realistic tasks, evaluation criteria, and expert review across evidence-grounded research workflows, state-changing enterprise workflows, and user-facing task-completion workflows, together with the domain policies, authority boundaries, reference artifacts, failure cases, and human-review-time and deployment-risk estimates that make a task gradeable. A strong contribution represents work performed in a real organization, produces a meaningful work product or system state, defines the agent's role, authority, and escalation boundaries, supports reproducible evaluation, and contains no data the contributor lacks the right to share. Contributors may participate as domain advisers, task contributors, expert reviewers, enterprise design partners, or evaluation researchers, and select one of three participation modes: public task and assets, public task description with private evaluation instances, or a fully confidential task executed only in a secure environment. The full contributor submission form appears in \cref{app:callform}.

\paragraph{Call B: agent and model participants.} The agent-participant call requests the agent's name, version, and model backbone; harness and orchestration details; tool access and external services; memory and retrieval configuration; any human assistance allowed during execution; token, infrastructure, and external API costs; the claimed supported deployment tier; and logging and audit support. The leaderboard submission contract evaluates the \textbf{whole agent system}, not only the underlying model.

\paragraph{Release plan.} We plan a phased release: freezing the construct (multi-axis taxonomy, task schema, acceptance criteria, risk and authority model, data policy, and deployment-profile specification); building the Tier-1 substrate (contributor portal, task registry, artifact sandbox, agent-run API, trace storage, and graders); a closed contributor pilot targeting roughly 12--15 workflow families with 8--12 instances each; benchmark validation with expert baselines, independent reference review, evaluator calibration, adversarial tests, and an oversight-cost study; and a first release comprising the taxonomy and methodology paper, a small public development set, a private evaluation pool, contributor and participant calls, an initial leaderboard, and deployment profiles for baseline agents. The primary leaderboard remains private or server-side, with private instances rotated over time to reduce contamination. A detailed schedule appears in \cref{app:roadmap}.


==> old/sections/12_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Professional-work benchmarks establish whether an agent can do the work; they do not establish whether an organization can safely employ it. Enterprise's First Exam fills that gap as both a benchmark and a governance mechanism, built as \emph{authentic executable workflows} (in the spirit of long-horizon computer-use exams), \emph{expert work products} (in the spirit of economically-grounded evaluation), \emph{business-demand mapping} (in the spirit of profession-aligned evaluation), and \emph{Enterprise's First Exam-specific deployment gates and oversight economics}. Its multi-axis taxonomy makes coverage and the deployment envelope of each task explicit; its headline metric reframes evaluation as economics, deriving the minimum-cost human-oversight policy that meets a target reliability; and its platform replaces a single global score with an auditable deployment profile produced by an oversight simulator. The concise differentiation is:

\begin{itemize}[leftmargin=1.6em]
  \item \textbf{GDPval / GDPEval:} is the work good?
  \item \textbf{Profession-aligned evaluation:} is it professionally useful?
  \item \textbf{Agents' Last Exam:} can the agent complete the workflow?
  \item \textbf{Enterprise's First Exam:} can an organization safely employ the agent, under a specified operating policy, at an acceptable total cost?
\end{itemize}

As agent quality improves, the expected human-oversight cost should decline, giving a practical, measurable path from supervised deployment toward higher automation while preserving safety, auditability, and enterprise trust.


==> old/standard_bk_0810.tex <==


% ==================================================================
\section{The EFE Open Standard}
\label{sec:standard}
% ==================================================================

\subsection{Design Principles and Conformance}
\label{sec:standard-principles}

The EFE standard is designed to make enterprise-agent evaluations:

\begin{itemize}
    \item authentic to real organizational workflows;
    \item reproducible across evaluation runs;
    \item interoperable across agent systems and platform implementations;
    \item auditable through complete evidence and action traces;
    \item sensitive to consequence, authority, and reversibility;
    \item extensible across industries and workflow classes.
\end{itemize}

% TODO:
% Define the minimum requirements for:
% 1. an EFE-compliant task specification;
% 2. an EFE-compatible execution platform;
% 3. an EFE benchmark release;
% 4. an EFE deployment profile.


\subsection{Deployment Tracks and Risk Surfaces}
\label{sec:standard-tracks}

Every EFE workflow specifies the deployment tracks it exercises and the
corresponding active risk surfaces.

The three deployment tracks are:

\begin{enumerate}
    \item evidence-grounded insight;
    \item state-changing workflow;
    \item open user-facing completion.
\end{enumerate}

The corresponding primary risk surfaces are:

\begin{enumerate}
    \item evidence and reasoning risk;
    \item enterprise-action risk;
    \item open-interaction risk.
\end{enumerate}

The tracks are composable rather than mutually exclusive. A workflow may
exercise one, two, or all three tracks.


\subsection{Deployment Contract}
\label{sec:standard-contract}

The deployment contract specifies the operating envelope within which the
agent is evaluated. It includes:

\begin{itemize}
    \item the agent's organizational role and accountable human owner;
    \item the intended user or beneficiary;
    \item the available information, systems, and tools;
    \item the actions permitted autonomously;
    \item the actions requiring human approval;
    \item the actions prohibited entirely;
    \item the expected work product or final enterprise state;
    \item the conditions requiring clarification, abstention, or escalation.
\end{itemize}

A correct result produced outside the granted authority boundary is an EFE
deployment failure.


\subsection{Consequence and Reversibility}
\label{sec:standard-risk}

Each workflow is assigned a risk class reflecting the consequence,
propagation, and recoverability of failure.

\begin{table}[t]
    \centering
    \caption{Illustrative EFE consequence and reversibility classes.}
    \label{tab:risk-classes}
    \begin{tabular}{
        >{\raggedright\arraybackslash}p{0.09\textwidth}
        >{\raggedright\arraybackslash}p{0.45\textwidth}
        >{\raggedright\arraybackslash}p{0.36\textwidth}
    }
        \toprule
        \textbf{Class} & \textbf{Description} & \textbf{Illustrative example} \\
        \midrule
        R0 & Informational and easily discarded
           & Internal research note \\

        R1 & Influences a decision but requires human approval
           & Due-diligence or patient-safety memo \\

        R2 & Reversible enterprise-state mutation
           & Draft CRM update or ticket routing \\

        R3 & Consequential external action
           & Claim or prior-authorization submission \\

        R4 & High-impact or difficult-to-reverse commitment
           & Payment, denial, clinical, or legal commitment \\
        \bottomrule
    \end{tabular}
\end{table}

Deployment track does not determine severity by itself. A read-only
recommendation may influence a high-consequence decision, while a
state-changing action may be low-risk if it is reversible and tightly
bounded.


\subsection{Evaluation Primitives}
\label{sec:standard-primitives}

EFE defines reusable evaluation primitives that may be selected according to
the workflow's active risk surfaces:

\begin{enumerate}
    \item outcome correctness and completeness;
    \item evidence grounding and citation support;
    \item policy and authority compliance;
    \item calibration, abstention, and escalation;
    \item write-operation correctness, recovery, and idempotency;
    \item interaction and adversarial robustness;
    \item auditability and trace completeness;
    \item repeated-trial reliability;
    \item human-review effort;
    \item oversight-adjusted operating cost.
\end{enumerate}


\subsection{Context and Coverage Metadata}
\label{sec:standard-metadata}

Context metadata organizes benchmark coverage without itself determining
deployment readiness. It includes:

\begin{itemize}
    \item industry;
    \item organizational function;
    \item professional role;
    \item workflow family;
    \item work activity;
    \item data and tool modalities;
    \item applicable policy and regulatory context.
\end{itemize}


\subsection{Canonical Task Record}
\label{sec:standard-record}

The canonical task record packages the deployment tracks, risk surfaces,
deployment contract, risk class, evaluation primitives, and context metadata
into a versioned, machine-readable specification.

The standard distinguishes four levels:

\begin{description}
    \item[Workflow template.]
    A reusable representation of an enterprise activity.

    \item[Task instance.]
    A concrete and gradeable execution case.

    \item[Benchmark release.]
    A validated, versioned collection of templates and instances.

    \item[Evaluation run.]
    A particular agent configuration executed against a specified benchmark,
    environment, policy, and grader version.
\end{description}

% TODO:
% Insert the finalized canonical YAML or JSON record here.
%
% Recommended fields:
% - task_id and version
% - benchmark release
% - context metadata
% - deployment tracks
% - active risk surfaces
% - role and authority
% - permitted / approval-gated / prohibited actions
% - expected work product or final state
% - escalation conditions
% - risk class
% - policies and policy versions
% - environment version
% - evaluation primitives
% - repeated-trial requirements
% - access and privacy mode


% ==================================================================
\section{Deployment Tracks and Risk Surfaces}
\label{sec:tracks}
% ==================================================================

\subsection{Composable Autonomy Surfaces}
\label{sec:tracks-composable}

The deployment tracks describe autonomy surfaces rather than mutually
exclusive agent categories or a universal maturity ladder. Requirements
compound as a workflow combines evidence synthesis, enterprise-state change,
and open interaction.


\subsection{Track 1: Evidence-Grounded Insight}
\label{sec:track1}

Track~1 agents retrieve, analyze, and synthesize enterprise information into
a reviewable decision-support artifact without directly changing enterprise
state.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the evidence, analysis, and conclusion?}
\end{quote}

Primary requirements include:

\begin{itemize}
    \item evidence grounding and citation support;
    \item completeness and decision relevance;
    \item policy-grounded reasoning;
    \item ambiguity recognition;
    \item abstention and escalation;
    \item auditability;
    \item human-review effort and oversight cost.
\end{itemize}


\subsection{Track 2: State-Changing Workflow}
\label{sec:track2}

Track~2 agents propose or commit actions that change enterprise systems of
record.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the action and its effect on enterprise state?}
\end{quote}

Additional requirements include:

\begin{itemize}
    \item correct action, object, and field selection;
    \item authority and approval compliance;
    \item final-state correctness;
    \item idempotency under retry;
    \item stale-state and partial-failure handling;
    \item rollback or compensating-action correctness;
    \item consequence, propagation, and reversibility analysis.
\end{itemize}


\subsection{Track 3: Open User-Facing Completion}
\label{sec:track3}

Track~3 agents negotiate and complete tasks through open-ended interaction
with live or simulated users.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the interaction under uncontrolled input?}
\end{quote}

Additional requirements include:

\begin{itemize}
    \item intent and required-information collection;
    \item multi-turn context retention and correction handling;
    \item policy compliance under pressure;
    \item privacy and sensitive-data minimization;
    \item manipulation and prompt-injection resistance;
    \item safe tool use;
    \item repeated-trial reliability;
    \item user experience and escalation quality.
\end{itemize}


\subsection{How Risk Surfaces Compound}
\label{sec:tracks-compound}

\begin{table}[t]
    \centering
    \caption{Deployment tracks and their primary risk surfaces.}
    \label{tab:tracks-risks}
    \begin{tabular}{
        >{\raggedright\arraybackslash}p{0.27\textwidth}
        >{\raggedright\arraybackslash}p{0.28\textwidth}
        >{\raggedright\arraybackslash}p{0.35\textwidth}
    }
        \toprule
        \textbf{Deployment track}
        & \textbf{Primary surface}
        & \textbf{Characteristic failures} \\
        \midrule

        Evidence-grounded insight
        & Evidence and reasoning
        & Missed evidence, unsupported claims, incorrect policy application,
          and failure to recognize ambiguity \\

        State-changing workflow
        & Enterprise action
        & Wrong-object mutation, unauthorized action, duplicate execution,
          failed recovery, or irreversible downstream effects \\

        Open user-facing completion
        & Open interaction
        & Misunderstood intent, improper policy concession, manipulation,
          privacy leakage, or unsafe behavior \\
        \bottomrule
    \end{tabular}
\end{table}



==> old/standard_bk_0817.tex <==
% ==================================================================
\section{The EFE Open Standard}
\label{sec:standard}
% ==================================================================

Enterprise's First Exam separates the \emph{standard} for describing an
enterprise deployment evaluation from the particular infrastructure used to
execute it. The standard defines the information that must be specified about
the workflow, agent authority, environment, risks, evaluation requirements,
and deployment assumptions. The reference platform in
Section~\ref{sec:platform} implements this standard on top of a reusable
agent-evaluation substrate, but conformance with EFE does not require use of
that particular implementation.

The purpose of this separation is interoperability. An enterprise workflow
should be specifiable once and executable against different agent systems,
evaluation platforms, and deployment policies without silently changing what
is being tested. Conversely, a result should be interpretable only together
with the workflow, authority boundary, environment, policy, and evaluator
versions under which it was obtained.

\subsection{Design Principles and Conformance}
\label{sec:standard-principles}

The EFE standard is designed to make enterprise-agent evaluations:

\begin{itemize}
    \item \textbf{authentic}, by representing real organizational workflows,
    information sources, policies, actions, and work products rather than
    isolated capability probes;

    \item \textbf{reproducible}, by versioning the task, environment,
    policies, references, graders, agent configuration, and deployment
    assumptions associated with an evaluation;

    \item \textbf{interoperable}, by defining the deployment and evaluation
    semantics independently of a particular model, agent harness, or
    execution platform;

    \item \textbf{auditable}, by requiring sufficient evidence, action,
    artifact, and state records to reconstruct consequential behavior;

    \item \textbf{authority-aware}, by distinguishing what an agent can
    technically do from what it is organizationally permitted to do;

    \item \textbf{consequence-sensitive}, by representing the severity,
    propagation, and reversibility of failures rather than treating all task
    errors equivalently; and

    \item \textbf{extensible}, by allowing new industries, workflow classes,
    environments, policies, risk surfaces, and evaluators to be added without
    changing the core representation.
\end{itemize}

EFE defines conformance at several different levels. This distinction is
important because an EFE-compatible task need not be executed on the EFE
reference platform, and an execution platform can support EFE without hosting
a particular public benchmark.

\paragraph{EFE-compliant task specification.}
A compliant task specification must identify a versioned workflow and
concrete task instance and must declare, at minimum:

\begin{itemize}
    \item the organizational and workflow context;
    \item the active deployment tracks and risk surfaces;
    \item the deployment contract, including role, information access,
    authority, approval, prohibition, and escalation boundaries;
    \item the expected work product or final enterprise state;
    \item the consequence and reversibility class;
    \item the governing policies and their versions;
    \item the environment and governed assets required by the task;
    \item the applicable evaluation primitives and hard gates;
    \item the evaluator or reference requirements;
    \item repeated-trial requirements where applicable; and
    \item the access, privacy, and release mode of the task and its assets.
\end{itemize}

\paragraph{EFE-compatible execution platform.}
A compatible platform must be capable of instantiating the declared task
environment and authority boundary, executing heterogeneous agents without
changing the task semantics, preserving evaluator-only assets from agent
access, and recording the artifacts, environment events, state transitions,
and grader outputs required by the specification. It must also preserve the
versions of the benchmark, environment, policies, agent configuration, and
graders associated with each run. A platform need not expose a particular
agent API or internal orchestration architecture.

\paragraph{EFE benchmark release.}
An EFE benchmark release is a versioned collection of validated workflow
templates and task instances together with the environments, policies,
references, evaluators, access conditions, and documentation necessary to
interpret the results. The release must state its coverage and known
limitations and must distinguish agent-visible assets from hidden or
evaluator-only assets.

\paragraph{EFE deployment profile.}
A conformant deployment profile must identify the exact evaluation
configuration from which it was derived and report, at minimum, hard-gate
outcomes, qualified workflow scope, permitted agent authority, autonomy and
approval boundaries, achievable reliability and autonomous coverage where
defined, observed residual risks, required escalation or human review, and
the assumptions used to estimate oversight and operating cost.

Conformance is always relative to a version of the EFE schema. Material
changes to the task, environment, policy corpus, authority configuration,
agent harness, model, evaluator, or deployment assumptions define a new
evaluation configuration and may require requalification.

\subsection{Deployment Tracks and Risk Surfaces}
\label{sec:standard-tracks}

EFE represents enterprise autonomy through three composable
\emph{deployment tracks}. A track describes a class of activity the agent is
expected to perform. Each track activates a corresponding primary
\emph{risk surface}, describing the characteristic way in which that activity
can fail.

The three deployment tracks are:

\begin{enumerate}
    \item \textbf{evidence-grounded insight}: retrieving, analyzing, and
    synthesizing information into a reviewable work product;

    \item \textbf{state-changing workflow}: selecting, proposing, or
    committing actions that can change enterprise state; and

    \item \textbf{open user-facing completion}: completing a task through
    open-ended interaction with a live or simulated user.
\end{enumerate}

Their primary risk surfaces are, respectively:

\begin{enumerate}
    \item \textbf{evidence and reasoning risk}: incorrect, incomplete,
    unsupported, or improperly grounded analysis;

    \item \textbf{enterprise-action risk}: incorrect, unauthorized,
    duplicated, poorly recovered, or consequential state change; and

    \item \textbf{open-interaction risk}: failures arising from uncontrolled
    user input, including misunderstanding, manipulation, policy concession,
    privacy leakage, or unsafe behavior.
\end{enumerate}

The mapping is not exclusive. A workflow can activate one, two, or all three
tracks and may therefore expose several risk surfaces simultaneously. The
tracks should not be interpreted as a universal maturity ladder or as global
agent categories. For example, a customer-facing informational assistant may
combine evidence-grounded insight with open interaction while remaining
read-only; a background prior-authorization agent may combine evidence
reasoning with state-changing action without interacting directly with a
user.

The active tracks determine which classes of evaluation are required, while
the deployment contract and consequence class determine the authority,
severity, and oversight conditions under which those capabilities are tested.

\subsection{Deployment Contract}
\label{sec:standard-contract}

The \emph{deployment contract} is the central operational object in the EFE
standard. It specifies the bounded role in which the agent is being
qualified. EFE therefore does not ask whether an agent is ``enterprise
ready'' in the abstract; it asks whether a particular agent configuration can
operate within a particular contract.

A deployment contract specifies:

\begin{itemize}
    \item \textbf{organizational role and accountability}: the role being
    performed, the intended user or beneficiary, and the human owner
    accountable for the workflow;

    \item \textbf{information authority}: the data, documents, systems,
    memory, communication channels, and other information the agent may
    access;

    \item \textbf{tool and system access}: the applications, APIs, databases,
    browsers, execution environments, or other tools available during the
    task;

    \item \textbf{action authority}: the operations the agent may perform
    autonomously, the operations it may propose but not commit, and the
    operations that require explicit approval;

    \item \textbf{prohibited actions}: operations that the agent must not
    perform under any deployment policy represented by the contract;

    \item \textbf{expected end state}: the required work product, enterprise
    state, external action, or completed interaction by which task completion
    is judged;

    \item \textbf{governing policy}: the regulations, organizational
    procedures, professional standards, contractual rules, or other
    authoritative sources that constrain the task;

    \item \textbf{clarification and escalation conditions}: circumstances
    under which the agent must request information, abstain, seek approval,
    or transfer responsibility to a human; and

    \item \textbf{operational constraints}: where relevant, resource,
    latency, time, cost, privacy, or security constraints that are part of
    the intended deployment.
\end{itemize}

EFE distinguishes \emph{technical capability} from \emph{granted authority}.
The fact that an environment technically exposes an operation does not imply
that the agent is permitted to use it. Conversely, a production policy may
require human approval for an action that the agent is being evaluated on its
ability to select correctly.

Actions are therefore classified by the contract rather than inferred from
the agent's behavior:

\begin{description}
    \item[Autonomous.] The agent may execute the operation without prior
    human approval when the specified conditions are satisfied.

    \item[Approval-gated.] The agent may prepare or propose the operation,
    but commitment requires approval from an authorized actor.

    \item[Prohibited.] The operation is outside the agent's authority for
    this workflow.
\end{description}

A correct task outcome produced by exceeding the declared authority boundary
is an EFE deployment failure. Likewise, successful task completion does not
compensate for a required escalation that the agent failed to make.

The standard also distinguishes \emph{agent-visible assets} from
\emph{evaluator-only assets}. Hidden references, protected grader logic,
private policy annotations, adversarial test state, and other evaluator
material must not become accessible simply because they are necessary to
score the task.

\subsection{Consequence and Reversibility}
\label{sec:standard-risk}

Task difficulty and deployment risk are different concepts. EFE therefore
represents the consequence of failure separately from both benchmark score
and deployment track.

Each task specifies a consequence and reversibility class reflecting three
properties: the severity of a plausible failure, the degree to which its
effect can propagate beyond the immediate task, and the cost or feasibility
of detecting and reversing it. Table~\ref{tab:risk-classes} gives the
reference classes.

\begin{table}[t]
\centering
\caption{Illustrative EFE consequence and reversibility classes.}
\label{tab:risk-classes}
\begin{tabular}{
>{\raggedright\arraybackslash}p{0.09\textwidth}
>{\raggedright\arraybackslash}p{0.45\textwidth}
>{\raggedright\arraybackslash}p{0.36\textwidth}
}
\toprule
\textbf{Class} & \textbf{Description} & \textbf{Illustrative example} \\
\midrule

R0
& Informational output with no persistent enterprise or external effect
& Internal research note \\

R1
& Influences a consequential decision but remains mediated by human review
or approval
& Due-diligence or patient-safety memo \\

R2
& Bounded and normally reversible enterprise-state mutation
& Draft CRM update or ticket routing \\

R3
& Consequential internal or external action whose correction may require
material recovery effort
& Claim or prior-authorization submission \\

R4
& High-impact, propagating, or difficult-to-reverse commitment
& Payment, denial, clinical, or legal commitment \\

\bottomrule
\end{tabular}
\end{table}

Deployment track does not determine severity by itself. A read-only
recommendation may influence a high-consequence decision, while a
state-changing operation can be relatively low risk if it is tightly bounded
and reliably reversible.

For workflows containing actions of materially different severity, the task
may annotate individual action classes in addition to a task-level class.
The task-level class should reflect the highest consequence that is
reasonably reachable within the granted authority envelope, rather than an
unreachable capability of the underlying software system.

The consequence class does not by itself determine whether a task passes
EFE. Instead, it informs the evaluation profile: higher-consequence tasks may
require stronger hard gates, more repeated trials, narrower autonomous
authority, explicit approval policies, stronger statistical evidence, or
lower tolerated critical-failure rates.

\subsection{Evaluation Primitives}
\label{sec:standard-primitives}

EFE defines reusable \emph{evaluation primitives} rather than prescribing a
single universal score. A task selects the primitives needed for its active
risk surfaces and declares how each primitive contributes to scoring,
diagnostics, or hard deployment gates.

The reference primitive set is:

\begin{description}

    \item[Outcome correctness and completeness.]
    Whether the required work product, decision, interaction result, or final
    enterprise state is correct and sufficiently complete for the workflow.

    \item[Evidence grounding and citation support.]
    Whether consequential claims can be traced to evidence available during
    the task, whether that evidence actually supports the claim, and whether
    the agent distinguishes observed facts from inference or assumption.

    \item[Policy and authority compliance.]
    Whether the agent applies the governing policy correctly, remains within
    its role and information boundary, obtains required approvals, and avoids
    prohibited actions.

    \item[Calibration, abstention, and escalation.]
    Whether uncertainty signals meaningfully discriminate safe from unsafe
    autonomous cases and whether the agent requests clarification, abstains,
    or escalates when evidence, confidence, policy, or authority is
    insufficient.

    \item[Write-operation correctness, recovery, and idempotency.]
    For state-changing workflows, whether the correct action is applied to
    the correct object with the correct values and whether the agent safely
    handles stale state, retries, duplicate requests, partial failure,
    rollback, and compensating actions.

    \item[Interaction and adversarial robustness.]
    For open-interaction workflows, whether the agent preserves intent,
    policy, privacy, and safety under multi-turn corrections, manipulation,
    prompt injection, malicious requests, and other uncontrolled input.

    \item[Auditability and trace completeness.]
    Whether an independent reviewer can reconstruct the material evidence,
    decisions, actions, approvals, state changes, and escalations relevant to
    the outcome.

    \item[Repeated-trial reliability.]
    Whether the system behaves consistently across repeated attempts,
    including the frequency and distribution of critical failures that may be
    obscured by mean task performance.

    \item[Human-review effort.]
    The time, correction, approval, or other human work required to safely
    use the agent's output or actions.

    \item[Oversight-adjusted operating cost.]
    The total expected cost of operating the agent under a deployment policy
    that satisfies the required reliability and hard-gate constraints,
    including model execution, review, approval, escalation, and recovery
    where applicable.

\end{description}

Each task defines an \emph{evaluation profile} that identifies which
primitives apply and how they are used. A primitive may be:

\begin{itemize}
    \item a \textbf{hard gate}, for which a specified violation is
    disqualifying;
    \item a \textbf{scored measure}, used to characterize comparative task
    performance;
    \item a \textbf{deployment measure}, used to determine autonomy,
    escalation, reliability, or cost; or
    \item a \textbf{diagnostic}, retained to characterize a failure mode
    without directly determining pass or fail.
\end{itemize}

This separation prevents strong performance on one dimension from averaging
away a non-negotiable failure on another. For example, high artifact quality
cannot compensate for an unauthorized write, and high average accuracy
cannot by itself establish acceptable reliability when a critical failure
class remains uncontrolled.

The qualification methodology in Section~\ref{sec:qualification} combines
these primitive outputs into hard gates, reliability--autonomy tradeoffs,
and oversight economics.

\subsection{Context and Coverage Metadata}
\label{sec:standard-metadata}

EFE separately records \emph{context and coverage metadata}. These fields
describe where the task sits in the enterprise landscape and enable
benchmark coverage analysis, but they do not by themselves imply deployment
readiness.

Context metadata includes, where applicable:

\begin{itemize}
    \item industry or sector;
    \item organizational function;
    \item professional role;
    \item workflow family;
    \item work activities;
    \item data modalities;
    \item tool and interaction modalities;
    \item jurisdiction or operating region;
    \item applicable policy, contractual, or regulatory context; and
    \item relevant data-sensitivity or access classification.
\end{itemize}

The distinction between context metadata and deployment semantics is
deliberate. ``Healthcare'' or ``financial services,'' for example, is not a
risk class. Two workflows in the same industry can expose radically
different authority and consequence surfaces, while similar workflow
structures may recur across industries.

Coverage metadata therefore supports questions such as which industries,
roles, work activities, modalities, and risk surfaces are represented in a
benchmark release. Deployment qualification is instead determined by the
specific contract, active risk surfaces, consequence class, evaluation
results, and deployment policy.

\subsection{Canonical Task Record and Evaluation Lineage}
\label{sec:standard-record}

The fields above are represented in a versioned, machine-readable canonical
record. The record is intended to be sufficiently explicit that a compatible
platform can instantiate the task without relying on undocumented benchmark
conventions.

EFE distinguishes the following objects in the evaluation lifecycle:

\begin{description}

    \item[Workflow template.]
    A reusable representation of an enterprise activity. It defines the
    organizational role, workflow semantics, possible authority envelope,
    expected work-product type, relevant risk surfaces, and evaluation
    requirements that are common across concrete cases.

    \item[Task instance.]
    A concrete and gradeable case instantiated from a workflow template. It
    supplies the particular inputs, initial environment state, applicable
    policies, task-specific references, hidden evaluation material, and
    expected end-state conditions.

    \item[Benchmark release.]
    A validated and frozen collection of workflow templates and task
    instances together with their associated environment, policy, reference,
    and evaluator versions.

    \item[Evaluation configuration.]
    A binding of a benchmark release to a particular model, agent harness,
    environment implementation, authority configuration, deployment policy,
    evaluator versions, and run-level assumptions.

    \item[Trial record.]
    The immutable record of one execution attempt, including the resulting
    artifacts, relevant trajectory, environment events, state changes,
    approvals, escalations, costs, and grader outputs.

    \item[Deployment profile.]
    The qualification output derived from one or more trial records under a
    specified evaluation configuration and deployment assumptions.

\end{description}

The resulting lineage is:

\begin{equation}
\text{workflow template}
\rightarrow
\text{task instance}
\rightarrow
\text{benchmark release}
\rightarrow
\text{evaluation configuration}
\rightarrow
\text{trial records}
\rightarrow
\text{deployment profile}.
\label{eq:efe-lineage}
\end{equation}

This lineage prevents a leaderboard result from becoming detached from the
conditions under which it was produced. In particular, benchmark release,
agent configuration, environment, policy corpus, graders, and deployment
assumptions remain recoverable from the deployment profile.

A canonical task record should contain, at minimum, the following groups of
fields:

\begin{itemize}
    \item identity and schema version;
    \item workflow-template and benchmark-release references;
    \item context and coverage metadata;
    \item deployment tracks and active risk surfaces;
    \item role, information access, and action authority;
    \item permitted, approval-gated, and prohibited actions;
    \item expected work product or final enterprise state;
    \item clarification, abstention, and escalation conditions;
    \item consequence and reversibility class;
    \item governing policy references and versions;
    \item environment and governed-asset references;
    \item evaluation primitives, hard gates, and evaluator versions;
    \item repeated-trial requirements; and
    \item access, privacy, and release mode.
\end{itemize}

Figure~\ref{fig:canonical-task-record} gives an illustrative YAML-style
representation for an evidence-grounded patient-safety workflow. The exact
serialization may evolve with the schema; the normative requirement is the
semantics of the represented fields rather than YAML itself.

\begin{figure}[t]
\small
\begin{verbatim}
schema_version: efe.v1

task:
  id: healthcare.patient_safety.review.001
  version: 1
  workflow_template:
    id: healthcare.patient_safety.review
    version: 1
  benchmark_release: clinicare.efe.v1

context:
  industry: healthcare
  function: quality_and_safety
  role: patient_safety_reviewer
  workflow_family: event_review
  work_activities:
    - investigation
    - analysis
    - inspection
  modalities:
    - longitudinal_records
    - clinical_notes
    - policy_documents

deployment:
  tracks:
    - evidence_grounded_insight
  risk_surfaces:
    - evidence_and_reasoning
  risk_class: R1

contract:
  accountable_owner: quality_manager

  information_access:
    - patient_record
    - approved_policy_corpus

  autonomous_actions:
    - retrieve_records
    - construct_timeline
    - draft_findings

  approval_gated_actions: []

  prohibited_actions:
    - amend_patient_record
    - contact_patient

  expected_end_state:
    type: patient_safety_review
    required:
      - event_timeline
      - evidence_citations
      - policy_mapping
      - findings
      - uncertainty

  escalation_conditions:
    - conflicting_material_evidence
    - missing_governing_policy
    - possible_immediate_harm

policies:
  - id: institutional_patient_safety
    version: 2026-07

environment:
  id: clinicare_mimic
  version: 1
  initial_state: case_001
  access_mode: server_side

evaluation:
  primitives:
    - outcome_correctness
    - evidence_grounding
    - policy_authority_compliance
    - abstention_escalation
    - auditability
    - human_review_effort
    - oversight_adjusted_cost

  hard_gates:
    - no_prohibited_action
    - required_traceability

  repeated_trials: 3

assets:
  agent_visible:
    - patient_record
    - approved_policy_corpus
  evaluator_only:
    - expert_reference
    - hidden_grader_state
\end{verbatim}
\caption{Illustrative canonical EFE task record. The serialization is
illustrative; EFE standardizes the deployment and evaluation semantics rather
than requiring YAML as the interchange format.}
\label{fig:canonical-task-record}
\end{figure}

The canonical record contains references to governed assets rather than
requiring confidential data to be embedded directly in the task
specification. This allows public, gated, private, and server-side benchmark
releases to share the same standard while applying different access controls.

The reference platform in Section~\ref{sec:platform} compiles these records
into executable task packages, governed environments, evaluation
configurations, and trial records. Other platforms may do the same provided
that they preserve the declared semantics and evaluation lineage.


% ==================================================================
\section{Deployment Tracks and Risk Surfaces}
\label{sec:tracks}
% ==================================================================

\subsection{Composable Autonomy Surfaces}
\label{sec:tracks-composable}

The deployment tracks identify distinct surfaces on which enterprise
autonomy creates value and risk. They are deliberately composable rather than
cumulative levels.

The distinction matters because evidence access, action authority, and
interaction openness can vary independently. A read-only customer assistant
may interact openly with users but never modify enterprise state. A
background payment or clinical workflow may have substantial mutation
authority without any user conversation. An interactive support agent may
converse freely and propose a state-changing action while requiring a human
to approve the commit.

EFE therefore characterizes a workflow by the set of tracks it exercises:

\begin{equation}
\mathcal{T}(w)
\subseteq
\{
\text{insight},
\text{state change},
\text{open interaction}
\}.
\end{equation}

The evaluation requirements for the workflow are formed from the risk
surfaces activated by that set, together with the deployment contract and
consequence class. Combining tracks generally increases the number of
failure modes that must be controlled, but it does not imply a universal
ordering of severity. A Track~1 workflow can be more consequential than a
Track~2 workflow if the former informs a high-stakes decision and the latter
performs a tightly bounded reversible write.

\subsection{Track 1: Evidence-Grounded Insight}
\label{sec:track1}

Track~1 covers workflows in which the agent retrieves, analyzes, and
synthesizes information into a reviewable work product without directly
committing a change to persistent enterprise or external state.

Typical outputs include research reports, due-diligence analyses,
patient-safety reviews, compliance assessments, contract analyses, financial
memos, and other decision-support artifacts.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the evidence, analysis, and conclusion?}
\end{quote}

The defining risk is not simply whether the final answer matches a reference.
A plausible conclusion may still be unsuitable for deployment if material
evidence was missed, claims are unsupported by retrieved sources, governing
policy was applied incorrectly, contradictory records were silently
resolved, or uncertainty that should have triggered escalation was hidden.

Track~1 evaluation therefore commonly requires:

\begin{itemize}
    \item outcome correctness and completeness;
    \item evidence grounding and citation support;
    \item distinction among evidence, inference, and assumption;
    \item policy-grounded reasoning;
    \item ambiguity and contradiction recognition;
    \item appropriate clarification, abstention, and escalation;
    \item auditability of the evidence-to-conclusion path;
    \item repeated-trial reliability where stochasticity matters; and
    \item human-review effort and oversight cost.
\end{itemize}

``Read-only'' refers to persistent enterprise state. The agent may create
temporary files, calculations, intermediate analyses, or draft artifacts
inside its execution environment. If the deployment contract authorizes the
agent to commit a persistent workflow action or external side effect, the
workflow also activates Track~2. If the agent must complete the task through
open-ended interaction with a user, it also activates Track~3.

\subsection{Track 2: State-Changing Workflow}
\label{sec:track2}

Track~2 covers workflows in which the agent must select, prepare, propose, or
commit an action whose intended effect is to change enterprise or external
state. Examples include updating CRM or ERP records, creating or routing
tickets, reconciling accounts, filing submissions, modifying workflow status,
issuing approvals, or triggering downstream services.

The track includes approval-gated deployments in which a human ultimately
commits the action. The relevant deployment question is still whether the
agent can identify and construct the correct state-changing operation, even
when the production policy does not permit autonomous commitment.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the action and its effect on enterprise state?}
\end{quote}

Track~2 adds a class of failures that cannot be captured by grading the final
natural-language artifact alone. An agent may select the wrong object,
modify the wrong field, act on stale state, exceed its authority, submit the
same operation twice, leave the workflow partially completed, or create a
downstream effect that is difficult to reverse.

Evaluation therefore commonly includes:

\begin{itemize}
    \item correct action, object, field, and value selection;
    \item authority and approval compliance;
    \item final-state correctness;
    \item before-and-after state verification;
    \item stale-state and concurrency handling;
    \item idempotency under retry;
    \item partial-failure detection and recovery;
    \item rollback or compensating-action correctness;
    \item prohibited-action detection;
    \item consequence and downstream-propagation analysis; and
    \item appropriate approval or escalation behavior.
\end{itemize}

The deployment contract determines which of these actions may be committed
autonomously. An agent can therefore demonstrate strong Track~2 capability
while still receiving a deployment profile that requires human approval for
particular operations because of their consequence class or the
organization's risk tolerance.

When the action depends on substantive evidence synthesis, the workflow also
activates Track~1. When the action is negotiated or completed through
open-ended user interaction, it also activates Track~3.

\subsection{Track 3: Open User-Facing Completion}
\label{sec:track3}

Track~3 covers workflows in which the task itself develops through
open-ended interaction with a live or simulated user. The agent must infer or
confirm intent, collect missing information, respond to corrections, apply
policy as new facts arrive, and determine when the interaction can safely be
completed or must be escalated.

Examples include customer support, benefits navigation, scheduling,
account-service workflows, claims intake, interactive troubleshooting, and
other tasks in which the user controls part of the information flow.

The primary deployment question is:

\begin{quote}
\textbf{Can we trust the interaction under uncontrolled input?}
\end{quote}

Open interaction introduces risk even when the agent is read-only. Users may
provide incomplete or inconsistent information, change their request,
pressure the agent for exceptions, expose unnecessary sensitive data,
attempt prompt injection, or deliberately pursue prohibited outcomes.
Conversational success therefore cannot be reduced to whether the final user
request appears to have been completed.

Track~3 evaluation commonly includes:

\begin{itemize}
    \item intent recognition and required-information collection;
    \item clarification efficiency and avoidance of unnecessary questioning;
    \item multi-turn context retention;
    \item correction and contradiction handling;
    \item policy compliance under user pressure;
    \item privacy and sensitive-data minimization;
    \item manipulation, prompt-injection, and jailbreak resistance;
    \item safe use of tools exposed during the conversation;
    \item refusal and escalation quality;
    \item repeated-trial reliability; and
    \item user experience, resolution clarity, and interaction efficiency.
\end{itemize}

Track~3 does not imply Track~2. An informational assistant can converse
openly while remaining unable to change enterprise state. Conversely, when
the interaction authorizes or causes persistent actions, both Tracks~2 and~3
are active and the evaluation must cover both interaction risk and
enterprise-action risk.

For simulated-user evaluation, information known only to the simulated user
may be retained as hidden environment state. This allows the evaluator to
measure whether the agent successfully elicits required information without
making that information directly available to the agent at the start of the
task.

\subsection{How Risk Surfaces Compound}
\label{sec:tracks-compound}

Each track has a characteristic primary risk surface, summarized in
Table~\ref{tab:tracks-risks}. These surfaces identify the dominant new
failure mode introduced by the corresponding activity; they do not imply
that other evaluation primitives become irrelevant.

\begin{table}[t]
\centering
\caption{Deployment tracks and their primary risk surfaces.}
\label{tab:tracks-risks}
\begin{tabular}{
>{\raggedright\arraybackslash}p{0.27\textwidth}
>{\raggedright\arraybackslash}p{0.28\textwidth}
>{\raggedright\arraybackslash}p{0.35\textwidth}
}
\toprule
\textbf{Deployment track}
& \textbf{Primary surface}
& \textbf{Characteristic failures} \\
\midrule

Evidence-grounded insight
& Evidence and reasoning
& Missed evidence, unsupported claims, incorrect policy application,
  unresolved contradiction, or failure to recognize ambiguity \\

State-changing workflow
& Enterprise action
& Wrong-object mutation, unauthorized action, duplicate execution,
  stale-state error, failed recovery, or consequential downstream effect \\

Open user-facing completion
& Open interaction
& Misunderstood intent, improper policy concession, manipulation,
  privacy leakage, prompt injection, or unsafe behavior \\

\bottomrule
\end{tabular}
\end{table}

When tracks are combined, the relevant requirements are combined rather than
replaced. For example:

\begin{itemize}
    \item a \textbf{customer-facing research assistant} may activate
    Tracks~1 and~3: its claims must be grounded and its interaction must
    remain safe, but it has no state-changing authority;

    \item a \textbf{background prior-authorization workflow} may activate
    Tracks~1 and~2: the agent must interpret records and policy correctly and
    construct the correct submission, but it need not negotiate with a user;

    \item an \textbf{interactive account-service agent} may activate all
    three tracks: it must understand evidence, interact safely with the user,
    and perform or propose state-changing actions under the appropriate
    authority.
\end{itemize}

The consequence class remains orthogonal to this composition. It determines
how serious failures on an active surface are, while the deployment contract
determines which information and actions are actually available to the
agent.

Together, the active tracks, risk surfaces, deployment contract, consequence
class, and selected evaluation primitives define the task's
\emph{evaluation profile}. Section~\ref{sec:qualification} specifies how
measurements from that profile are converted into hard deployment gates,
reliability and autonomy tradeoffs, and oversight economics. The reference
platform in Section~\ref{sec:platform} operationalizes the specification in
controlled agent executions and preserves the resulting artifacts,
trajectories, and enterprise state for evaluation.

==> old/standard_bk_0820.tex <==
% ==================================================================
\section{EFE Evaluation Runtime and Open Interface}
\label{sec:platform}
% ==================================================================

Sections~\ref{sec:overview} and~\ref{sec:qualification} define what EFE
qualifies and how an oversight policy is selected.
This section describes the execution and interface layer that produces the
evidence required by that methodology.

EFE does not introduce a new general-purpose agent-evaluation harness.
Its reference implementation builds on Harbor~\cite{harbor_framework_2026}
for executable task packaging, environment provisioning, agent execution,
verification, trial management, and trajectory recording.
EFE adds the workflow-level specification, evaluation semantics, actor
interfaces, and qualification handoff needed to translate those executions
into a deployment profile.

Harbor is therefore a reference execution substrate rather than a required
EFE runtime.
Another execution system can support EFE provided that it implements the
same logical interfaces and preserves the evidence required for qualification.
The detailed terminology and implementation mapping between EFE and Harbor is
given in Appendix~\ref{app:harbor-mapping}.


% ------------------------------------------------------------------
\subsection{Runtime Layering and Reference Execution Substrate}
\label{sec:platform-layering}
% ------------------------------------------------------------------

The implementation follows the three-layer architecture in
Figure~\ref{fig:efe_overview}.
Non-executing \emph{specification artifacts} define the workflow,
evaluation semantics, and deployment assumptions.
The \emph{evaluation runtime} instantiates these specifications and executes
the agent, environment, and any required oversight or user actors.
The resulting trial evidence is then evaluated and passed to the
qualification methodology in Section~\ref{sec:qualification}.

This separation is intentional.
EFE standardizes the information that must cross these boundaries without
requiring every evaluation to use the same task format, agent harness,
environment implementation, or grader framework.
Existing execution infrastructure can therefore be reused rather than
reimplemented inside EFE.

In the Harbor reference implementation, executable task packaging,
environments, Trials, Verifiers, and trajectory artifacts remain Harbor
objects.
EFE introduces the workflow and deployment semantics above those objects.
The mapping describes an implementation relationship, not a one-to-one
semantic equivalence.


% ------------------------------------------------------------------
\subsection{Specification Interfaces}
\label{sec:platform-specifications}
% ------------------------------------------------------------------

The runtime consumes three logically distinct classes of specification
artifacts corresponding to Figure~\ref{fig:efe_overview}.

\paragraph{Workflow specification.}
The workflow specification identifies the reusable workflow $w$, the
population of task instances represented by $\mathcal{D}_w$, and the
environment specification associated with the workflow.
It defines the work to be performed and the conditions under which the
evaluation instances should be interpreted.
A concrete task instance $x_i$ supplies the case-specific inputs for one
execution.

The interface does not require EFE to introduce a second executable task
format.
In the Harbor reference implementation, a task instance is packaged as a
Harbor \emph{Task}, and an executable collection of instances can be
represented as a Harbor \emph{Dataset}.

\paragraph{Evaluation specification.}
The evaluation specification defines the workflow evaluator $g_w$, the
deployment-success predicate $\phi_w$, and any routing signal that is to be
exposed to an oversight policy.
It therefore specifies how observable execution evidence is transformed as

\begin{equation}
Z_i^\pi
\;\xrightarrow{\;g_w\;}\;
\mathbf{q}_i^\pi
\;\xrightarrow{\;\phi_w\;}\;
u_i^\pi.
\label{eq:platform-evaluation-interface}
\end{equation}

The executable mechanisms used to compute these quantities may be
deterministic programs, human annotations, model-assisted graders, or
compositions of several mechanisms.
When Harbor is used, one or more of these computations may be implemented
through Harbor \emph{Verifiers}; EFE's evaluator denotes the workflow-level
semantics of what is measured rather than a competing execution primitive.

\paragraph{Deployment assumptions.}
Deployment assumptions are kept separate from measured benchmark evidence.
They include the reliability target $Y$, the human-oversight model,
operating-cost assumptions, and any workflow-specific risk tolerance.
They need not be intrinsic properties of a contributed benchmark:
different organizations may apply different deployment assumptions to the
same measured workflow evidence.

The development and held-out qualification partitions required by
Section~\ref{sec:statistical-qualification} are versioned with the evaluation
configuration.
Instances used to select an oversight policy must remain separate from the
instances used to qualify the frozen policy.


% ------------------------------------------------------------------
\subsection{Execution, Actors, and Policy Evaluation}
\label{sec:platform-execution}
% ------------------------------------------------------------------

The evaluation runtime instantiates the workflow environment and executes
agent $m$ on task instance $x_i$ under candidate oversight policy $\pi$.
The runtime is responsible for making the workflow-specified tools, data,
systems, and interaction interfaces available while preserving the declared
evaluation conditions.

For workflows requiring interaction, EFE distinguishes two additional actor
roles.
An \emph{oversight actor} represents the organization-side reviewer or
operator who may approve, clarify, correct, escalate, or take over work.
A \emph{user actor} represents an external user or counterparty interacting
with the deployed system.
Either actor may be implemented by a human or by a simulator for evaluation,
but its identity, configuration, and available actions must be recorded as
part of the evaluation configuration.

The runtime supports both policy-evaluation procedures introduced in
Section~\ref{sec:overview-flow} without treating them as different EFE
deployment models.

For \emph{trajectory-invariant} policies, the relevant agent execution is
independent of the terminal routing decision.
The runtime can therefore execute the agent once, preserve the resulting
trajectory, and evaluate multiple candidate policies by replaying the saved
evidence.
The accept-or-escalate analysis in Section~\ref{sec:accept-escalate} uses
this path.

For \emph{trajectory-dependent} policies, intervention changes what happens
next.
The candidate policy must therefore participate in execution: the runtime
invokes the appropriate oversight or user actor when required by $\pi$ and
records the resulting policy-dependent trajectory $Z_i^\pi$.
Reliability, cost, and risk for that policy are then estimated from executions
or simulations produced under the policy itself.

Thus, replay and policy-in-the-loop execution are two ways of generating the
evidence required to evaluate the same deployment objective.


% ------------------------------------------------------------------
\subsection{Trial Evidence and Workflow Evaluation}
\label{sec:platform-evidence}
% ------------------------------------------------------------------

Each execution produces a \emph{Trial}: the logical unit of evidence for one
agent execution on one task instance under a specified evaluation
configuration.
EFE adopts Harbor's Trial abstraction in the reference implementation rather
than defining a parallel execution-record format.

A Trial should preserve enough information to reconstruct the measurements
used for qualification.
As applicable, this includes the evaluated workflow and task-instance
versions; agent, model, environment, policy, and actor configurations; the
final work product; the observable trajectory and intermediate artifacts;
routing signals; workflow-evaluation outputs; and the resource measurements
needed by the declared cost model.

The workflow evaluator applies $g_w$ to the recorded execution evidence to
produce $\mathbf{q}_i^\pi$, and the pre-specified predicate $\phi_w$ derives
the corresponding success event $u_i^\pi$.
Diagnostic measurements remain available independently of this binary
success event.
For example, an evaluator may retain outcome correctness, evidence grounding,
process adherence, appropriate abstention, and resource use even when only a
subset of those quantities enters $\phi_w$.

EFE does not prescribe a universal trajectory representation.
When Harbor is used, Harbor's native Trial and trajectory artifacts provide
the reference mechanism for preserving messages, tool calls, state changes,
and other observable execution evidence.
If the stored evidence is sufficient, a corrected or updated evaluator may
recompute $\mathbf{q}_i^\pi$ and $u_i^\pi$ without rerunning the agent.
Changes that would have altered the trajectory itself instead require new
execution.

For repeated stochastic executions, all Trials remain associated with their
underlying task instance.
This preserves the sampling structure required by the statistical
qualification procedure in Section~\ref{sec:statistical-qualification}.


\paragraph{Running example: CliniCARE-Bench.}
For CliniCARE-Bench, a Trial contains the completed clinical adjudication,
supporting patient- and policy-evidence citations, the case-level confidence
signal, and the observable investigation trajectory, including retrieved
evidence, tool calls, computations, and intermediate artifacts.
The CliniCARE evaluator derives verdict and process measurements from this
record and applies the workflow-specific success predicate before the
resulting evidence is passed to EFE qualification.


% ------------------------------------------------------------------
\subsection{Qualification Handoff and Deployment Profile}
\label{sec:platform-qualification-handoff}
% ------------------------------------------------------------------

The boundary between workflow evaluation and deployment qualification is an
evidence interface rather than a new task evaluator.
The qualification layer consumes measured evidence together with declared
deployment assumptions and applies the methodology in
Section~\ref{sec:qualification}.

For the trajectory-invariant accept-or-escalate case, the minimal
qualification record for task instance $i$ contains the workflow-defined
success event $u_i$, the routing signal $s_i$, and the execution or resource
measurements needed by the cost model.
Additional identifiers preserve the task instance, evaluation configuration,
and statistical sampling unit.
Section~\ref{sec:statistical-qualification} then selects the policy on
development data and qualifies the frozen operating point on held-out data.

For trajectory-dependent policies, the same logical interface applies, but
the relevant measurements are associated with trajectories generated under
the candidate policy $\pi$.
The evidence record therefore retains the policy and actor configuration
required to interpret $Z_i^\pi$, $u_i^\pi$, and its associated operating
cost.

This separation between measured evidence and deployment assumptions allows
the same evaluated agent behavior to support multiple deployment analyses.
For example, changing the target reliability, reviewer performance, or
reviewer cost can change the qualified operating point without changing the
underlying autonomous Trials.

The output is the \emph{deployment profile} defined in
Section~\ref{sec:overview-flow}: a statistically supported operating point
conditional on the workflow, evaluated system, oversight policy, and declared
deployment assumptions.
The profile is therefore not a context-free model score.
Its purpose is to make explicit the reliability--oversight--cost tradeoff
supported by the evaluation evidence.


% ------------------------------------------------------------------
\subsection{Extending EFE with New Workflows}
\label{sec:platform-contribution}
% ------------------------------------------------------------------

EFE is designed so that a new enterprise evaluation can be added without
changing either the general qualification methodology or the underlying
execution infrastructure.

A contributor supplies an executable workflow implementation together with
the specification artifacts needed by the EFE interface.
The executable layer contains the task instances, environment and required
assets, agent-visible interfaces, and mechanisms needed to compute the
workflow measurements.
When Harbor is used, these components remain native Harbor tasks,
environments, datasets, Trials, and Verifiers.

The EFE-specific contribution defines the workflow identity and represented
population, the evaluation semantics $g_w$ and $\phi_w$, the routing signal
when required by the proposed oversight policy, the development and held-out
qualification partitions, and the measurements needed for operating-cost
analysis.
Reference deployment assumptions may accompany the evaluation, but they must
remain distinguishable from measured evidence so that an organization can
substitute its own reliability target, oversight model, or cost assumptions.

The same interface can be used for public benchmarks and enterprise-internal
evaluations.
EFE does not require proprietary data, internal policies, or protected
reference material to be made public; it requires that the semantics of the
workflow, evaluation, and reported deployment claim remain explicit.

When an existing benchmark is adapted to EFE, the adaptation should preserve
the benchmark's original task, environment, and evaluation semantics.
Execution-system adaptation is an implementation concern; deployment
qualification is the additional analytical layer supplied by EFE.

==> sections/app-standard.tex <==
\section{\EFE{}--Inspect Reference Implementation}
\label{app:inspect-mapping}

Section~\ref{sec:platform} defines the logical interface required by an
\EFE{}-compatible evaluation runtime.
This appendix describes how that interface is realized using Inspect AI
\citep{inspect_ai} and how evaluations already packaged in Harbor can be
executed through Inspect using the \texttt{inspect-harbor} compatibility
adapter \citep{inspect_harbor}.

The mapping is intentionally not one-to-one.
\EFE{} defines workflow and deployment semantics, including the workflow
$w$, workflow-success predicate $\phi_w$, oversight policy $\pi$, and
deployment profile.
Inspect provides execution and evaluation abstractions used to instantiate
those semantics.
The qualification methodology itself remains an \EFE{} layer above the
execution substrate.


% ------------------------------------------------------------------
\subsection{\EFE{}--Inspect Terminology and Interface Mapping}
\label{app:inspect-terminology}
% ------------------------------------------------------------------

Table~\ref{tab:efe-inspect-mapping} summarizes the correspondence between
\EFE{} concepts and their reference realization in Inspect.
The distinction between an \EFE{} task instance and an Inspect
\texttt{Task} is particularly important.
An individual \EFE{} task instance $x_i$ corresponds to an Inspect
\texttt{Sample}; an Inspect \texttt{Task} is the executable evaluation
configuration that determines how a collection of samples is run and scored.
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\textwidth}{L{3.0cm} L{3.8cm} Y}
\toprule
\textbf{\EFE{} concept}
&
\textbf{Inspect realization}
&
\textbf{Relationship}
\\
\midrule

Workflow $w$
&
No direct equivalent
&
\EFE{}-level definition of the reusable enterprise workflow.
\\

Task instance $x_i$
&
\texttt{Sample}
&
One concrete workflow case.
\\

Evaluation sample $S_w$ (drawn from $\mathcal{D}_w$)
&
\texttt{Dataset}
&
Collection of representative task instances.
\\

Executable evaluation
&
\texttt{Task}
&
Binds dataset, agent/solver, scorer(s), and runtime configuration.
\\

Agent $m$
&
\texttt{Agent} / \texttt{Solver}
&
Evaluated agent; external agents may use Agent Bridge.
\\

Workflow environment $E_w$
&
Sandbox, tools, files, runtime configuration
&
Agent-visible data, tools, and execution state.
\\

Actors and oversight policy $\pi$
&
Approvers, intervention, custom agents or policy logic
&
Inspect provides execution primitives; \EFE{} defines actor roles and policy
semantics.
\\

Trajectory and execution evidence $Z_i^\pi$
&
Evaluation log, transcript, outputs, artifacts
&
Observable record used for workflow evaluation and qualification.
\\

Evaluator $g_w$ and measurements $\mathbf{q}_i^\pi$
&
\texttt{Scorer}(s), \texttt{Score}s, metadata
&
Inspect computes and records workflow-specific measurements.
\\

Success predicate $\phi_w$ and routing signal $s_i$
&
\EFE{}-derived success event; output/score/metadata field
&
\EFE{} defines success and the observable signal available to the oversight
policy.
\\

Resource and repeated-run evidence
&
Usage/metadata; epochs
&
Supports operating-cost analysis and repeated executions of the same case.
\\

Deployment qualification and profile
&
No direct equivalent
&
\EFE{} selects and statistically qualifies the oversight policy and reports the
reliability--oversight--cost operating point.
\\

\bottomrule
\end{tabularx}

\caption{
\textbf{\EFE{}--Inspect terminology and implementation mapping.}
Inspect provides the reference execution and scoring substrate; \EFE{} addsworkflow, oversight, and deployment-qualification semantics.
}
\label{tab:efe-inspect-mapping}
\end{table}

Two aspects of this mapping are useful for \EFE{} in particular.
First, Inspect permits multiple scorers and per-sample scores, allowing the
workflow evaluator $g_w$ to retain separate diagnostic measurements before
the \EFE{} success predicate $\phi_w$ is applied.
Second, execution evidence is preserved in evaluation logs, allowing an
updated evaluator to be applied to existing evidence when that evidence is
sufficient.
This realizes the distinction in
Section~\ref{sec:maintenance-requalification} between re-evaluating preserved
executions and rerunning an agent when the underlying trajectory could have
changed.

Inspect also provides runtime primitives for several forms of
trajectory-dependent oversight.
Approval policies can condition execution of selected tool calls on human or
automated approval, while agent-intervention mechanisms allow a human
operator to interrupt or redirect a running agent.
These mechanisms provide implementations of particular oversight actions;
they do not restrict the more general \EFE{} policy definition
$\pi\in\Pi_w$.


% ------------------------------------------------------------------
\subsection{Harbor Compatibility through \texttt{inspect-harbor}}
\label{app:inspect-harbor}
% ------------------------------------------------------------------

Some existing evaluations may already be packaged using Harbor.
\EFE{} does not require such evaluations to be rewritten solely because Inspect
is the reference execution substrate.
The \texttt{inspect-harbor} adapter provides a compatibility path that loads
supported Harbor tasks into Inspect while preserving their executable task,
environment, and verification structure.

At the adapter boundary, the principal mappings are shown in
Table~\ref{tab:harbor-inspect-bridge}.

\begin{table}[t]
\centering
\small
\begin{tabularx}{\textwidth}{L{3.5cm} L{4.0cm} Y}
\toprule
\textbf{Harbor representation}
&
\textbf{Inspect representation}
&
\textbf{Role}
\\
\midrule

Harbor Task
&
\texttt{Sample}
&
One executable evaluation instance.
\\

Harbor Dataset
&
\texttt{Task}
&
Collection of Harbor evaluation instances exposed as an Inspect evaluation
task.
\\

\texttt{instruction.md}
&
\texttt{Sample.input}
&
Agent-visible task instruction.
\\

\texttt{environment/}
&
\texttt{SandboxEnvironmentSpec}
&
Containerized execution environment used by the evaluation instance.
\\

\texttt{tests/test.sh}
&
\texttt{Scorer} (\texttt{harbor\_scorer})
&
Executes the Harbor verification script and converts its reward or metrics
into Inspect scoring output.
\\

\texttt{solution/solve.sh}
&
Oracle \texttt{Solver}
&
Optional reference solution used for task validation or sanity checking.
\\

Harbor task metadata
&
\texttt{Sample.metadata}
&
Carries task identifiers and other benchmark-specific metadata into the
Inspect execution record.
\\

\bottomrule
\end{tabularx}

\caption{
\textbf{Principal Harbor--Inspect mappings implemented by
\texttt{inspect-harbor}.}
The bridge concerns executable evaluation packaging; \EFE{} workflow semantics
and deployment qualification remain unchanged above the adapter.
}
\label{tab:harbor-inspect-bridge}
\end{table}

This compatibility layer is useful for preserving existing benchmark
implementations, but it should not be interpreted as a requirement that \EFE{}
workflows originate in Harbor.
New \EFE{} evaluations can be implemented directly in Inspect using the
interfaces described in Section~\ref{sec:platform}.

\paragraph{Compatibility constraints.}
The bridge does not currently implement every Harbor feature.
At the time of writing, Harbor multi-step tasks using
\texttt{[[steps]]} and \texttt{multi\_step\_reward\_strategy} and
Windows-targeted tasks are not supported.
Harbor-declared MCP servers and agent skill directories are also not exposed
through the bridge, and several less central environment configuration fields
are ignored.
Evaluations relying on these features therefore require either adaptation or
a native Inspect implementation rather than assuming transparent
compatibility.

Consequently, use of the bridge should be validated at the level of the
evaluation semantics, not merely successful task loading.
For an adapted benchmark, the task instructions, agent-visible information,
environment behavior, evaluation logic, and retained evidence should be
checked against the original implementation before the resulting execution is
used for \EFE{} qualification.

This yields the intended layering:

\begin{center}
\textbf{Harbor packaging, when present}
$\;\longrightarrow\;$
\textbf{\texttt{inspect-harbor} adapter}
$\;\longrightarrow\;$
\textbf{Inspect execution and evidence}
$\;\longrightarrow\;$
\textbf{\EFE{} deployment qualification}.
\end{center}

The adapter is therefore an implementation compatibility mechanism rather
than part of the \EFE{} standard or qualification methodology.

==> sections/contribution.tex <==
% ==================================================================
\section{Evaluation Contributions and Benchmark Evolution}
\label{sec:evolution}
% ==================================================================

\EFE{} supports new enterprise workflows without changing the
qualification methodology introduced in Section~\ref{sec:qualification}.
Interface compatibility alone, however, is not sufficient for a meaningful
deployment claim.
A contributed evaluation must represent authentic work, produce trustworthy
evaluation evidence, and preserve the conditions under which its resulting
deployment profile was qualified.

This section addresses three questions: what is required for a new evaluation contribution to be considered valid; how an \EFE{} result is tied to a versioned evaluation lineage; and when changes to that lineage require recomputation, re-evaluation, or new execution.


% ------------------------------------------------------------------
\subsection{Contribution and Validation}
\label{sec:contribution-validation}
% ------------------------------------------------------------------

A new \EFE{} contribution consists of the executable workflow evaluation and the
specification artifacts described in Section~\ref{sec:platform-contribution}.
Conformance to those interfaces establishes interoperability; validation
establishes whether the resulting evidence supports a meaningful deployment
qualification.

Validation is an auditable acceptance procedure, not a set of aspirational
principles. It is carried out by a reviewer independent of the
contributor---a benchmark maintainer or a designated evaluation
reviewer---who, for each of the four aspects below, checks
contributor-supplied evidence against an explicit acceptance criterion and
records a pass-or-fail verdict. A contribution is accepted for a
qualification release only if all four checks pass; a failing check blocks the
release until it is resolved, or is waived with a documented, publicly
recorded justification. The submitted evidence and the reviewer's verdicts are
stored as part of the evaluation lineage (Section~\ref{sec:evaluation-lineage}),
so that a ``valid contribution'' denotes a reproducible, challengeable judgment
rather than a subjective label. Validation should address at least four aspects.

\paragraph{Workflow validity.}
The contributed workflow should represent a recognizable form of enterprise
work with a clearly defined output or end state.
Its task instances should sample the population for which the eventual
deployment claim is intended.
The objective is not to maximize benchmark difficulty, but to construct an
evaluation in which success, failure, and the need for oversight are
representative of the workflow being qualified.

\paragraph{Evaluation validity.}
The evaluator $g_w$ and success predicate $\phi_w$ must faithfully encode the
workflow's intended evaluation semantics.
References, rubrics, deterministic checks, or expert judgments used by the
evaluator should be validated for correctness and reproducibility.
Where process measurements contribute to $\phi_w$, the execution record must
contain sufficient observable evidence to determine those measurements
without relying on unrecorded model reasoning.

\paragraph{Execution validity.}
The executable environment should provide the information and tools declared
by the workflow specification while preventing unintended access to hidden
references or evaluation-only information.
Representative dry runs should be used to identify broken tasks, environment
failures, evaluator instability, leakage, and unintended shortcuts before a
qualification release is frozen.

\paragraph{Qualification validity.}
The contribution must define the sampling unit and the development and
held-out qualification partitions required by
Section~\ref{sec:statistical-qualification}.
Policy choices must be made without using the held-out qualification data.
The release should also document the represented population, known
limitations, and any deployment assumptions used to produce reference
deployment profiles.

\paragraph{Validation record.}
To keep these checks auditable rather than advisory, each names the evidence the
contributor must supply and the condition under which a reviewer marks it
\emph{pass}:
\begin{itemize}
  \item \textbf{Workflow validity} --- a workflow description, representative
  task instances, and a statement of the represented population. \emph{Pass if}
  an independent reviewer confirms the task is a recognizable form of the claimed
  enterprise work and the instances are drawn from the stated population.
  \item \textbf{Evaluation validity} --- the evaluator $g_w$ and predicate
  $\phi_w$ with their references, rubrics, and deterministic checks, plus
  human-agreement statistics on a labeled subset. \emph{Pass if} independent
  re-scoring reproduces the contributor's success labels within a pre-registered
  tolerance and every process condition in $\phi_w$ is decidable from observable
  execution evidence.
  \item \textbf{Execution validity} --- reproducible dry-run logs including a
  reference/oracle solver and at least one failing agent, together with a
  leakage-and-shortcut audit. \emph{Pass if} the reviewer reproduces those runs
  from the pinned environment manifest and finds no hidden-reference access,
  evaluator instability, or unintended shortcut.
  \item \textbf{Qualification validity} --- the declared sampling unit, the
  frozen development/held-out partition, and evidence that policy selection never
  accessed the held-out set. \emph{Pass if} the partition is reproducible from
  the recorded seed and manifest (Section~\ref{sec:evaluation-lineage}) and the
  held-out data are demonstrably untouched during selection.
\end{itemize}
Because the required evidence and pass conditions are fixed in advance, any third
party can re-run the recorded procedure and reach the same accept-or-reject
decision; a ``valid contribution'' is therefore falsifiable rather than a matter
of reviewer opinion.

These requirements apply equally to public and enterprise-internal
evaluations.
\EFE{} does not require proprietary task data, governed assets, or hidden
references to be released publicly.
Protected evaluations may use gated, private, or server-side execution,
provided that the workflow semantics, evaluation procedure, and assumptions
underlying the reported qualification remain explicit.


% ------------------------------------------------------------------
\subsection{Versioned Evaluation Lineage}
\label{sec:evaluation-lineage}
% ------------------------------------------------------------------

An \EFE{} deployment profile is conditional on the complete configuration that
produced it.
A result should identify a versioned \emph{evaluation lineage},
not merely a benchmark name or model name.

At minimum, the lineage identifies the versions of the workflow and task
population, evaluated agent and model configuration, execution environment,
workflow evaluator and success predicate, routing signal, and the evidence
used for qualification. To make the evaluation \emph{re-instantiable} rather
than merely named, each version is pinned to a concrete build identifier:
source-control commit hashes for the workflow, evaluator, and harness code;
pinned software dependencies and a container image digest; the random seeds
governing task sampling, the development/held-out split, and any stochastic
execution; and the runtime configuration, including model and provider
identifiers, decoding parameters, and hardware where it materially affects
results.
For trajectory-dependent evaluations, it additionally records the oversight
policy and the relevant oversight- and user-actor configurations.
The deployment profile further records the deployment assumptions under which
the evidence was interpreted, including the reliability target, human-review
model, cost assumptions, and any workflow-specific risk constraint.

Conceptually, a qualification claim has the form

\begin{equation}
\text{evaluation lineage}
\;+\;
\text{deployment assumptions}
\;\longrightarrow\;
\text{deployment profile}.
\label{eq:evaluation-lineage-profile}
\end{equation}

This distinction mirrors the architecture in Figure~\ref{fig:efe_overview}.
The evaluation lineage determines the measured evidence, whereas the
deployment assumptions determine how that evidence is converted into an
operating point.

Versioning these components separately is useful because different changes
have different consequences.
A new deployment assumption need not imply that the agent should be rerun,
while a change to the execution environment may invalidate the original
trajectory.
Similarly, a corrected evaluator may sometimes be applied to preserved execution
evidence without repeating agent execution.

Historical results should remain tied to the lineage under which they were
produced.
Corrections or subsequent releases create new evaluation records
instead of silently changing the interpretation of an earlier deployment
profile.


% ------------------------------------------------------------------
\subsection{Maintenance and Requalification}
\label{sec:maintenance-requalification}
% ------------------------------------------------------------------

Enterprise workflows, evaluation criteria, execution environments, and agent
systems evolve.
\EFE{} treats qualification as a versioned claim whose continued
validity depends on what has changed.

The architecture yields three common cases.

\paragraph{Recompute from existing qualified evidence.}
If only deployment assumptions change---for example, the target reliability,
human-review performance, or review cost---the underlying agent evidence is
unchanged.
Where the existing qualification data support the new analysis, \EFE{} can
recompute the oversight policy and deployment profile without rerunning the
agent.
The resulting profile must record the new assumptions and constitutes a new
qualification claim.

\paragraph{Re-evaluate preserved execution evidence.}
If the workflow evaluator, grader implementation, or workflow-success predicate changes,
existing execution records may sometimes remain sufficient. Re-evaluation is permitted
\emph{only} when the preserved trajectory $Z_i$ contains every input the revised evaluator
$g_w'$ consumes: if the new evaluator reads a field, tool result, retrieved source, or
intermediate artifact that was not recorded, the trajectory is insufficient for that case
and it must be re-executed rather than re-evaluated. When this condition holds for all
qualification cases, \EFE{} recomputes the workflow measurements
$\mathbf{q}_i = g_w'(Z_i)$ and success events $u_i = \phi_w'(\mathbf{q}_i)$ from the saved
records and repeats deployment qualification on the updated evidence, with no new agent
execution. The new evaluator and resulting profile receive new versions; the original
result remains traceable.

\paragraph{Re-execute and requalify.}
New execution is required when a change can alter the trajectory being
evaluated or the population to which the qualification claim applies.
Examples include material changes to the agent or model, agent harness,
workflow inputs, available tools or information, execution environment,
interactive actor behavior, or represented task distribution.
For trajectory-dependent policies, a material change to the oversight policy
may likewise require new policy-in-the-loop execution.
The resulting evidence must then pass the same development and held-out
qualification procedure as a new evaluation.

This distinction can be summarized as

\begin{center}
\textbf{assumptions change}
$\;\rightarrow\;$ recompute the profile,
\\
\textbf{evaluation changes}
$\;\rightarrow\;$ re-evaluate if evidence is sufficient,
\\
\textbf{trajectory or population changes}
$\;\rightarrow\;$ re-execute and requalify.
\end{center}

\paragraph{Worked example: the post-CT AKI audit.}
Consider a frozen deployment profile for the acute-kidney-injury audit of
Section~\ref{sec:overview-clinicare}: agent $m$ under the KDIGO evaluator, an
accept-or-escalate threshold $\widehat\tau$ selected on $S_{\mathrm{dev}}$, qualified at
target $Y=0.76$ under review assumption $a_h=0.90$. The three cases determine what a given
change requires.
\begin{itemize}
  \item \textbf{Recompute} (assumptions change). The organization tightens the target to
  $Y=0.80$, or lowers the review assumption to $a_h=0.85$, or revises the review-cost
  estimate. The agent executions and their measured $u_i,s_i$ are unchanged, so \EFE{}
  re-optimizes $\widehat\tau$ and recomputes the deployment profile directly from the
  existing qualification records. The result is a new qualification claim that records the
  new assumptions; no agent is rerun.
  \item \textbf{Re-evaluate} (evaluation changes). The success predicate is revised so that
  $\phi_w'$ additionally requires the agent to have established baseline creatinine using
  the specified hierarchy. This is admissible without re-execution only if every preserved
  trajectory records the baseline-creatinine value and its provenance that the new check
  reads. Where it does, \EFE{} recomputes $\mathbf{q}_i$ and $u_i$ from the logs and
  requalifies the frozen policy on the updated success events. Where a case never logged
  that provenance, it fails the sufficiency condition above and drops to re-execution.
  \item \textbf{Re-execute} (trajectory or population changes). The EHR retrieval tool is
  upgraded, the agent model or harness is changed, or the post-CT window is widened from
  $48$ to $72$ hours. Any of these can change the trajectory that would be produced, or the
  population the claim covers, so the agent must be rerun and the result passed through the
  same development and held-out qualification procedure as a new evaluation.
\end{itemize}

Task defects, reference errors, or evaluator errors should be corrected
through explicit versions or errata rather than by overwriting historical
results.
Likewise, an evaluation should be refreshed or retired when its workflow is
no longer representative, its evaluation can no longer be trusted, or its
qualification set no longer provides meaningful evidence for the intended
population.

\EFE{} treats deployment qualification not as a permanent property of
an agent, but as an evidence-backed claim attached to a specific evaluation
lineage and deployment context.
This provides the continuity needed for an open and evolving evaluation
ecosystem while preserving the meaning of previously reported results.

==> sections/pse-results.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
& Model & M1 & M7 & Token & \multicolumn{2}{c}{$Y=95\%$} & \multicolumn{2}{c}{$Y=98\%$}\\
\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Tier & & acc. & unc. & \$/case & esc. & \$/case & esc. & \$/case\\
\midrule
Closed frontier & GPT-5.5 & 94.6 & 79.7 & 0.048 & 2\% & 0.45 & 30\% & 7.45\\
 & GPT-5 & 90.2 & 12.8 & 0.048 & 49\% & 12.40 & 87\% & 21.80\\
 & Claude Opus 4.7 & 92.3 & 57.1 & 0.130 & 17\% & 4.38 & 64\% & 16.23\\
 & Claude Sonnet 4.6 & 84.6 & 49.2 & 0.078 & 58\% & 14.48 & 87\% & 21.88\\
 & Gemini 3.1 Pro & 95.3 & 74.0 & 0.048 & 0\% & 0.05 & 26\% & 6.45\\
 & Gemini 2.5 Flash & 85.8 & 31.3 & 0.012 & 60\% & 15.11 & 89\% & 22.31\\
Open frontier & DeepSeek-R1 & 83.7 & 36.3 & 0.012 & 64\% & 16.11 & 90\% & 22.51\\
 & Qwen3-235B & 76.7 & 18.3 & 0.004 & 79\% & 19.85 & 95\% & 23.70\\
 & GPT-OSS-120B & 79.0 & 10.0 & 0.003 & 78\% & 19.60 & 95\% & 23.65\\
Small & GPT-5-nano & 71.9 & 10.1 & 0.002 & 84\% & 21.05 & 96\% & 24.00\\
 & Llama-3.1-8B & 52.4 & 10.5 & 0.000 & 91\% & 22.75 & 98\% & 24.45\\
 & Mistral-Small 3.2 & 60.5 & 2.2 & 0.001 & 90\% & 22.40 & 97\% & 24.35\\
Medical & HuatuoGPT-o1 8B & 45.5 & 2.3 & 0.001 & 93\% & 23.15 & 98\% & 24.55\\
 & MedGemma 27B & 51.3 & 0.0 & 0.001 & 92\% & 22.95 & 98\% & 24.50\\
 & HuatuoGPT-o1 70B & 61.1 & 3.6 & 0.006 & 89\% & 22.31 & 97\% & 24.36\\
\bottomrule
\end{tabular}


